Tracking Most Significant Shifts in Infinite-Armed Bandits

We study an infinite-armed bandit problem where actions' mean rewards are initially sampled from a reservoir distribution. Most prior works in this setting focused on stationary rewards (Berry et al., 1997; Wang et al., 2008; Bonald and Proutiere, 2013; Carpentier and Valko, 2015) with the more challenging adversarial/non-stationary variant only recently studied in the context of rotting/decreasing rewards (Kim et al., 2022; 2024). Furthermore, optimal regret upper bounds were only achieved using parameter knowledge of non-stationarity and only known for certain regimes of regularity of the reservoir. This work shows the first parameter-free optimal regret bounds for all regimes while also relaxing distributional assumptions on the reservoir. We first introduce a blackbox scheme to convert a finite-armed MAB algorithm designed for near-stationary environments into a parameter-free algorithm for the infinite-armed non-stationary problem with optimal regret guarantees. We next study a natural notion of significant shift for this problem inspired by recent developments in finite-armed MAB (Suk & Kpotufe, 2022). We show that tighter regret bounds in terms of significant shifts can be adaptively attained by employing a randomized variant of elimination within our blackbox scheme. Our enhanced rates only depend on the rotting non-stationarity and thus exhibit an interesting phenomenon for this problem where rising rewards do not factor into the difficulty of non-stationarity.

==> impact.tex <==
\section*{Impact Statement}

As our contribution here is primarily theoretical, advancing the state-of-art in infinite-armed non-stationary bandits, we do not foresee any major societal impact concerns.
%This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.

==> joe/joe_icml_preamble.tex <==
%\NeedsTeXFormat{LaTeX2e}
%\ProvidesClass{joe_icml}[2014/08/16 Example LaTeX class]

% misc starter packages
%\usepackage{fullpage}
%\usepackage{authblk} % getting rid of this makes author list on same line
\usepackage{blindtext}
\usepackage{booktabs} % for professional tables
\usepackage{makecell} % for makecell command for line breaks in table cells
\usepackage[round]{natbib}
\usepackage{url}
\usepackage{wrapfig} % for wrapping figure inside paragraph
%\restylefloat{figure} % to allow for caption or \captionlistentry{} inside wrapfig
\usepackage{caption}
%\usepackage{bookmark} % suggested by slow arxiv.tex
%\usepackage{labelschanged}

% For theorems and such
%\usepackage[amsmath]{ntheorem}
%\usepackage{thmtools}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{nameref}
\usepackage{hyperref}
\usepackage[capitalize,noabbrev]{cleveref}


\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{graphicx}
%\usepackage[right=1in,left=1in,top=1in,bottom=1in]{geometry}
\usepackage[svgnames,dvipsnames]{xcolor}
\usepackage{mathrsfs,bm}
\usepackage{amssymb}
\usepackage{titlesec}
\usepackage{tikz-cd}
\usepackage[most]{tcolorbox}
\usepackage{etoolbox}
\setlength{\parindent}{0in}
\setlength{\parskip}{0.5em}
%\usepackage{listings}
%\usepackage{color}
%\usepackage{nameref}
\usepackage{ stmaryrd }
%\usepackage{tgbonum}
%\usepackage[sfdefault]{noto}
%\usepackage[sfdefault]{roboto}
\usepackage[T1]{fontenc}
\usepackage[shortlabels]{enumitem}


\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{fancyhdr}
%\usepackage[obeyFinal,textsize=scriptsize,shadow]{todonotes}
\usepackage{mathtools}
\usepackage{microtype}
\usepackage[normalem]{ulem}
\usepackage{stmaryrd}
\usepackage{wasysym}
\usepackage{multirow}
\usepackage{prerex}

\theoremstyle{plain}
% \usepackage{titlesec}

% \titleformat{\chapter}[block]
%   {\normalfont\huge\bfseries}{\thechapter}{20pt}{}
% \titlespacing*{\chapter}
%   {0pt}{20pt}{20pt}

\setcounter{tocdepth}{5}
\setcounter{secnumdepth}{5}


%\usepackage{joe_macros}


% section formatting
\titleformat{\section}[block]{\color{black}\Large\bfseries}{\thesection}{1em}{}
\titleformat{\subsection}[hang]{\color{black}\large\bfseries}{\thesubsection}{1em}{}

\titleformat{\subsubsection}[hang]{\color{black}\large\bfseries}{\thesubsubsection}{1em}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{cor}[thm]{Corollary}
%\theoremstyle{definition} % don't italicize environments in articles
\newtheorem{definition}{Definition}
%\newtheorem*{notation}[theorem]{Notation}
\newtheorem{condition}{Condition}
\newtheorem{assumption}{Assumption}
%\theoremstyle{remark}
%\theoremstyle{definition}
\newtheorem{remark}{Remark}
\newtheorem{rmk}{Remark}
\newtheorem{conj}[thm]{Conjecture}
%\newtheorem{definition}[thm]{Definition}
%\newtheorem{assumption}[thm]{Assumption}
\newtheorem*{assumption*}{Assumption}
\newtheorem{note}[thm]{Notation}
\newtheorem{defn}[thm]{Definition}
\newtheorem{fact}[thm]{Fact}
%\newtheorem{prop}[prop]{Proposition}
\newtheorem{answer}[thm]{Answer}
\newtheorem{ques}[thm]{Question}
\newtheorem{goal}{Goal}
\newtheorem{exer}[thm]{Exercise}
\newtheorem{prob}[thm]{Problem}
\newtheorem*{conj*}{Conjecture}
\newtheorem*{defn*}{Definition}
\newtheorem*{note*}{Notation}
\newtheorem*{fact*}{Fact}
%\newtheorem*{answer*}{Answer}
\newtheorem*{ques*}{Question}
\newtheorem*{exer*}{Exercise}
\newtheorem*{prob*}{Problem}
\newtheorem{algo}{Algorithm}
\newtheorem*{algo*}{Algorithm}


% solution environment
\renewcommand{\qedsymbol}{$\blacksquare$} % change qed symbol to blacksquare
\newenvironment{sol}
  {\renewcommand\qedsymbol{$\blacksquare$}\begin{proof}[Solution]}
  {\end{proof}}
\newenvironment{solution}
  {\renewcommand\qedsymbol{$\blacksquare$}\begin{proof}[Solution]}
  {\end{proof}}

% solution block
\usepackage{cleveref}
\usepackage[most]{tcolorbox}
\newtcbtheorem{solb}{Solution}{
                lower separated=false,
                colback=white!80!gray,
colframe=white, fonttitle=\bfseries,
colbacktitle=white!50!gray,
coltitle=black,
enhanced,
breakable,
boxed title style={colframe=black},
attach boxed title to top left={xshift=0.5cm,yshift=-2mm},
}{solb}

% cleveref setup shortened
%\Crefname{defn}{Defn.}{Defn.}
%\Crefname{definition}{Defn.}{Defn.}
%\Crefname{rmk}{Rem.}{Rem.}
%\Crefname{prop}{Prop.}{Prop.}
%\Crefname{thm}{Thm.}{Thm.}
%\Crefname{theorem}{Thm.}{Thm.}
%\Crefname{cor}{Cor.}{Cor.}
%\Crefname{lemma}{Lem.}{Lem.}
%\Crefname{algo}{Alg.}{Alg.}
%\Crefname{ex}{Ex.}{Ex.}
%\Crefname{answer}{Answer}{Answers}
%\Crefname{ques}{Question}{Questions}
%\Crefname{prob}{Problem}{Problems}
%\Crefname{assumption}{Assumption}{Assumptions}
%\Crefname{note}{Notation}{Notations}
%\Crefname{fact}{Fact}{Facts}
%\Crefname{exer}{Exercise}{Exercises}
%\Crefname{conj}{Conjecture}{Conjectures}
%\Crefname{claim}{Claim}{Claims}
%\Crefname{figure}{Fig.}{Fig.}
%\Crefname{subsection}{Subsec.}{Subsec.}
%\Crefname{section}{Sec.}{Sec.}
%\Crefname{appendix}{App.}{App.}
%\Crefname{table}{Table}{Tables}
%\crefformat{equation}{(#2#1#3)}
%\Crefname{algocf}{Alg.}{Alg.}
%\Crefname{algocfproc}{Alg.}{Alg.}

% cleveref setup long
\Crefname{defn}{Definition}{Definitions}
\Crefname{definition}{Definition}{Definitions}
\Crefname{rmk}{Remark}{Remarks}
\Crefname{prop}{Proposition}{Propositions}
\Crefname{thm}{Theorem}{Theorems}
\Crefname{theorem}{Theorem}{Theorems}
\Crefname{cor}{Corollary}{Corollaries}
\Crefname{lemma}{Lemma}{Lemmas}
\Crefname{algo}{Algorithm}{Algorithms}
\Crefname{ex}{Example}{Examples}
\Crefname{answer}{Answer}{Answers}
\Crefname{ques}{Question}{Questions}
\Crefname{prob}{Problem}{Problems}
\Crefname{assumption}{Assumption}{Assumptions}
\Crefname{note}{Notation}{Notations}
\Crefname{fact}{Fact}{Facts}
\Crefname{exer}{Exercise}{Exercises}
\Crefname{conj}{Conjecture}{Conjectures}
\Crefname{claim}{Claim}{Claims}
\Crefname{figure}{Figure}{Figures}
\Crefname{subsection}{Subsection}{Subsections}
\Crefname{section}{Section}{Sections}
\Crefname{appendix}{Appendix}{Appendices}
\Crefname{table}{Table}{Tables}
\crefformat{equation}{(#2#1#3)}
\Crefname{algocf}{Algorithm}{Algorithms}
\Crefname{algocfproc}{Algorithm}{Algorithms}

% algorithms stuff

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% algorithm2e
\usepackage[algo2e, vlined, ruled, linesnumbered]{algorithm2e}
% algorithm2e commenting
%\newcommand{\com}[1]{{\color{red}\textbf{[[} #1 \textbf{]]}}}
%\newcommand\mycommfont[1]{\footnotesize\textcolor{black}{#1}}
\newcommand\mycommfont[1]{\textcolor{black}{#1}}
\SetCommentSty{mycommfont}

\usepackage{etoolbox}  % patch def of algorithmic environment
\makeatletter
\patchcmd{\algorithmic}{\addtolength{\ALC@tlm}{\leftmargin} }{\addtolength{\ALC@tlm}{\leftmargin}}{}{}
\makeatother


\newenvironment{protocol}[1][htb]
  {\renewcommand{\algorithmcfname}{Protocol}% Update algorithm name
   \begin{algorithm2e}[#1]%
   }{\end{algorithm2e}}


\newenvironment{exampl}[1][htb]
  {%\refstepcounter{examcounter}\par\medskip
  \renewcommand{\algorithmcfname}{Algorithm}
   \begin{algorithm2e}[#1]%
   }{\end{algorithm2e}}


\newenvironment{procedures}[1][htb]
  {\renewcommand{\algorithmcfname}{Procedure}% Update algorithm name
   \begin{algorithm2e}[#1]%
   }{\end{algorithm2e}}

\def\QED{{\phantom{x}} \hfill \ensuremath{\rule{1.3ex}{1.3ex}}}
\newcommand{\extraproof}[1]{\rm \trivlist

\item[\hskip \labelsep{\bf Proof of #1. }]}
\def\endextraproof{\QED \endtrivlist}

\newenvironment{rtheorem}[3][]{

\bigskip

\noindent \ifthenelse{\equal{#1}{}}{\bf #2 #3}{\bf #2 #3 (#1)}
\begin{it}
}{\end{it}}

\newcommand{\nonl}{\renewcommand{\nl}{\let\nl}}
\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}
\newcommand{\obs}{o}

% enable do while
\SetKwRepeat{Do}{do}{while}

% number one line of align*
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% fix algorithm2e labelling by cleverref
\crefalias{AlgoLine}{line}%
\makeatletter
\let\cref@old@stepcounter\stepcounter
\def\stepcounter#1{%
  \cref@old@stepcounter{#1}%
  \cref@constructprefix{#1}{\cref@result}%
  \@ifundefined{cref@#1@alias}%
    {\def\@tempa{#1}}%
    {\def\@tempa{\csname cref@#1@alias\endcsname}}%
  \protected@edef\cref@currentlabel{%
    [\@tempa][\arabic{#1}][\cref@result]%
    \csname p@#1\endcsname\csname the#1\endcsname}}
\makeatother

% tags for underbrace in equation
\usepackage{mathtools}% http://ctan.org/pkg/mathtools
\makeatletter
\newcommand{\mytag}[2]{%
  \text{#1}%
  \@bsphack
  \begingroup
    \@onelevel@sanitize\@currentlabelname
    \edef\@currentlabelname{%
      \expandafter\strip@period\@currentlabelname\relax.\relax\@@@%
    }%
    \protected@write\@auxout{}{%
      \string\newlabel{#2}{%
        {#1}%
        {\thepage}%
        {\@currentlabelname}%
        {\@currentHref}{}%
      }%
    }%
  \endgroup
  \@esphack
}
\makeatother



% colors and hypersetup
\definecolor{aqua}{rgb}{0.0, 1.0, 1.0}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{charcoal}{rgb}{0.21, 0.27, 0.31}

\hypersetup{
	%backref=true,
    %pagebackref=true,
    %hyperindex=true,
    colorlinks=true,
    breaklinks=true,
	citecolor=Mulberry,
	filecolor=black,
	linkcolor=azure,
	urlcolor=PineGreen,
	linkbordercolor=blue
}


% table of contents spacing
\usepackage{subfigure}
\usepackage[subfigure]{tocloft}
\setlength{\cftbeforesecskip}{5pt}

% citation style

% wrapfig stuff
\makeatletter
\def\clearwf{\par{\count@\c@WF@wrappedlines\zz}\par}

\def\zz{{%
\ifnum\count@>\@ne
\noindent\mbox{zz}\\%
\advance\count@\m@ne
\expandafter\zz
\else
\ifhmode\unskip\unpenalty\fi
\fi}}

\makeatother


==> joe/joe_notes_preamble.tex <==
%\NeedsTeXFormat{LaTeX2e}
%\ProvidesClass{joe_notes}[2014/08/16 Example LaTeX class]


\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage[right=0.5cm,left=0.5cm,top=1.5cm,bottom=2cm]{geometry}
\usepackage[svgnames,dvipsnames]{xcolor}
\usepackage{mathrsfs,amsmath,bm}
\usepackage{amssymb}
\usepackage{titlesec}
\usepackage{tikz-cd}
\usepackage{hyperref}
\usepackage[most]{tcolorbox}
\usepackage{etoolbox}
\usepackage[round]{natbib}
\usepackage{url}
\usepackage{makecell} % allow for line breaks in cell of array
\setlength{\parindent}{0in}
\setlength{\parskip}{0.5em}
%\usepackage{listings}
%\usepackage{color}
%\usepackage{nameref}
\usepackage{ stmaryrd }
%\usepackage{tgbonum}
\usepackage[sfdefault]{noto}
%\usepackage[sfdefault]{roboto}
\usepackage[T1]{fontenc}
\usepackage[shortlabels]{enumitem}


\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{fancyhdr}
%\usepackage[obeyFinal,textsize=scriptsize,shadow]{todonotes}
\usepackage{mathtools}
\usepackage{microtype}
\usepackage[normalem]{ulem}
\usepackage{stmaryrd}
\usepackage{wasysym}
\usepackage{multirow}
\usepackage{prerex}
\usepackage{hyperref}
\usepackage[capitalize,noabbrev]{cleveref}


\usepackage{amsthm}
\theoremstyle{plain}
% \usepackage{titlesec}

% \titleformat{\chapter}[block]
%   {\normalfont\huge\bfseries}{\thechapter}{20pt}{}
% \titlespacing*{\chapter}
%   {0pt}{20pt}{20pt}

\setcounter{tocdepth}{5}
\setcounter{secnumdepth}{5}


%\usepackage{joe_macros}


% section formatting
\titleformat{\section}[block]{\color{violet}\Large\bfseries}{\thesection}{1em}{}
\titleformat{\subsection}[hang]{\color{violet}\large\bfseries}{\thesubsection}{1em}{}

\titleformat{\subsubsection}[hang]{\color{violet}\large\bfseries}{\thesubsubsection}{1em}{}

%% theorems

% solution environment
\renewcommand{\qedsymbol}{$\blacksquare$} % change qed symbol to blacksquare
\newenvironment{sol}
  {\renewcommand\qedsymbol{$\blacksquare$}\begin{proof}[Solution]}
  {\end{proof}}
\newenvironment{solution}
  {\renewcommand\qedsymbol{$\blacksquare$}\begin{proof}[Solution]}
  {\end{proof}}

% solution block
\usepackage{cleveref}
%\usepackage[most]{tcolorbox}
\newtcbtheorem{solb}{Solution}{
                lower separated=false,
                colback=white!80!gray,
colframe=white, fonttitle=\bfseries,
colbacktitle=white!50!gray,
coltitle=black,
enhanced,
breakable,
boxed title style={colframe=black},
attach boxed title to top left={xshift=0.5cm,yshift=-2mm},
}{solb}


% napkin theorem style
\usepackage{thmtools}
\usepackage[framemethod=TikZ]{mdframed}

\newenvironment{boxtype1}
  {%
  \begin{mdframed}[
    linewidth=.5,
    everyline=true,
    %margin=8.5,
    backgroundcolor=gray!2,
    linecolor=red,
    fontcolor=black,
    roundcorner=10pt,
    middlelinewidth=2pt,
    splittopskip=25pt,
    secondextra={
      \node[
        overlay,
        fill=white,
        anchor=west,
        font=\sffamily\large,
        inner xsep=10pt
      ] at ([xshift=10pt]O|-P) {Excursus (Cont.)};
      },
    middleextra={
      \node[
        overlay,
        fill=white,
        anchor=west,
        font=\sffamily\large,
        inner xsep=10pt
      ] at ([xshift=10pt]O|-P) {Excursus (Cont.)};
      }
  ]%
  \fontsize{12}{14}\sffamily\selectfont%
  }
  {\end{mdframed}}

\theoremstyle{definition}
\mdfdefinestyle{mdbluebox}{%
	roundcorner = 5pt,
	frametitlerule=true,
	linewidth=1pt,
	skipabove=12pt,
	innerbottommargin=9pt,
	skipbelow=2pt,
	linecolor=RedViolet,
	backgroundcolor=WildStrawberry!20,
}
\declaretheoremstyle[
	headfont=\sffamily\bfseries\color{RoyalPurple},
	mdframed={style=mdbluebox},
	spaceabove=7pt,
	headpunct={\\[5pt]},
	postheadspace={0pt}
]{thmbluebox}

\mdfdefinestyle{pinegreenbox}{%
	linewidth=0.5pt,
	skipabove=12pt,
	frametitleaboveskip=5pt,
	frametitlebelowskip=0pt,
	skipbelow=2pt,
	frametitlefont=\bfseries,
	innertopmargin=4pt,
	innerbottommargin=8pt,
	linecolor=PineGreen,
	backgroundcolor=SeaGreen!10,
}
\declaretheoremstyle[
	headfont=\bfseries\color{PineGreen},
	mdframed={style=pinegreenbox},
	spaceabove=7pt,
	headpunct={\\[3pt]},
	postheadspace={0pt},
]{thmpinegreenbox}
\declaretheoremstyle[
	headfont=\bfseries\color{RedOrange},
	mdframed={style=mdanswerbox},
	spaceabove=7pt,
	headpunct={\\[3pt]},
	postheadspace={0pt},
]{thmanswerbox}



\mdfdefinestyle{mdgreenbox}{%
	skipabove=8pt,
	linewidth=2pt,
	rightline=false,
	leftline=true,
	topline=false,
	bottomline=false,
	linecolor=ForestGreen,
	backgroundcolor=ForestGreen!5,
}
\declaretheoremstyle[
	headfont=\bfseries\sffamily\color{ForestGreen!70!black},
	bodyfont=\normalfont,
	spaceabove=2pt,
	spacebelow=1pt,
	mdframed={style=mdgreenbox},
	headpunct={ --- },
]{thmgreenbox}

\declaretheoremstyle[
	headfont=\bfseries\sffamily\color{ForestGreen!70!black},
	bodyfont=\normalfont,
	spaceabove=2pt,
	spacebelow=1pt,
	mdframed={style=mdgreenbox},
	headpunct={},
]{thmgreenbox*}

\mdfdefinestyle{mdblackbox}{%
	skipabove=8pt,
	linewidth=3pt,
	rightline=false,
	leftline=true,
	topline=false,
	bottomline=false,
	linecolor=black,
	backgroundcolor=RedViolet!5!gray!5,
}
\mdfdefinestyle{mdanswerbox}{%
	linewidth=0.5pt,
	skipabove=12pt,
	frametitleaboveskip=5pt,
	frametitlebelowskip=0pt,
	skipbelow=2pt,
	frametitlefont=\bfseries,
	innertopmargin=4pt,
	innerbottommargin=8pt,
	nobreak=true,
	linecolor=Melon,
	backgroundcolor=Dandelion!10,
}
\declaretheoremstyle[
	headfont=\bfseries,
	bodyfont=\normalfont\small,
	spaceabove=0pt,
	spacebelow=0pt,
	mdframed={style=mdblackbox}
]{thmblackbox}


\declaretheorem[style=thmbluebox,name=Theorem,numberwithin=section]{thm}
\declaretheorem[style=thmbluebox,name=Theorem,numberwithin=section]{theorem}
\declaretheorem[style=thmbluebox,name=Lemma,sibling=thm]{lemma}
\declaretheorem[style=thmbluebox,name=Lemma,sibling=thm]{lem}
\declaretheorem[style=thmbluebox,name=Proposition,sibling=thm]{prop}
\declaretheorem[style=thmbluebox,name=Corollary,sibling=thm]{cor}
\declaretheorem[style=thmbluebox,name=Theorem,numbered=no]{thm*}
\declaretheorem[style=thmbluebox,name=Lemma,numbered=no]{lemma*}
\declaretheorem[style=thmbluebox,name=Proposition,numbered=no]{prop*}
\declaretheorem[style=thmbluebox,name=Corollary,numbered=no]{cor*}
\declaretheorem[style=thmgreenbox,name=Algorithm]{algo}
\declaretheorem[style=thmgreenbox,name=Algorithm,numbered=no]{algo*}
\declaretheorem[style=thmgreenbox,name=Claim,sibling=thm]{claim}
\declaretheorem[style=thmgreenbox,name=Claim,numbered=no]{claim*}
\declaretheorem[style=thmpinegreenbox,name=Example,sibling=thm]{ex}
\declaretheorem[style=thmpinegreenbox,name=Example,numbered=no]{ex*}
\declaretheorem[style=thmpinegreenbox,name=Example,sibling=thm]{example}
\declaretheorem[style=thmpinegreenbox,name=Example,numbered=no]{example*}
\declaretheorem[style=thmanswerbox,name=Answer,numbered=no]{answer}
\declaretheorem[style=thmblackbox,name=Remark,sibling=thm]{rmk}
\declaretheorem[style=thmblackbox,name=Remark,numbered=no]{rmk*}
\declaretheorem[style=thmblackbox,name=Remark,sibling=thm]{remark}
\declaretheorem[style=thmblackbox,name=Remark,numbered=no]{remark*}
\declaretheorem[style=thmbluebox,name=Proposition,sibling=thm]{proposition}
\declaretheorem[style=thmbluebox,name=Corollary,sibling=thm]{corollary}
\declaretheorem[style=thmpinegreenbox,name=Example,sibling=thm]{exercise}


\theoremstyle{definition}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{definition}[thm]{Definition}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem*{assumption*}{Assumption}
\newtheorem{note}[thm]{Notation}
\newtheorem{defn}[thm]{Definition}
\newtheorem{fact}[thm]{Fact}
%\newtheorem{prop}[prop]{Proposition}
%\newtheorem{answer}[thm]{Answer}
\newtheorem{ques}[thm]{Question}
\newtheorem{exer}[thm]{Exercise}
\newtheorem{prob}[thm]{Problem}
\newtheorem*{conj*}{Conjecture}
\newtheorem*{defn*}{Definition}
\newtheorem*{note*}{Notation}
\newtheorem*{fact*}{Fact}
%\newtheorem*{answer*}{Answer}
\newtheorem*{ques*}{Question}
\newtheorem*{exer*}{Exercise}
\newtheorem*{prob*}{Problem}

% cleveref setup
\Crefname{defn}{Defn.}{Defn.}
\Crefname{definition}{Defn.}{Defn.}
\Crefname{rmk}{Rmk.}{Rmk.}
\Crefname{prop}{Prop.}{Prop.}
\Crefname{thm}{Thm.}{Thm.}
\Crefname{cor}{Cor.}{Cor.}
\Crefname{lem}{Lem.}{Lem.}
\Crefname{lemma}{Lem.}{Lem.}
\Crefname{algo}{Alg.}{Alg.}
\Crefname{ex}{Ex.}{Ex.}
\Crefname{answer}{Answer}{Answers}
\Crefname{ques}{Ques.}{Ques.}
\Crefname{prob}{Prob.}{Prob.}
\Crefname{assumption}{Assumption}{Assumptions}
\Crefname{note}{Notation}{Notations}
\Crefname{fact}{Fact}{Facts}
\Crefname{exer}{Exer.}{Exer.}
\Crefname{conj}{Conj.}{Conj.}
\Crefname{claim}{Claim}{Claims}
\Crefname{subsection}{Subsec.}{Subsec.}
\Crefname{section}{Sec.}{Sec.}
\Crefname{table}{Table}{Tables}
\crefformat{equation}{(#2#1#3)}

% algorithm2e
\usepackage[algo2e, vlined, ruled, linesnumbered]{algorithm2e}
% algorithm2e commenting
%\newcommand{\com}[1]{{\color{red}\textbf{[[} #1 \textbf{]]}}}
%\newcommand\mycommfont[1]{\footnotesize\textcolor{black}{#1}}
\newcommand\mycommfont[1]{\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\usepackage{etoolbox}  % patch def of algorithmic environment
\makeatletter
\patchcmd{\algorithmic}{\addtolength{\ALC@tlm}{\leftmargin} }{\addtolength{\ALC@tlm}{\leftmargin}}{}{}
\makeatother



\newenvironment{protocol}[1][htb]
  {\renewcommand{\algorithmcfname}{Protocol}% Update algorithm name
   \begin{algorithm2e}[#1]%
   }{\end{algorithm2e}}


\newenvironment{exampl}[1][htb]
  {%\refstepcounter{examcounter}\par\medskip
  \renewcommand{\algorithmcfname}{Algorithm}
   \begin{algorithm2e}[#1]%
   }{\end{algorithm2e}}


\newenvironment{procedures}[1][htb]
  {\renewcommand{\algorithmcfname}{Procedure}% Update algorithm name
   \begin{algorithm2e}[#1]%
   }{\end{algorithm2e}}

\def\QED{{\phantom{x}} \hfill \ensuremath{\rule{1.3ex}{1.3ex}}}
\newcommand{\extraproof}[1]{\rm \trivlist

\item[\hskip \labelsep{\bf Proof of #1. }]}
\def\endextraproof{\QED \endtrivlist}

\newenvironment{rtheorem}[3][]{

\bigskip

\noindent \ifthenelse{\equal{#1}{}}{\bf #2 #3}{\bf #2 #3 (#1)}
\begin{it}
}{\end{it}}

\newcommand{\nonl}{\renewcommand{\nl}{\let\nl}}
\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}
\newcommand{\obs}{o}

% enable do while
\SetKwRepeat{Do}{do}{while}


% if you use cleveref..
%\usepackage{nameref}
%\usepackage[capitalize,noabbrev]{cleveref}
\crefname{algocf}{Alg.}{Alg.}
\Crefname{algocfproc}{Alg.}{Alg.}

% fix algorithm2e labelling by cleverref
\crefalias{AlgoLine}{line}%
\makeatletter
\let\cref@old@stepcounter\stepcounter
\def\stepcounter#1{%
  \cref@old@stepcounter{#1}%
  \cref@constructprefix{#1}{\cref@result}%
  \@ifundefined{cref@#1@alias}%
    {\def\@tempa{#1}}%
    {\def\@tempa{\csname cref@#1@alias\endcsname}}%
  \protected@edef\cref@currentlabel{%
    [\@tempa][\arabic{#1}][\cref@result]%
    \csname p@#1\endcsname\csname the#1\endcsname}}
\makeatother

% colors and hypersetup
\definecolor{aqua}{rgb}{0.0, 1.0, 1.0}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{charcoal}{rgb}{0.21, 0.27, 0.31}
\hypersetup{
	%backref=true,
    %pagebackref=true,
    %hyperindex=true,
    colorlinks=true,
    breaklinks=true,
	citecolor=Mulberry,
	filecolor=black,
	linkcolor=azure,
	urlcolor=PineGreen,
	linkbordercolor=blue
}


% table of contents spacing
\usepackage{tocloft}
\setlength{\cftbeforesecskip}{5pt}

% redefine title command
\makeatletter
\def\@maketitle{%
  \begin{center}%
  { \begin{tcolorbox}[colframe=caribbeangreen,colback=caribbeangreen!10]
		  \LARGE\bf\centering\@title \color{charcoal}
\end{tcolorbox}
}%
  \end{center}%
  }
\makeatother

\endinput


==> lemmas.tex <==
\section{Auxilliary Lemmas}

%\begin{lemma}[Tail Bound for Uniform Sample Order Statistics]\label{lem:gaps}
	%Let $X_1,\ldots,X_n$ be an i.i.d. sample from a $\Unifu$ distribution.
	%Let $X_{(1)} \leq \cdots \leq X_{(n)}$ be the corresponding order statistics.
	%Then, we have for any natural number $n \geq 3$:
	%\begin{align*}
		%\mb{P}\left( \exists i \in [n], i \geq 3 : \frac{1}{X_{(i)}} \geq z_{n,i} \right) &\leq \frac{1}{n^2},
	%\end{align*}
	%where
	%\[
		%z_{n,i} := 1 \vee \frac{n^{\frac{2}{i-2}}}{(i-1)^{\frac{n-i+2}{i-2}}}.
	%\]
	%%We also have:
	%%\[
		%%\mb{P}\left( \min\left\{ \frac{C\log(n)}{X_{(2)}} , n^2 \cdot X_{(2)} \right\} \geq n \right) \leq \frac{1}{n}.
	%%\]
%\end{lemma}
%
%\begin{proof}
	%%Fix $i \geq 3$.
	%First, we recall a standard fact about the order statistics of an i.i.d. sample.
	%Suppose $X_{(1)},\ldots,X_{(n)}$ are the order statistics of an i.i.d. sample $X_1,\ldots,X_n$ from a distribution supported on $[0,1]$ with density $g$ and cdf $G$.
	%Then, we have \citep[Lemma D.4]{bayati20} that $X_{(i)}$ for $i\geq 2$ has density
	%\[
		%g_{X_{(i)}}(u) = n (n-1) \binom{n-2}{i-2} \int_0^{1-u} (G(u+z) - G(z))^{i-2} \cdot g(u+z) \cdot g(z) \cdot G(z)^{k-i} \,dz.
	%\]
	%Thus, now we write:
	%\begin{align*}
		%\mb{P}\left( \frac{1}{X_{(i)}} \geq z_{n,i} \right) &= \mb{P}\left( X_{(i)} \leq \frac{1}{z_{n,i}} \right)\\
								    %&= \int_0^{z_{n,i}^{-1}} n \cdot (n-1) \cdot \binom{n-2}{i-2} \int_0^{1-u} u^{i-2} \cdot z^{n-i} \,dz \,du\\
								    %&=  \int_0^{z_{n,i}^{-1}} n \cdot (n-1) \cdot \binom{n-2}{i-2} \cdot u^{i-2} \cdot \frac{(1-u)^{n-i+1}}{n-i+1} \,du \\
								    %&= \frac{n (n-1)}{n-i+1} \cdot \binom{n-2}{i-2} \cdot \frac{\Gamma(i-1) \cdot \Gamma(n-i+2)}{\Gamma(n+1)} \cdot I_{z_{n,i}^{-1}}(i-1,n-i+2) \\
								    %&= \frac{n (n-1) \cdot (n-2)! \cdot (i-2)! \cdot (n-i+1)!}{(n-i+1) \cdot (i-2)! \cdot (n - i)! \cdot n!} \cdot I_{z_{n,i}^{-1}}(i-1,n-i+2) \\
								    %&= I_{z_{n,i}^{-1}}(i-1,n-i+2),
	%\end{align*}
%where we plug in the cdf of a beta distribution and then the regularized incomplete beta function $I_x(\alpha,\beta)$ at the third and fourth steps.
%
	%We use the well-known relationship between beta and binomial distribution cdf's, to get:
	%\begin{align*}
		%I_{z_{n,i}^{-1}}(i-1,n-i+2) &= \mb{P}\left( \Bin\left( n, z_{n,i}^{-1} \right) \leq n - i + 1 \right) \\
					    %&\leq \mb{P}( n\cdot z_{n,i}^{-1} - \Bin(n,z_{n,i}^{-1}) > n \cdot z_{n,i}^{-1} - ( n - i + 1) ).
	%\end{align*}
	%Now, if we can choose $z_{n,i}$ such that
	%\[
		%n \cdot z_{n,i}^{-1} - (n-i+1) \gtrsim n^{1/2} \log^2(n),
	%\]
	%then by Hoeffding's inequality we will have the tail probability is bounded above by
	%\[
		%\exp\left( - \frac{2 (n-i+1 - n \cdot z_{n,i}^{-1})^2}{n} \right) \leq \frac{1}{n^3}.
	%\]
	%Rearranging the previous inequality, we see that we require \com{the below only works for $i > n^{1/2}\log^2(n)$ as we need $z_{n,i}^{-1}$ to be less than $1$}
	%\[
		%z_{n,i}^{-1} \gtrsim \frac{n-i+1 + n^{1/2} \log^2(n)}{n}.
	%\]
	%Can we safely set $z_{n,i}$ like this?
	%Well, let's sum over $i$:
	%\[
		%\sum_{i=3}^n z_{n,i} = \sum_{i=3}^n \frac{1}{\frac{n-i+1}{n} + \log^2(n)/\sqrt{n}} = \sum_{i=3}^{n-\sqrt{n}} \frac{n}{n-i+1} + \sum_{i=n-\sqrt{n}}^n \frac{\sqrt{n}}{\log^2(n)}.
	%\]
	%Both sums on the RHS are order $n$ which is what we want.
%
%
	%%Next, note that, using Stirling approximation, for $i < n - \ceil{\log(n)}$:
	%%\begin{align*}
		%%\frac{1}{(n-i)!} &\leq \frac{1}{(\ceil{\log(n)})!} \\
				 %%&\leq \frac{1}{\sqrt{2 \pi \log(n)} \cdot (\log(n)/e)^{\log(n)} \cdot e^{\frac{1}{12 \ceil{\log(n)}} - \frac{1}{360\ceil{\log^3(n)}}} }
	%%\end{align*}
	%%Next, we observe the bound
	%%\[
		%%\left( \frac{\log(n)}{e} \right)^{\log(n)} = \frac{n^{\log(n)\cdot \log(\log(n))}}{n} = n^{\log(n)\cdot \log(\log(n)) - 1}.
	%%\]
	%%For $n > 10$, we have $\log(n) \cdot \log(\log(n)) - 1 > 1$ so that $\frac{1}{(\log(n))!} < 1/n$.
%
	%\com{
	%Thus, it suffices to bound this last beta distribution cdf.
	%%We use a bound on the regularized incomplete beta function $I_x(\alpha,\beta)$ scaling like
	%We start by expressing the regularized incomplete beta function $I_x(\alpha,\beta)$ as a ratio of the incomplete beta function and the (ordinary) beta function
	%\[
		%I_x(\alpha,\beta) = \frac{ \int_0^x u^{\alpha-1} (1-u)^{\beta-1} \,du }{ \frac{\Gamma(\alpha)\cdot \Gamma(\beta)}{\Gamma(\alpha+\beta)}},
	%\]
	%%and then using the bounds of Theorem 5 of \citet{cerone07}.
	%Specifically, let
	%\begin{align*}
		%B(\alpha,\beta,x) &= \int_0^x u^{\alpha-1} (1-u)^{\beta-1}\,du \\
		%B(\alpha,\beta) &= B(\alpha,\beta,1) = \frac{\Gamma(\alpha) \cdot \Gamma(\beta)}{\Gamma(\alpha+\beta)}.
	%\end{align*}
	%Then, we have by Theorem 5 of \citet{cerone07}:
	%\begin{align*}
		%B(\alpha,\beta,x) &\leq \frac{x^{\alpha-1}}{\beta} \left( 1 - \left( 1 - \frac{x}{\alpha} \right)^{\beta} \right) \\
		%B(\alpha,\beta) &\geq \frac{1}{\beta \cdot \alpha^{\beta}}.
	%\end{align*}
	%Putting the above two bounds together, we have
	%\[
		%I_x(\alpha,\beta) \leq x^{\alpha-1} \cdot \alpha^{\beta} \left( 1 - \left( 1 - \frac{x}{\alpha}\right)^{\beta} \right).
	%\]
	%Thus, it remains to show
	%\[
		%(z_{n,i}^{-1})^{i-2} \cdot (i-1)^{n-i+2} \cdot \left( 1 - (1 - z_{n,i}^{-1} / (i-1) )^{n-i+2}  \right) \leq \frac{1}{n^2}.
	%\]
	%\com{actually the above shows we need $z_{n,i}^{-1} = (i-1)^{ - \frac{n-i+2}{i-2}} n^{ - \frac{2}{i-2}}$}
	%This inequality is clearly satisfied for our choice of $z_{n,i}$ by virtue of $z_{n,i}^{-1} \in [0,1]$ so that
	%\[
		%z_{n,i}^{-1} \left( 1 - \left( 1 - \frac{z_{n,i}^{-1}}{i-1} \right)^{n-i+2}\right)^{\frac{1}{i-2}} \leq \frac{(i-1)^{\frac{n-i+2}{i-2}}}{n^{\frac{2}{i-2}}}.
	%\]
	%%For the inequality for $i=2$, we have by virtue of $X_{(2)}$ having a continuous distribution that:
	%%\begin{align*}
		%%\mb{P}\left( \frac{C\log(n)}{X_{(2)}} \land n^2 \cdot X_{(2)} \geq n \right) &= \mb{P}\left( \frac{C\log(n)}{n} \geq X_{(2)} \geq \frac{C^{1/2} \log^{1/2}(n)}{n} \text{ or } \frac{C^{1/2} \log^{1/2}(n)}{n} \geq X_{(2)} \geq \frac{1}{n} \right) \\
											     %%&= \int_{1/n}^{C\log(n)/n} n \cdot (n-1) \int_0^{1-u} z^{n-2} \,dz \,du \\
											     %%&\propto \left( 1 - \frac{1}{n} \right)^n - \left( 1 - \frac{C\log(n)}{n} \right)^n \\
											     %%&\approx e^{-1} - e^{-C\log(n)}
	%%\end{align*}
%}
%\end{proof}
%
%\begin{lemma}\label{lem:sum-inverse}
	%For any natural number $n \geq 8$, we have $\sum_{i=3}^n \frac{n^{\frac{2}{i-2}}}{(i-1)^{\frac{n-i+2}{i-2}}} \leq n\log(n)$.
%\end{lemma}
%
%\begin{proof}
	%%Let's try setting
	%%\[
		%%z_{n,i}^{-1} := \frac{(i-1)^{\frac{n-i+2}{i-2}}}{n^{\frac{2}{i-2}}} \land 1.
	%%\]
	%%This clearly satisfies the previous inequality.
	%%On the other hand, we claim this formula for $z_{n,i}$ is of the right order since when summed over $i$.
	%%We have:
	%%\[
		%%\sum_{i=2}^n z_{n,i} = \sum_{i=2}^n \frac{n^{\frac{2}{i-2}}}{(i-1)^{\frac{n-i+2}{i-2}}}.
	%%\]
	%We split the sum into two parts.
	%First, for $i \leq \frac{n+4}{2}$, we have $\frac{n-i+2}{i-2} \geq 1$ so that that we can bound the first sum over such $i$'s by
	%\[
		%\sum_{i=3}^{\frac{n+4}{2}} \frac{n}{i-1} \leq n\log(n).
	%\]
	%The sum over $i=\frac{n+4}{2}$ to $i=n$ is
	%\[
		%\sum_{i=\frac{n+4}{2}}^n \frac{n}{i-1} \leq \sum_{i=\frac{n+4}{2}}^n \frac{n^{\frac{2}{(n+4)/2-2}}}{(i-1)^{1/2}},
	%\]
	%where we use the fact that $\frac{n-i+2}{i-2} \geq \frac{n/2}{n-2} \geq 1/2$ for $i\geq \frac{n+4}{2}$.
	%By an integral approximation, the above sum is at most order $n^{4/n+1/2}$ which is at most $n$ for $n \geq 8$.
%
	%%%For $i \geq n - \ceil{\log(n)}$, we %now bound
%%%	\[
%%%		\mb{P}\left( \frac{1}{X_{(i)}} \geq \frac{n}{i-2} \right) \leq I_{\frac{i-2}{n}}( i-1, n-i+2).
%%%	\]
	%\com{
	%We use the well-known relationship between beta and binomial distribution cdf's, to get:
	%\begin{align*}
		%I_{z_{n,i}^{-1}}(i-1,n-i+2) &= \mb{P}\left( \Bin\left( n, z_{n,i}^{-1} \right) \leq n - i + 1 \right) \\
					    %&\leq \exp\left( - \frac{2 (n-i+1 - n \cdot z_{n,i}^{-1})^2}{n} \right),
						    %%&\leq  \mb{P}\left( \Bin\left( n, z_{n,i}^{-1} \right) \leq \ceil{\log(n)} + 1 \right)
	%\end{align*}
	%where the second step is by Hoeffding's inequality.
	%Now, the above RHS is less than $1/n^3$ so long as
	%\[
		%|n-i+1 - n \cdot z_{n,i}^{-1} | \gtrsim n^{1/2} \log^2(n).
	%\]
	%%Let $z_{n,i}^{-1} = \frac{i-1}{n} \land \frac{3}{4}$.
	%Then, for $i < \frac{n}{4} + 1$, we have $z_{n,i}^{-1} = \frac{i-1}{n}$ and
	%\[
		%| n - i + 1 - n \cdot z_{n,i}^{-1}| \geq n - 2i +2  \geq \frac{n}{2} \gtrsim n^{1/2} \log^2(n),
	%\]
	%for large enough $n$.
	%For $i \geq \frac{n}{4} + 1$, we have:
	%\[
		%|n - i + 1 - n \cdot z_{n,i}^{-1} | \geq n \cdot z_{n,i}^{-1} - n + i - 1 \geq \frac{n}{4} \gtrsim n^{1/2} \log^2(n),
	%\]
	%again for large enough $n$.
	%\com{application of hoeffding doesn't make sense for $i=2$.
	%Intuitvely, $\Bin(n,1/2) \approx n/2$ so we should have $\mb{P}(\Bin(n,1/2) \leq n-1)$ should be very large, not small.
%
	%The problem is that the parameter $t$ in the typical Hoeffding ineq (see wikipedia) is not positive here.
%}
%}
%%
	%%%For $i=2$, we run the same argument with $z_{n,i}^{-1} = 2$.
	%%%\com{why do we have to use $2$ for $i=2$, kinda weird.
	%%%Also consider \href{https://math.stackexchange.com/questions/1290246/estimates-for-the-normal-approximation-of-the-binomial-distribution}{Berry-Eseen bound} instead of using Hoeffding.
	%%%}
%\end{proof}


==> scrap/beta.tex <==
\section{Extension to $\beta$-Regular Reservoir Distributions}\label{app:beta}

We consider a non-stationary infinite-armed bandit problem where every time an arm is sampled for the first time, its initial reward value is drawn i.i.d. from a distribution with $\mb{P}(\mu_0(a) > 1 - x) = \Theta(x^{\beta})$.
%Specifically, suppose there exist $c_0,C_0$ such that for all $x \in [0,1]$:
%\[
	%c_0 x^{\beta} \leq \mb{P}(\mu_0(a) > 1 - x) \leq C_0 x^{\beta}.
%\]
Thereafterwards, the reward changes according to an adaptive adversary.

Let's suppose the agent knows $\beta$ and that it's fixed across time.

\begin{rmk}
	We do not require conditions on the density of $\mu_0(a)$ as does \citet{bayati20} p. 18, and so our results are more general than theirs even in the stationary setting.
	In particular, they require a bounded density for $\beta > 1$ and a more restrictive condition that that the density of $\mu_0(\cdot)$ at $x\in [0,1]$ is $O((1-x)^{\beta-1})$ for $\beta<1$.
	Interestingly, the results of \citet{kim24} for general $\beta$ also do not require such density conditions either.
\end{rmk}

Considering the lower bounds of \citet{kim24}, we aim to get a regret upper bound of
\[
	(V^{\frac{1}{\beta+2}} T^{\frac{\beta+1}{\beta+2}} + T^{\frac{\beta}{\beta+1}}) \land ( (L+1)^{\frac{1}{\beta+1}} \cdot T^{\frac{\beta}{\beta+1}}).
\]
Previously, they only obtain this bound for $\beta>1$ and while requiring parameter knowledge of $V$ and $L$.
For $\beta<1$, it was not even known how to get the bound for the stationary setting $L=V=0$. \jk{You may already know that \cite{wang08} obtain tight results when $\mu^*=1$ for all $\beta$ considering the variance term. I guess \cite{bayati20} considers 1-sub gaussian noise distribution which is the main reason why they have $\sqrt{T}$ for $\beta<1$.}
\joe{Thanks, I didn't notice they already obtain the correct upper bound when $\mu^*=1$.
	Now, I see that $\mu^* = 1$ is quite critical to my result.
	Suppose we have bounded rewards $Y_t(a) \in [0,1]$, but $\mu^* < 1$.
	Then, it could be the case that the variance of $Y_t(a)$ is large enough so that $Y_t(a) > \mu^*$ with constant probability even though the mean $\mu_t(a) \leq \mu^*$.
	This means the variance of the estimator
	\[
		\Var( \mu^* - Y_t(a)) \leq \mb{E}[ (\mu^* - Y_t(a))^2 ] \leq \mb{E}[ | \mu^* - Y_t(a)| ].
	\]
	Unfortunately, the above RHS is only an {\bf absolute} first moment and not the first moment $\mb{E}[\mu^*-Y_t(a)] = \delta_t(a)$.
	The absolute first moment can be large $\Omega(1)$ while $\delta_t(a)$ is small.
	This means my variance-based/self-bounding tricks will not work if $\mu^* < 1$ but $Y_t(a) \in [0,1]$ can have large variance.
	Note that if we assume $Y_t(a) \in [0,\mu^*]$ a.s. then the issue is completely resolved and the absolute first moment becomes just the usual first moment.

	\citet{bayati20} use $\mu^*=1$ and $Y(a) \in [0,1]$, so I don't understand why they cannot get $T^{\frac{\beta}{\beta+1}}$ for $\beta<1$ like \citet{wang08} can. 
}\jk{As you mentioned via email, \citet{bayati20} may assume sub-guasisan distribution including gaussian distribution rather than bounded $[0,1]$.}

We give a complete parameter-free result for all values of $\beta$.

To start, we first generalize the notion of significant shift (\Cref{defn:sig-shift}) for the case of general $\beta$.

\begin{defn}[Significant Shift]\label{defn:sig-shift-beta}
	Let $\tau_0 := 1$.
	Define $\tau_{i+1}$ given $\tau_i$ in the following recursive way:
	let $\tau_{i+1}$ be the smallest round $t > \tau_i$ such that there is a set $\hat{\mc{A}}$ of arms of size at least $(t - \tau_i)^{\frac{\beta}{\beta+1}}$ sampled by the agent since round $\tau_i$ such that: each $a\in \hat{\mc{A}}$ incurs significant regret in the sense of $\exists [s_1,s_2] \subseteq [\tau_i,t]$ such that:
	\begin{equation}\label{eq:sig-regret-beta}
		(s_2 - s_1 + 1)^{\frac{\beta}{\beta+1}} \leq \sum_{s=s_1}^{s_2} \delta_s(a).
	\end{equation}
	Let $\Lsig$ be the latest significant shift over $T$ rounds and by convention let $\tau_{\Lsig+1} := T+1$.

	We say a bandit environment over $T$ rounds is {\bf safe} if there exists an arm $a$ among the first $T^{\frac{\beta}{\beta+1}}$ arms sampled by the agent such that $\sum_{s \in I} \delta_s(a) \leq |I|^{\frac{\beta}{\beta+1}}$ for all intervals of rounds $I \subseteq [T]$, i.e. if no significant shift occurs over $T$ rounds.
\end{defn}

Note the key difference with \Cref{defn:sig-shift} for the case of $\beta=1$ is the different choice of number of subsampled arms and regret threshold, which are both chosen to match the stationary minimax regret rate of $T^{\frac{\beta}{\beta+1}}$ for this setting.

\bld{Algorithm:} our procedure will actually be the same restarting elimination as \Cref{alg:elim} with the only change being the number of subsampled arms on \Cref{line:subsample} of \Cref{alg:elim}.
Here, we'll subsample $\ceil{ 2^{(m+1) \cdot \frac{\beta}{\beta+1}}}$ in each block of length $2^m$.

Then, analogous to \Cref{thm:blackbox}, we aim to show a cumulative regret bound of $\sum_{\ell} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}}$.
Then, a $((\Lsig +1)^{\frac{1}{\beta+1}}\cdot T^{\frac{\beta}{\beta+1}} \land (V^{\frac{1}{\beta+2}} T^{\frac{\beta+1}{\beta+2}} + T^{\frac{\beta}{\beta+1}})$ will follow using analogous arguments as \Cref{cor:elim-bounds} (namely, applying Jensen and H\"{o}lder to the respective regret rate functions).

%This can be, for example, attained by getting a ``summed over phases or episodes'' bound of $\sum_{\ell} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}}$ using Jensen and Holder so long as each phase $\ho{t_{\ell}}{t_{\ell+1}}$ has variation at least $(t_{\ell+1} - t_{\ell})^{- \frac{1}{\beta+1}}$.
%
%%For the proof, our blackbox algorithm needs to have a $t$-round guarantee of:
%%\[
	%%\sum_{s=1}^t \max_{a' \in \mc{A}_0} \mu_s(a) - \mu_s(a_s) \leq C_0 \left( \sum_{i=2}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1}\left\{ \Delta_{(i)} \geq \frac{|\mc{A}_0|}{t} \right\} + |\mc{A}_0| \right).
%%\]
%%Then, the regret upper bound proof follows the same steps except we need to calculate the mean of the variable $N_j$ as:
%%\begin{align*}
	%%|\mc{A}_0| \cdot \mb{P}( \mu_0(a) \in [2^{-(j+1)} , 2^{-j} ) ) &\geq |\mc{A}_0| \cdot (C_0 (1-2^{-(j+1)})^{\beta} - c_0 (1-2^{-j})^{\beta} ) \\
								       %%&\geq c_0 |\mc{A}_0| \cdot ( (1-2^{-(j+1)}) -  (1 - 2^{-j})) \\
								       %%&\geq c_0 |\mc{A}_0| \cdot 2^{-(j+1)},
%%\end{align*}
%%where we use in the second inequality the fact that $C_0 > c_0$, the elementary inequality $(1-x)^{\beta} \geq 1 - x$ for $\beta>1$ and $x \in [0,1]$, and the fact that $\beta>1$.
%%
%%On the other hand,
%%\[
	%%\mb{P}(\mu_0(a) \in [2^{-(j+1)},2^{-j}))
%%\]
%
%For significant shifts, we also have a phenomenon similar to \Cref{prop:adaptive-lower} for $\beta=1$.
%Any algorithm which maintains $T^{\frac{\beta}{\beta+1}}$ regret in stationary environments will have to sample at least $K = \Omega(T^{\frac{\beta}{\beta+1}})$ arms (to ensure we have an arm with regret $o(T^{-\frac{1}{\beta+1}})$). Thus, an adversary can force $\sqrt{KT} = T^{\frac{\beta+1/2}{\beta+1}}$ regret in a safe environment (as measured by regret threshold of $T^{\frac{\beta}{\beta+1}}$).
%This suggests the minimax regret rate in terms of $\Lsig$ significant shifts should be $T^{\frac{\beta+1/2}{\beta+1}} \cdot (\Lsig + 1)^{\frac{1/2}{\beta+1}}$.

\begin{thm}{(Regret Upper Bound for \Cref{alg:elim})}
	\Cref{alg:elim} using subsampling of $\ceil{ 2^{(m+2) \cdot \frac{\beta}{\beta+1}} }$ arms in the $m$-th block achieves a regret bound of, with probability at least $1 - 1/T$:
	\[
		\bld{R}_T \lesssim \sum_{\ell=1}^{\hat{L}} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}} \leq ((\Lsig +1)^{\frac{1}{\beta+1}}\cdot T^{\frac{\beta}{\beta+1}} ) \land (V^{\frac{1}{\beta+2}} T^{\frac{\beta+1}{\beta+2}} + T^{\frac{\beta}{\beta+1}}).
	\]
\end{thm}

\begin{proof}{(Sketch)}
	The proof follows the exact same steps as the proof of \Cref{thm:regret-episodes} except we upper bound $|\mc{A}_m|$ by $(t_{\ell}^{m+1} - t_{\ell}^m)^{\frac{\beta}{\beta+1}}$ at the last step and use the key fact that $T^{\frac{\beta}{\beta+1}}$ arms is sufficient to secure an arm with initial gap $O(T^{-\frac{1}{\beta+1}})$, which is enough to show the total variation over episode $\ho{t_{\ell}}{t_{\ell+1}}$ concluding in a restart is at least
	\[
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{1}{(t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}}}.
	\]
\end{proof}

\begin{rmk}
	We note it's quite crucial here that the the top reward value $\mu^*$ is exactly $1$.
	If we'd instead worked in the setting where the top reward value $\mu^* < 1$, then a rate of $T^{\frac{\beta}{\beta+1}}$ is conjectured to be impossible for $\beta<1$ due to the lower bound on simple regret established in Theorem 1 of \citet{carpentier15}.
	This phenomenon is also observed in the rates (Theorem 2) of \citet{wang08}, which differ for $\beta < 1$ depending on whether $\mu^* < 1$ or $\mu^* = 1$.
\end{rmk}

\com{can we get a suboptimal bound for unknown $\beta$ by plugging in the wrong value of $\beta$?}

%\begin{proof}{(Sketch)}
	%\Cref{thm:regret-episodes} remains true without modification.
	%Then, further upper bounding $\sqrt{\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mc{G}_t| }$ mostly follows the same proof with some key modifications to the relevant intermediate mathematical variables arising within the proof of \Cref{cor:elim-bounds}.
%
	%The $T^{\frac{\beta+1/2}{\beta+1}} \cdot (\Lsig +1)^{\frac{1/2}{\beta+1}}$ bound follows immediately from the way we set the arm sizes since
	%\[
		%\sqrt{\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mc{G}_t| } \leq \sqrt{ (t_{\ell+1} - t_{\ell})^{1 + \frac{\beta}{\beta+1}} } = (t_{\ell+1} - t_{\ell})^{\frac{\beta+1/2}{\beta+1}}.
	%\]
	%We next outline how to get the bound in terms of $L$ and $V$.
	%Using the notation of the proof of \Cref{cor:elim-bounds}, the following modifications are required:
	%\begin{itemize}
		%\item let $t \in \ho{t_{\ell}^m+K}{t_{\ell}^{m+1}}$ be the first round such that $|\mc{G}_t| > c_0 \log(T) \cdot 2^{m \cdot \frac{\beta}{\beta+1}} \cdot (t - t_{\ell}^m + 1)^{-\frac{1}{\beta+1}}$.
		%\item let $\Delta = c_1 \log(T) \cdot (t - t_{\ell}^m + 1)^{-\frac{1}{1+\beta}}$.
		%\item Our multiplicative Chernoff bound tells us with high probability that $N(\Delta) < 2 K \Delta^{\beta}$ (importantly, this makes use of the fact that $\mb{P}( 1 - \mu_0(a) < \Delta) = \mb{P}( \mu_0(a) > 1 - \Delta) = \Theta(\Delta^{\beta})$).
		%\item Thus, we can conclude using the same arguments as the proof of \Cref{cor:elim-bounds} that the variation within a block which concludes with a restart is at least $|\mc{G}_t|\cdot \Delta \gtrsim 2^{m \cdot \frac{\beta}{\beta+1}} \cdot (t - t_{\ell}^m + 1)^{-\frac{1}{\beta+1}}$.
		%\item Then, we can use H\"{o}lder's inequality to bound
		%\[
			%\sum_{\ell,m} (2^m)^{3/4} \cdot (\tilde{t}_{\ell,m} - t_{\ell}^m)^{-1/4} \leq \left( \sum_{\ell,m} 2^{\frac{m}{1+\beta}} \cdot (\tilde{t}_{\ell,m} - t_{\ell}^m + 1)^{-\frac{2}{1+\beta}} \right)^{\frac{1}{\beta+2}} \cdot \left( \sum_{\ell,m} 2^m \right)^{\frac{\beta+1}{\beta+2}} \leq V^{\frac{1}{\beta+2}} \cdot T^{\frac{\beta+1}{\beta+2}}.
		%\]
		%\item In particular, the reason we get the $2^m$ term inside the second parentheses on the RHS above is because of the elementary result that
			%\[
				%\forall \beta \geq -1/2:	\left( \left( \frac{3\beta}{4 (1+\beta)} - \frac{1}{(\beta+1)(2+\beta)} \right) + \left( - \frac{1}{4} + \frac{2}{(1+\beta) (2+\beta)} \right) \right) \cdot \left(\frac{\beta+2}{\beta+1} \right) \leq 1.
			%\]
	%\end{itemize}
%
%\end{proof}
%
%\com{
	%I think the blackbox procedure \Cref{alg:blackbox} can also attain the regret bound in terms of $L$ and $V$ when using subsampling with $K = T^{\frac{\beta}{\beta+1}}$ arms and tracking the dynamic regret at $T^{\frac{\beta}{\beta+1}} > \sqrt{T}$ rates.
	%Meanwhile, any reasonable finite-armed stochastic bandit algorithm will get high-prob logarithmic regret bound in environments with variation at most $T^{-\frac{1}{\beta+1}} < T^{-\frac{1/2}{\beta+1}} = \sqrt{K/T}$ where $K = T^{\frac{\beta}{\beta+1}}$ is the number of subsampled arms here.
%
	%The key substitution in the proof has to come in when bounding mass of the initially sampled gaps
	%\[
		%\mb{P}( \mu_0(a) \in \ho{2^{-(j+1)}}{2^{-j}}).
	%\]
	%However, it's unclear how to bound this using the definition of $\beta$-regular distribution without making further assumptions on the distribution
%}
%
%\com{why doesn't the above proof also work for $\beta<1$?
%I think this is because $\sqrt{\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mc{G}_t|}$ must always be at least $\sqrt{t_{\ell+1} - t_{\ell}}$ and so we can't surpass this rate}
%


%\subsection{$\beta \in (0,1)$}
%
%For $\beta<1$, even in the stationary setting, \citet{bayati20} can only get a regret bound of $\sqrt{T}$ which might be suboptimal.
%Their algorithm for this setting involves subsampling $K = T^{\beta/2}$ arms and then bounding the regret by $K + K^{1/\beta} + K \cdot T^{\frac{1-\beta}{2}}$.
%
%Likewise, in the rotting bandit setup, the best known bounds are still $\sqrt{LT} \land V^{1/3} T^{2/3}$, same as in the $\beta=1$ case \citep{kim24}.
%
%Now, the sig shift lower bound is a bit more nuanced.
%The discussion on p. 46 of \citet{bayati20} suggests we only need to subsample $K=T^{\beta/2}$ arms to secure an arm with gap $O(1/\sqrt{T})$.
%This means the adversary can only force $\sqrt{KT} = T^{1/2+\beta/4}$ regret which is a smaller rate than that forced by the adversary for $\beta>1$, but still larger than the ``expected'' stationary rate of $T^{1/2}$.
%This suggests the minimax regret rate in terms of $\Lsig$ significant shifts should be $T^{1/2+\beta/4} \cdot (\Lsig + 1)^{1/2 - \beta/4}$.
%
%\begin{thm}{(Regret Upper Bound for \Cref{alg:elim})}\label{thm:upper-beta-small}
	%\Cref{alg:elim} using subsampling of $\ceil{ 2^{(m+2) \cdot \frac{\beta}{2}} }$ arms in the $m$-th block achieves a regret bound of, with probability at least $1 - 1/T$:
	%\[
		%\bld{R}_T \leq \tilde{O}\left( \min\left\{ T^{1/2+\beta/4} \cdot (\Lsig+1)^{1/2-\beta/4}, \sqrt{(L + 1) \cdot T}, V^{1/3} T^{2/3} + T^{1/2} \right\} \right).
	%\]
%\end{thm}
%
%\begin{proof}{(Sketch)}
	%\Cref{thm:regret-episodes} remains true without modification.
	%Then, further upper bounding $\sqrt{\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mc{G}_t| }$ mostly follows the same proof with some key modifications to the relevant intermediate mathematical variables arising within the proof of \Cref{cor:elim-bounds}.
%
	%The bound in terms of significant shifts is immediate from noticing that subsampling $K = T^{\beta/2}$ arms leads to a worst-case regret of $\sqrt{KT} = T^{1/2+\beta/4}$ over $T$ rounds and then using Jensen's inequality.
%
	%Using the notation of the proof of \Cref{cor:elim-bounds}, the following modifications are required:
	%\begin{itemize}
		%\item let $t \in \ho{t_{\ell}^m+K}{t_{\ell}^{m+1}}$ be the first round such that $|\mc{G}_t| > c_0 \log(T) \cdot 2^{m \cdot \frac{\beta}{2}} \cdot (t - t_{\ell}^m + 1)^{-\beta/2}$.
		%\item let $\Delta = c_1 \log(T) \cdot (t - t_{\ell}^m + 1)^{-\frac{1}{2}}$.
		%\item Our multiplicative Chernoff bound tells us with high probability that $N(\Delta) < 2 K \Delta^{\beta}$ (importantly, this makes use of the fact that $\mb{P}( 1 - \mu_0(a) < \Delta) = \mb{P}( \mu_0(a) > 1 - \Delta) = \Theta(\Delta^{\beta})$).
		%\item Thus, we can conclude using the same arguments as the proof of \Cref{cor:elim-bounds} that the variation within a block which concludes with a restart is at least $|\mc{G}_t|\cdot \Delta \gtrsim 2^{m \cdot \frac{\beta}{2}} \cdot (t - t_{\ell}^m + 1)^{-\frac{1}{2}}$.
		%\item Then, we can use H\"{o}lder's inequality to bound
		%\[
			%\sum_{\ell,m} (2^m)^{1/2 + \beta/4} \cdot (\tilde{t}_{\ell,m} - t_{\ell}^m)^{-\beta /4} \leq \left( \sum_{\ell,m} 2^{m \beta/2 } \cdot (\tilde{t}_{\ell,m} - t_{\ell}^m + 1)^{ - \frac{1+\beta}{2}} \right)^{1/3}  \left( \sum_{\ell,m} 2^m \right)^{2/3} \leq V^{1/3} T^{2/3}.
		%\]
	%\end{itemize}
%\end{proof}


%In this case, we need a base algorithm which can get the logarithmic regret bound in environments with variation at most $T^{-1/2} < T^{\beta/4 - 1/2} = \sqrt{K/T}$.
%Then, we can get $\sum_{\ell} d_{\ell}^{1/2}$ regret w.r.t. small-variation phases.


==> scrap/blackbox.tex <==
\section{A Blackbox for Optimally Tracking Unknown Non-Stationarity}\label{sec:blackbox}

A key idea, introduced for the stationary problem in \citet{bayati20}, is that of {\em subsampling} a finite number of arms from the reservoir.
The main algorithmic design principle is to then run a finite-armed MAB algorithm over the subsampled arms.
The choice of number of arms to subsample is key here and exhibits its own exploration-exploitation tradeoff.
This tradeoff is best exemplified through the natural regret decomposition with respect to the subsampled set of arms, which we'll denote by $\mc{A}_0 \subseteq \mc{A}$:
%For minimizing regret over $T$ rounds, the minimax optimal regret of $\sqrt{T}$ can be achieved by subsampling $\sqrt{T}$ arms.

%In particular, within a sample of $\sqrt{T}$ arms, with high probability at least one arm will have reward at least $1-1/\sqrt{T}$.
%Then, it turns out one can reduce the problem to finite-armed bandits by subsampling $\sqrt{T}$ arms and then bounding regret between the subsampled arms:
%Thentural regret decomposition induced by a subsampled set of arms $\mc{A}_0$:
\begin{equation}\label{eq:regret-decomp}
	\sum_{t=1}^T \delta(a_t) = \underbrace{ \sum_{t=1}^T  1 - \max_{a \in \mc{A}_0} \mu(a)}_{\text{Regret of best subsampled arm}}  + \underbrace{ \sum_{t=1}^T  \max_{a \in \mc{A}_0} \mu(a) - \mu(a_t)}_{\text{Regret of played arms to best subsampled arm}}.
\end{equation}
Let's suppose there are $K := |\mc{A}_0|$ subsampled arms.
Then, a sample of $K$ arms drawn from $\Unifu$ contains, with high probability, an arm with reward at least $1-1/K$ and, thus, gap at most $1/K$.
Thus, the first sum in \Cref{eq:regret-decomp} is at most $T/K$.

Then, plugging in the classical gap-dependent regret bounds for finite-armed MAB, the second term in \Cref{eq:regret-decomp} is $\tilde{O}\left( \sum_{a \in \mc{A}_0 \bs \argmax_{a' \in \mc{A}_0} \mu(a')} \Delta_{a}^{-1} \right)$ where $\Delta_{a}$ is the (random) gap of $a$ to the best subsampled arm.
Then, it is further shown \citep[Section A.2]{bayati20} that this gap-dependent quantity scales like $K\log(T)$ in expectation.

Then, we may choose $K$ to balance the bounds $T/K$ and $K \cdot \log(T)$ for which $K \propto \sqrt{T}$ is optimal giving a regret bound of $\sqrt{T}$.
As it turns out, the $\sqrt{T}$ regret rate is minimax.

Extending this to the non-stationary problem, it is first natural to ask whether we can follow the same strategy using a reduction to finite-armed non-stationary bandits.
However, this strategy poses two key difficulties:
\begin{enumerate}[(a)]
	\item Firstly, it's quite crucial in the above argument that the logarithmic gap-dependent regret bound was plugged in and not the gap-independent worst-case bound of $\sqrt{K T}$ (which would only lead to a suboptimal $T^{2/3}$ bound when optimizing $K$).

	As our goal in the non-stationary problem is to achieve {\em adaptive} regret bounds, free of parameter knowledge, a natural proposal is to reduce to $K$-armed non-stationary bandits and employ the known adaptive algorithms for this setting \citep{auer2019,wei2021,suk22,abbasi22}.
	However, it's long been known in this literature that no algorithm can adaptively secure a gap-dependent regret of $\sum_{\ell=1}^L \frac{K}{\Delta_{\ell,\min}}$ over $L$ stationary phases with minimal gaps $\Delta_{\ell,\min}$ \citep{garivier2011,lattimore}.
	This suggests we cannot do a full blackbox reduction to finite-armed non-stationary bandits.
	\item Secondly, we observe that upon experiencing changes, it may be necessary to {\em re-sample} arms from the reservoir distribution or else the first sum in \Cref{eq:regret-decomp} can become large if the rewards of all arms in $\mc{A}_0$ degrade over time.
	Thus, we require a more refined subsampling strategy which works in tandem with non-stationarity detection.
\end{enumerate}

We handle both of the above issues with the new idea of tracking the empirical regret $1 - Y_t(a_t)$ as a proxy for tracking non-stationarity.
The key observation is that the empirical cumulative regret of played actions up to round $t$, $\sum_{s=1}^t 1 - Y_s(a_s)$, concentrates around $\sum_{s=1}^t 1 - \mu_s(a_s)$ at a rate of $\sqrt{t}$ by Freedman's inequality.

This means, so long as $\sum_{s=1}^t 1 - Y_s(a_s) \lesssim \sqrt{t}$, our regret will be safe up to stationary rates.
On the other hand, if $\sum_{s=1}^t 1 - Y_s(a_s) \gg \sqrt{t}$, then the learner must be experiencing large regret.

On the other side, if the agent is playing according to an optimal algorithm for stationary infinite-armed bandits, then the only way large empirical regret is observed is if large non-stationarity has occurred.
Hence, checking empirical regret is a valid changepoint detection test.

Putting these observations together, our procedure (\Cref{alg:blackbox}), similar to the adaptive algorithms for the finite-armed setting \citep{auer2019,wei2021,suk22,abbasi22}, proceeds in episodes and restarts upon detecting non-stationarity.
A restart, or new episode, is triggered when the empirical regret over the current episode becomes too large.
Within each episode, we further employ doubling epochs, termed {\em blocks}, to account for unknown horizons and changepoints.


Going into more detail, our blackbox will rely on a stochastic finite-armed MAB base algorithm designed for stochastic environments, which we'll denote by $\base(t,\mc{A}_0)$, taking as input a horizon $t$ and finite subsample $\mc{A}_0$.

Our only requirement of $\base$ is that it attains a standard logarithmic regret bound in so-called mildly corrupt environments, defined below.
It's straightforward to show this is satisfied by classical stochastic MAB algorithms such as UCB \citep{LaiRo85} and Successive Elimination \citep{Even-Dar+02}.
We give proofs of these facts in \Cref{app:base}.

\begin{defn}\label{defn:mild}
	We say a finite-armed non-stationary bandit environment $\{ \mu_t(a)\}_{t \in [T], a \in \mc{A}_0}$ over horizon $T$ with armset $\mc{A}_0$ is {\bf mildly corrupt} if there exists a {\bf stationary reward profile} $\{ \mu(a)\}_{a \in \mc{A}_0}$ such that
\[
	\forall t \in [T] , a \in \mc{A}_0: |\mu_t(a) - \mu(a) | \leq \frac{1}{\sqrt{T}}.
\]
\end{defn}



\begin{assumption}\label{assumption:base}
	$\base(T,\mc{A}_0)$ attains, with probability at least $1-1/T$, for all $t \in [T]$, a $t$-round regret bound of
	\[
		\max_{a' \in \mc{A}_0} \sum_{s=1}^t \mu_s(a') - \mu_s(a_s) \leq C_0 \left( \sum_{i=2}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1}\{ \Delta_{(i)} \geq \sqrt{\log(T) / t} \} + \sqrt{t \log(T)} \right) . %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, T \cdot \Delta_{(2)} \right\} \right).
	\]
	in any $T$-round environment which is mildly corrupt with stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with ordered gaps $\Delta_{(2)} \leq \Delta_{(3)} \leq \cdots \Delta_{(|\mc{A}_0|)}$.
	%minimal gap
	%\[
		%\Delta_{\min} := \min_{a \in \mc{A}_0 \bs \{ \argmax_{a' \in \mc{A}_0} \mu(a') \} } \max_{a' \in \mc{A}_0} \mu(a') - \mu(a).
	%\]
\end{assumption}

%Next, our blackbox is surprisingly simple.
%In doubling epochs, we'll run $\base$ with a doubling set of subsampled arms and then restart the entire procedure based on checking the cumulative empirical regret $\sum_{s=1}^t 1 - Y_s(a_s) \gg \sqrt{t}$.
%This is captured in \Cref{alg:blackbox}.


\IncMargin{1em}
\begin{algorithm2e}[h]
 	\caption{{Blackbox Non-Stationary Algorithm}}
 \label{alg:blackbox}
 \bld{Input}: finite-armed MAB algorithm robust to mildly non-stationary environments $\base$. \\
 \bld{Initialize}: episode count $\ell \leftarrow 1$, first episode start round $t_1 \leftarrow 1$.\\
 \For{$m=1,2,\ldots,\ceil{\log(T)}$}{ \label{line:doubling}
		 Subsample $\ceil{2^{m/2}}$ arms $\mc{A}_m$ from the reservoir distribution.\\
		 Initiate a new instance of $\base(2^m,\mc{A}_m)$ with horizon $2^m$ and arm-set $\mc{A}_m$.\\
		 Let $t_{\ell}^m := t_{\ell} + 2^{m-1} - 1$ be the start of the $m$-th {\em block} in the $\ell$-th episode.\\
		 \For{$t = t_{\ell}^m,\ldots,t_{\ell}^m + 2^m$}{
			 Play arm $a_t$ as chosen by $\base(2^m,\mc{A}_m)$.\\
			 Obtain reward $Y_t(a_t)$ from $\base(2^m,\mc{A}_m)$.\\
			 \bld{Changepoint Test:} \uIf{$\sum_{s = t_{\ell}^m}^t 1 - Y_s(a_s) \geq C_1 \left( \sqrt{(t - t_{\ell}^m + 1) \log(T)} + \log(T) \right) $}{ \label{line:cpd-test}
				 Restart: $t_{\ell} \leftarrow t+1$, $\ell \leftarrow \ell+1$. \label{line:restart}\\
				 Return to \Cref{line:doubling}. \textcolor{red}{**JK: This may mean starting from $m=1$?**} \joe{yes, one must restart from $m=1$}
		}
	}
}
		 %\Indp $\mc{A}_{t} \leftarrow \mc{A}_{t} \bs \left\{a\in [K]:\text{$\exists $ round $t_0 \leq t$ s.t. $\underset{a' \in \mc{A}_t}{\max} \sum_{s=t_0}^{t} \hat{\delta}_s(a',a) > C_5\sqrt{\sum_{s=t_0}^t \frac{\log(T)}{|\mc{A}_s|} }$ holds}\right\}$. \label{line:evict-At}\\
 		%\Indm
\end{algorithm2e}
\DecMargin{1em}


The main result of this section is that \Cref{alg:blackbox} in fact attains the optimal regret in terms of number of changes $L$ and total-variation $V$.
The proof is surprisingly simple with much of the difficulty of non-stationarity handled by our \Cref{assumption:base} on the base algorithm.

\begin{thm}\label{thm:blackbox}
	\Cref{alg:blackbox} satisfies, with probability at least $1-1/T$:
	\[
		{\normalfont \bld{R}}_T \leq \tilde{O} \left( \sqrt{(L+1) T} \land V^{1/3} T^{2/3} \right) .
	\]
\end{thm}

\begin{proof}
	Let $t_{\ell}$ be the the $\ell$-th restart round per \Cref{line:restart} of \Cref{alg:blackbox} so that $\ho{t_{\ell}}{t_{\ell+1}}$ is the $\ell$-th episode.
	Let $\hat{L}$ be the (random) number of restarts triggered over $T$ rounds.

	\paragraph*{$\bullet$ Using Empirical Regret Bound to get Regret Bound.}
	Next, we establish a high-probability event over which our empirical regret concentrates around its mean.
	First, fix an interval of rounds $[s_1,s_2]$.
	Then, we note that
	\[
		\sum_{s=s_1}^{s_2} Y_s(a_s) - \mb{E}[ Y_s(a_s) \mid \mc{H}_{s-1}],
	\]
	is a martingale difference sequence with respect to the natural filtration $\{\mc{H}_t\}_t$ of $\sigma$-algebras $\mc{H}_{t}$, generated by the observations and decisions (of both decision-maker and adversary) up to round $t-1$.

	Now, since the choice of arm $a_t$ at round $t$ is fixed conditional on $\mc{H}_{t-1}$, we have $\mb{E}[ Y_t(a_t) \mid \mc{H}_{t-1}] = \mu_t(a_t)$.

	\textcolor{red}{**JK: I was just wondering the reason to use Freedman inequality.**} \joe{I need martingale concentration since R.V.'s are not iid, variance scaling is not important here and Azuma or Bernstein would have also sufficed. Later on, in proof of \Cref{thm:regret-episodes}, Freedman's variance scaling is important}
	Then, by Freedman's inequality (\Cref{lem:freedman}) we have with probability at least $1 - 1/T^3$,
	\[
		\left| \sum_{s=s_1}^{s_2} Y_s(a_s) - \mu_s(a_s)  \right| \leq 3 \sqrt{ (s_2-s_1+1) \cdot \log\left(2 T^3 \right) } + 2 \log\left( 2 T^3 \right) .
	\]
	Taking a further union bound over all choices of intervals $[s_1,s_2]$, we have that, with probability at least $1 - 1/T$, for all final blocks $\ho{t_{\ell}^m}{t_{\ell+1}}$:
	\[
		\left| \sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} (1 - Y_s(a_s)) - (1 - \mu_s(a_s)) \right| \leq 3\sqrt{ 3 (t_{\ell+1} - t_{\ell}^m) \log(2T)} + 6\log(2T).
	\]
	Let $\mc{E}_1$ be the good event on which this concentration holds for episodes $\ell$ and blocks $m$.
	Thus, summing over blocks and episodes, a regret bound of $\log(T) \sum_{\ell=1}^{\hat{L}} \sqrt{t_{\ell+1} - t_{\ell}}$ is evident on $\mc{E}_1$. \textcolor{red}{**JK: Could you explain this for me?**}

	\rev{
		Let $t_{\ell}^m$ denote the start round of the $m$-th block in the $\ell$-th episode and let $t_{\ell}^m := t_{\ell+1}$ if the $(m-1)$-th block resulted in a restart.
		Then, we first decompose the regret along episodes and blocks contained therein:
		\[
			\sum_{t=1}^T 1 - \mu_t(a_t) = \sum_{\ell = 1}^{\hat{L}} \sum_m \sum_{t = t_{\ell}^m}^{t_{\ell}^{m+1}-1} 1 - \mu_t(a_t).
		\]
		Then, on event $\mc{E}_1$, by Freedman, each inner sum $\sum_t 1 - \mu_t(a_t)$ concentrates around its mean $\sum_t 1 - Y_t(a_t)$ with concentration error
		\[
			\sqrt{(t_{\ell}^{m+1} - t_{\ell}^m) \cdot \log(T)} + \log(T).
		\]
		Thus, on event $\mc{E}_1$:
		\[
			\sum_{t=1}^T 1 - \mu_t(a_t) = \sum_{\ell} \sum_m \sqrt{(t_{\ell}^{m+1} - t_{\ell}^m) \cdot \log(T)} + \log(T) + \sum_{t=t_{\ell}^m}^{t_{\ell}^{m+1} - 1} 1 - Y_t(a_t).
		\]
		Then, we upper bound each inner sum over $t$ on the RHS using \Cref{line:cpd-test} by $\sqrt{(t_{\ell}^{m+1} - t_{\ell}^m)\log(T)}$  \textcolor{red}{*jk*} because
		Acknowledging that the periods $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$ are doubling blocks for the larger episode $\ho{t_{\ell}}{t_{\ell+1}}$, we can upper bound the resultant sum over $m$ by $\sqrt{t_{\ell+1} - t_{\ell}}$ by introducing another $\log^{1/2}(T)$ factor and using Jensen.
	}

	\paragraph*{$\bullet$ Showing \Cref{line:cpd-test} is a Valid Changepoint Detection Test.}
	It then remains to show
	\[
		\sum_{\ell=1}^{\hat{L}} \sqrt{t_{\ell+1} - t_{\ell}} \leq \sqrt{(L+1) \cdot T} \land V^{1/3} T^{2/3},
	\]
	which amounts to showing \Cref{line:cpd-test} of \Cref{alg:blackbox} is a valid changepoint detection test which doesn't restart unnecessarily.



	Then, for large enough choice of threshold $C_1>0$ in \Cref{line:cpd-test}, we have that a restart in the $\ell$-th episode corresponds to large regret for the final block $\ho{t_{\ell}^m}{t_{\ell+1}}$:
	\begin{equation}\label{eq:large-regret-last-block}
		\sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(a_s) \geq C_2 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T) \right).
	\end{equation}
	Now, let $\mc{E}_2$ be the high-probability event of \Cref{assumption:base} holds.
	Then, it remains to show on event $\mc{E}_1 \cap \mc{E}_2$ that either (a) the regret of the best subsampled arm is large (indicating large variation) or (b) the subsampled bandit environment over the rounds $\ho{t_{\ell}^m}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).  \textcolor{red}{**JK: Could you explain this for me?**}
	\joe{sorry this explanation was rushed. Using the notation from below, we can decompose the regret  in the final block of the episode as
		\[
			\sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(a_s) = \sum_s 1 - \mu_s(\hat{a}_{\ell,m}) + \sum_s \mu_s(\hat{a}_{\ell,m}) - \mu_s(a_s).
		\]
		Thus, we know from \Cref{eq:large-regret-last-block} that one of the two sums on the RHS above is large.
		If the first sum is large, we want to show this implies large variation must have elapsed in the episode.
		Our goal is to show in both situations that the variation over the episode is large or that $\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \gtrsim (t_{\ell+1} - t_{\ell})^{-1/2}$.\textcolor{red}{*jk: in the middle*}
	}

	Let $\hat{a}_{\ell,m}$ be the best arm in terms of initial reward among the arms $\mc{A}_m$ subsampled for block $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$.
	We first argue that with probability at least $1-1/T$,
	\[
		\mu_0(\hat{a}_{\ell,m}) > 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}.
	\]
	This is true since
	\begin{align*}
		\mb{P}(\mu_0(\hat{a}_{\ell,m}) < 1 - (t_{\ell+1} - t_{\ell}^m)^{-1/2}) &\leq \left( 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \right)^{|\mc{A}_0|} \\
										       &\leq \exp\left( - |\mc{A}_0| \cdot \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \right) \\
										       &\leq \frac{1}{T},
	\end{align*}
	where the last inequality follows from $|\mc{A}_0| \geq \sqrt{t_{\ell+1} - t_{\ell}^m}$.

	Now, using the regret decomposition of \Cref{eq:regret-decomp}, if
	\begin{equation}\label{eq:bad-reg-best}
		\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(\hat{a}_{\ell,m}) > 2\log(T)\sqrt{t_{\ell+1} - t_{\ell}^m},
	\end{equation}
	then we must have with probability at least $1/T$ that the variation must be at least
	\[
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}},
	\]
	since the adversary can only modify the rewards of arms $a_t$ after the round $t$ they're played. \textcolor{red}{**JK: Could you explain this for me?**}
	\joe{
	From our earlier tail probability bound, we know $\delta_0(\hat{a}_{\ell,m}) < \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}$.
	We also know from (3) above that there exists a round $t \in \ho{t_{\ell}^m}{t_{\ell+1}}$ such that
	\[
		\delta_t(\hat{a}_{\ell,m}) > \frac{2\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}.
	\]
	This means the gap of arm $\hat{a}_{\ell,m}$ must have moved by amount $\frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}$ over the course of the block.
	Since the adversary can only modify the rewards of an arm $a_t$ after the round $t$ it is played, this must have occurred on a round where $\hat{a}_{\ell,m}$ was chosen by the agent.
	Thus,
	\[
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}.
	\]

}

	Suppose, going forward that \Cref{eq:bad-reg-best} is reversed.
	By our regret decomposition \Cref{eq:regret-decomp} and the restart criterion (\Cref{line:restart}) of \Cref{alg:blackbox}, for $C_1$ large enough, this must mean that:
	\[
		\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} \mu_s(\hat{a}_{\ell}^m) - \mu_s(a_s) \gtrsim \sqrt{(t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T).
	\]


	Then, we want to show that the subsampled bandit environment over the episode is not mildly corrupt. \textcolor{red}{**jk: <-could you explain why?**}
	\joe{basically, I want to arrive at a contradiction: if the subsampled bandit environment was only mildly corrupt, then the restart criterion (\Cref{line:restart}) would not be triggered.
	Taking the contrapositive of this statement, I want to show that if the restart criterion is triggered, then the subsampled bandit environment must be more heavily corrupt.
	}
	In other words, by \Cref{assumption:base}, we want to show by contradiction that if it were mildly corrupt with stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with gaps $\{ \Delta_a\}_{a \in \mc{A}_0}$, then:
	\begin{equation}\label{eq:bound-gap-rate}
		C_2 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T) \right) > C_0 \left( \sum_{i=3}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}}} \right\}  + \sqrt{ (t_{\ell+1} - t_{\ell}) \cdot \log(T)} \right). %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, (t_{\ell+1} - t_{\ell}) \cdot \Delta_{(2)} \right\} \right),
	\end{equation}
	%for any stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with ordered gaps $\Delta_{(2)} \leq \Delta_{(3)} \leq \cdots \Delta_{(|\mc{A}_0|)}$.
	We'll show this sub-claim by refining the sum over $i = 3, \ldots, |\mc{A}_0|$ into a geometric grid based on the values of the gaps and applying concentration over the number of gaps which fall within a particular segment of said grid.

	For $j = 0, \ldots, \ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}}{\log(T)} \right) }$, let $N_j := \sum_{j=3}^{|\mc{A}_0|} \pmb{1}\left\{ \Delta_{(j)} \in [ 2^{-(j+1)}, 2^{-j} ) \right\}$.
	Then, we bound
	\begin{align*}
		\sum_{i=3}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}}} \right\} &\leq \sum_{j=0}^{\ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}}{\log(T)} \right) }} N_j \cdot 2^{j+1}.
	\end{align*}
	Let $\mu_{m,(1)}$ be the top initial reward of the arms $\mc{A}_m$ subsampled during block $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$.
	Next, by a multiplicative Chernoff bound, since, conditional on $\mu_{m,(1)}$, the gaps are uniform random variables with order statistics $\Delta_{(2)},\ldots,\Delta_{(|\mc{A}_0|)}$.
	This means $N_j$ has mean $|\mc{A}_0| \cdot 2^{-(j+1)}$ so that:
	\[
		\mb{P}\left( N_j \geq 2 \cdot |\mc{A}_0| \cdot 2^{-(j+1)} \mid \mu_{m,(1)} \right) \leq \exp\left( - |\mc{A}_0| \cdot 2^{-(j+1)} / 3 \right).
	\]
	The RHS is less than $T^{-3}$ for $t_{\ell+1} - t_{\ell}$ sufficiently larger than a constant.
	Using tower law, the tail probability upper bound also holds unconditional of $\mu_{m,(1)}$, for all $j$.
	Let $\mc{E}_3$ be the corresponding high-probability event.

	Thus, on event $\mc{E}_1 \cap \mc{E}_2 \cap \mc{E}_3$, we have $N_j < 2 \cdot |\mc{A}_0| \cdot 2^{-(j+1)}$ and so
	\[
		N_j \cdot 2^{j+1} \leq 2 \cdot |\mc{A}_0|.
	\]
	Thus,
	\[
		\sum_{i=3}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}}} \right\} \leq 2 \ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}}{\log(T)} \right) } \cdot |\mc{A}_0| \leq 2\log(T) \cdot |\mc{A}_0|.
	\]
	Now,
	\[
		|\mc{A}_0| \leq \ceil{2^{m/2}} \leq \ceil{\sqrt{ t_{\ell+1} - t_{\ell}}}.
	\]

	Thus, \Cref{eq:bound-gap-rate} is shown which shows that the bandit environment over the rounds $\ho{t_{\ell}}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).

	This means that since the adversary can only modify the rewards of arms $a_t$ after the round $t$ they're played, the variation of change in each episode $\ho{t_{\ell}}{t_{\ell+1}}$ concluding with a restart must be at least
	\[
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{1}{\sqrt{t_{\ell+1} - t_{\ell}}}.
	\]
 
\jk{I'm currently struggling to understand that the left hand side above is increasing when the gap between $t_l$ and $t_{l+1}$ increases while the right hand side decreases. Could you provide some insights for it?}
\joe{Yes, this is a correct observation. The LHS increases as the episode duration $t_{\ell+1} - t_{\ell}$ increases while the RHS decreases.
	My intuition for this is as follows: if the episode $\ho{t_{\ell}}{t_{\ell+1}}$ is longer than that means we haven't detected a change over a longer period.
	This means the safe amount of total variation that can be accounted for in the episode is {\bf smaller} because our guarantees are more sensitive to small changes (i.e., finding a $T^{-1/2}$ optimal arm will be sensitive to $T^{-1/2}$ magnitude changes and thus sensitivitiy increases as $T$ increases).
	Viewed another way, \Cref{defn:mild} becomes more restrictive as $T$ increases.

	I think we can also view it the following way: if our \Cref{alg:blackbox} experiences a longer episode $\ho{t_{\ell}}{t_{\ell+1}}$, then that means it's very confident about the environment being stationary and finding the best arm over that episode.
	That higher confidence is more sensitive to a slight perturbation in the rewards which is why the threshold $(t_{\ell+1} - t_{\ell})^{-1/2}$ is smaller.
}

    This allows us to further bound the rate
	\[
		\sum_{\ell=1}^{\hat{L}} \sqrt{t_{\ell+1} - t_{\ell}} \leq \sqrt{(L+1) \cdot T} \land V^{1/3} T^{2/3}.
	\]
	In particular, the above is achieved using standard arguments seen in prior works \citep[Lemma 26]{wei2021} \citep[Corollary 2]{suk22}.
	%If we restart $\sum_{s=1}^t 1 - Y_s(a_s) \gtrsim \sqrt{t}$, then this means $\sum_{s=1}^t 1 - \mu_s(a_s) \gtrsim \sqrt{t}$.
	%This means large total variation must have elapsed in the environment so long as we have the base algorithm guarantee:
	%\[
		%\sum_{s=1}^t 1 - \mu_s(a_s) \lesssim \sqrt{t},
	%\]
	%in all environments with small total variation (at most $t^{-1/2}$ over $t$ rounds).
\end{proof}


\begin{rmk}
	At first glance, our base algorithm assumption (\Cref{assumption:base}) seems similar to Assumption 1 of \citet{wei2021}, but our base algorithm needs to maintain {\bf gap-dependent regret bounds} in environments with variation at most $T^{-1/2}$ which is stronger than their requirement of maintaining $\sqrt{KT}$ regret in nearly stationary $T$-round environments for $K$-armed bandits.
\end{rmk}

\begin{rmk}
	Bandit algorithm with optimal regret guarantees in {\bf stochastic regimes with adversarial corruption} \citep{lykouris18,zimmert19,ito21,ito23,dann23} would suffice for \Cref{assumption:base} as one can view our ``mildly corrupt'' regime as falling under these works' setting with corruption parameter of $T^{-1/2}$.
\end{rmk}


==> scrap/blackbox_details.tex <==
\section{Details for the Proof of \Cref{thm:blackbox}}

We first present Freedman's inequality which was used in \Cref{sec:blackbox} to bound the regret using the empirical regret bound of \Cref{line:cpd-test} of \Cref{alg:blackbox}.

\begin{lemma}[Strengthened Freedman's Inequality, Theorem 9 \citep{zimmert22}]\label{lem:freedman}
	Let $X_1,X_2,\ldots,X_T$ be a martingale difference sequence with respect to a filtration $\mc{F}_1 \subseteq \mc{F}_2 \subseteq \cdots \subseteq \mc{F}_T$ such that $\mb{E}[X_t \mid \mc{F}_t ] = 0$ and assume $\mb{E}[ | X_t | \mid \mc{F}_t] < \infty$ a.s.. Then, with probability at least $1-\delta$,
	\[
		\sum_{t=1}^T X_t \leq 3 \sqrt{ V_t \log\left( \frac{2 \max\{ U_t, \sqrt{V_T}\}}{\delta} \right) } + 2 U_T \log \left( \frac{2 \max\{ U_T, \sqrt{V_T}\}}{\delta} \right),
	\]
	where $V_T = \sum_{t=1}^T \mb{E}[ X_t^2 \mid \mc{F}_t]$, and $U_T = \max \{ 1 ,\max_{s \in [T]} X_s \}$.
\end{lemma}

\subsection{Using Concentration to Bound Per-Block Regret (Proof of \Cref{lem:concentration-bounds})}\label{subsec:proof-concentration-bounds}

First, fix an interval of rounds $[s_1,s_2]$.
Then, we note that
\[
	\sum_{s=s_1}^{s_2} 1 - Y_s(a_s) - \mb{E}[ 1 - Y_s(a_s) \mid \mc{H}_{s-1}],
\]
is a martingale difference sequence with respect to the natural filtration $\{\mc{H}_t\}_t$ of $\sigma$-algebras $\mc{H}_{t}$, generated by the observations and decisions (of both decision-maker and adversary) up to round $t-1$.
Now, since the choice of arm $a_t$ at round $t$ is fixed conditional on $\mc{H}_{t-1}$, we have $\mb{E}[ Y_t(a_t) \mid \mc{H}_{t-1}] = \mu_t(a_t)$.
We also have
\[
	\Var( 1 - Y_t(a_t) \mid \mc{H}_{t-1} ) \leq \mb{E}[ (1 - Y_t(a_t))^2 \mid \mc{H}_{t-1}] \leq \mb{E}[ 1 - Y_t(a_t) \mid \mc{H}_{t-1} ] = \delta_t(a_t).
\]
% \textcolor{red}{**JK: I was just wondering the reason to use Freedman inequality.**} \joe{I need martingale concentration since R.V.'s are not iid, variance scaling is not important here and Azuma or Bernstein would have also sufficed. Later on, in proof of \Cref{thm:regret-episodes}, Freedman's variance scaling is important}
Then, by Freedman's inequality (\Cref{lem:freedman}) we have with probability at least $1 - 1/T^3$: for all choices of intervals $[s_1,s_2] \subseteq [T]$:
\begin{align}
	\left| \sum_{s=s_1}^{s_2} (1 - Y_s(a_s)) - (1 - \mu_s(a_s))  \right| &\leq 3 \sqrt{  \log\left(2 T^3 \right) \sum_{s=s_1}^{s_2} \delta_s(a_s) } + 2 \log\left( 2 T^3 \right) \nonumber \\
									     &\leq \half \sum_{s=s_1}^{s_2} \delta_s(a_s) + \frac{13}{2}\log(2T^3), \label{eq:good_event1}
\end{align}
where the second inequality is by AM-GM.
%Let $t_{\ell}^m := t_{\ell+1}$ if the $(m-1)$-th block resulted in a restart and {$m_\ell$ be the last block in the $\ell$-th episode.}	 Taking a further union bound over all choices of intervals $[s_1,s_2] \subseteq [T]$, we have that, with probability at least $1 - 1/T$, we have
%\begin{align}
	%\jk{\left| \sum_{s=s_1}^{s_2} (1-Y_s(a_s)) - (1-\mu_s(a_s))  \right| \leq 3 \sqrt{ 3(s_2-s_1+1) \cdot \log\left(2 T \right) } + 6 \log\left( 2 T\right) .}\label{eq:good_event1}
%\end{align}
Let $\mc{E}_1$ be the good event on which this concentration of \eqref{eq:good_event1} holds for all subintervals $[s_1,s_2] \subseteq [T]$.
%Then under $\mc{E}_1$,
%for all blocks of $[t_\ell^{m},t_\ell^{m+1})$ for $l\in[\hat{L}]$ and $m\in[m_\ell]$:
%% for all final blocks $\ho{t_{\ell}^m}{t_{\ell+1}}$:
%\begin{align*}
	%\left| \sum_{s=t_{\ell}^m}^{\jk{t_{\ell}^{m+1}-1}} (1 - Y_s(a_s)) - (1 - \mu_s(a_s)) \right| \leq 3\sqrt{ 3 (\jk{t_{\ell}^{m+1}}   - t_{\ell}^m) \log(2T)} + 6\log(2T).
%\end{align*}
%Let $\mc{E}_1$ be the good event on which this concentration of \eqref{eq:good_event1} holds for all episodes $\ell$ and blocks $m$.

At the same time, on each $m$-th block, \Cref{line:cpd-test} of \Cref{alg:blackbox} gives us an empirical regret upper bound since the changepoint test is not triggered until possibly the last round of the block.
%\jk{except $m_\ell$}:
\rev{Specifically, the inequality in \Cref{line:cpd-test} of \Cref{alg:blackbox} must be reversed for the second-to-last round of the block or
\[
	\sum_{s=t_{\ell}^m}^{t_{\ell}^{m+1} -2} 1 - Y_s(a_s) < C_1 \cdot |\mc{A}_m| \cdot \log(T), % \implies \sum_{s=t_{\ell}^m}^{t_{\ell}^m-1} 1 - Y_s(a_s) < C_1 \cdot |\mc{A}_m| \cdot \log(T) + 1,
\]
where by convention we let $t_{\ell}^{m_{\ell}+1} := t_{\ell+1}$.
Thus,
}
\begin{equation}\label{eq:empirical-upper-bound}
	\sum_{s=t_{\ell}^m}^{t_{\ell}^{m+1}-1} 1 - Y_s(a_s) < C_1 \cdot |\mc{A}_m| \cdot \log(T) + 1.
\end{equation}
%Now, we note
%\[
	%|\mc{A}_m| \geq C_2 2^{m \frac{\beta}{\beta+1}} \cdot \log^{\frac{1}{\beta+1}}(T) \geq C_2 \log(T),
%\]
%for $2^m \geq \log(T)$.
%Going forward, we only consider {\em long blocks} where $2^m \geq \log(T)$.
Combining the above with \Cref{eq:good_event1}, we conclude
\[
	\sum_{s=t_{\ell}^m}^{t_{\ell}^{m+1}-1} \delta_s(a_s) < 2 C_1 \cdot |\mc{A}_m| \cdot \log(T) + 2 + 13\log(2T^3) \leq 3 C_1 \cdot |\mc{A}_m| \cdot \log(T).
\]
where the last inequality holds for $C_1$ large enough.

At the same time, for constant $C_1$ in \Cref{line:cpd-test} of \Cref{alg:blackbox} chosen large enough, we have that, for the last block $\ho{t_{\ell}^{m_{\ell}}}{t_{\ell+1}}$ of an episode concluding in a restart, we must have
\begin{align*}
	\sum_{s=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} 1 - Y_s(a_s) &\geq C_1 \cdot |\mc{A}_m| \cdot \log(T) \implies \\
	\sum_{s=t_{\ell}^{m_{\ell}}}^{t_{\ell+1}-1} \delta_s(a_s) &\geq \frac{2C_1}{3} \cdot |\mc{A}_{m_{\ell}}| \cdot \log(T) - \frac{13}{3} \log(2T^3) \geq \frac{C_1}{2} \cdot |\mc{A}_{m_{\ell}}| \cdot \log(T),
\end{align*}
where the first inequality in the second line above comes from combining the first line with \Cref{eq:good_event1} and the last inequality holds for $C_1$ large enough.

\subsection{Summing Regret Over Blocks (Proof of \Cref{lem:regret-bd-episode-length})}\label{subsec:proof-regret-bd-ep-length}

We first decompose the regret along episodes and blocks contained therein:
		\[
			\sum_{t=1}^T 1 - \mu_t(a_t) = \sum_{\ell = 1}^{\hat{L}} \sum_{m\in [m_\ell]} \sum_{t = t_{\ell}^m}^{t_{\ell}^{m+1}-1} 1 - \mu_t(a_t).
		\]
		% Then, on event $\mc{E}_1$, by Freedman, each inner sum $\sum_t 1 - \mu_t(a_t)$ concentrates around its mean $\sum_t 1 - Y_t(a_t)$ with concentration error
		% \[
		% 	\sqrt{(t_{\ell}^{m+1} - t_{\ell}^m) \cdot \log(T)} + \log(T).
		% \]
		Then, on event $\mc{E}_1$, we have summing \Cref{eq:block-bound}: \jkc{The regret of the last block for each episode may not be bounded. how can we get the below?}
        \begin{align*}
            \sum_{t=1}^T 1 - \mu_t(a_t)  &\leq
	    \sum_{\ell\in [\hat{L}]} \sum_{m\in[m_\ell]} 3 C_1 \cdot |\mc{A}_m| \cdot \log(T) \\
					 &\leq c_2 \sum_{\ell \in [\hat{L}]} \sum_{m \in [m_{\ell}]} 2^{m \cdot \frac{\beta}{\beta+1}} \log(T) \\
					 &\leq c_3 \sum_{\ell \in [\hat{L}]} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}} \cdot \log^{2}(T) .
        \end{align*}
	where in the last step we use Jensen's inequality w.r.t. the concave function $x \mapsto x^{\frac{\beta}{\beta+1}}$ on the sum over $m$.

		%Then, we upper bound the last inner sum over $m$ on the RHS as follows
        %\begin{align*}
            %&\sum_{\ell\in [\hat{L}]}\sum_{m\in [m_\ell]} \sum_{t=t_\ell^m}^{t_\ell^{m+1}-1}1-Y_t(a_t)\cr &=\sum_{\ell\in [\hat{L}]}\sum_{m\in [m_\ell-1]} \sum_{t=t_\ell^m}^{t_\ell^{m+1}-1}1-Y_t(a_t)+\sum_{\ell\in [\hat{L}]} \sum_{t=t_\ell^{m_\ell}}^{t_\ell^{m_\ell+1}-2}1-Y_t(a_t)+\sum_{\ell\in [\hat{L}]} 1-Y_{t_\ell^{m_\ell+1}-1}(a_{t_\ell^{m_\ell+1}-1})
            %\cr &\lesssim \sum_{\ell \in[\hat{L}]}\sum_{m\in [m_{\ell}]}\sqrt{(t_\ell^{m+1}-t_\ell^m)\log(T)}+ |\mc{A}_m|\log(T)+ \hat{L}
             %\cr &\lesssim \sum_{\ell \in[\hat{L}]}\sum_{m\in [m_{\ell}]}\sqrt{(t_\ell^{m+1}-t_\ell^m)\log(T)},
        %\end{align*}
        %where the first inequality is obtained from  the condition of \Cref{line:cpd-test} in Algorithm~\ref{alg:blackbox}.
	%Since the periods $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$ are doubling blocks for the  episode $\ho{t_{\ell}}{t_{\ell+1}}$, using Jensen's inequality, we can show that
    %\begin{align*}
	    %\sum_{m\in[m_\ell]}\sqrt{t_\ell^{m+1}-t_\ell^m}\le \sqrt{m_\ell \sum_{m\in[m_l]}(t_\ell^{m+1}-t_\ell^m)} \leq \sqrt{\log(T) \cdot ( t_{\ell+1}-t_\ell ) }.
    %\end{align*}
    %%which concludes the proof.

%\subsection{temp}
%Now, from \Cref{line:cpd-test}, and our earlier concentration bounds, we know that the LHS above must be large which means one of the two sums on the RHS must also be large or $\Omega(|\mc{A}_{m_{\ell}}|)$.
%If the first sum on the RHS above is large, then this already means there is sufficient variation in the episode since the initial gap is small, as asserted by the following lemma.
%
%On the other hand, if the second sum in the display above is large, then this also means large variation must have elapsed in the episode.
%The proof of this fact will be by contradiction.
%If there is little variation in the episode, then the finite-armed bandit environment experienced by the base algorithm is mildly corrupt (\Cref{defn:mild}) and so we can use \Cref{assumption:base} to bound the second sum in the display above.
%Now, the logarithmic regret bound of \Cref{assumption:base} can be further bounded by discretizing the gaps according to a geometric grid.
%Key in this argument is the following lemma:
%
%\begin{lemma}
	%Let $\{ \Delta_a \}_{a \in \mc{A}_0}$ be the the gaps of a subsample $\mc{A}_0$ of arms from a $\beta$-regular reservoir (\Cref{ass:reservoir}).
	%Then, let $\rho := \frac{2\kappa_2}{\kappa_1}$ where $\kappa_1,\kappa_2$ are as in \Cref{ass:reservoir}.
	%We then have
%\end{lemma}

\subsection{Showing there is Large Variation in Each Episode (Proof of \Cref{lem:variation-bound})}\label{subsec:proof-variation-bound}

% We first show that the variation over the episode is large, i.e. \[\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})| \gtrsim (t_{\ell+1} - t_{\ell})^{-1/2}.\]
%Here, we constrain our attention to long blocks of length $2^m \geq C_2^{\beta+1} \log(T)$ so that
%\[
	%C_2 \cdot 2^{m \cdot \frac{\beta}{\beta+1}} \cdot \log^{\frac{1}{\beta+1}}(T)  \leq 2^m,
%\]
%and
%\[
	%|\mc{A}_m| \geq C_2 \cdot 2^{m \cdot \frac{\beta}{\beta+1}} \cdot \log^{\frac{1}{\beta+1}}(T) \geq C_2 \log(T).
%\]
%%Now, for large enough choice of threshold $C_1>0$ in \Cref{line:cpd-test}, we have that a restart in the $\ell$-th episode corresponds to large regret for the final block $\ho{t_{\ell}^{m_\ell}}{t_{\ell+1}}$, so that under $\mc{E}_1$, for some constant $C>0$, we have
	%%\begin{align*}%\label{eq:large-regret-last-block}
		%%\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_t(a_t) \geq C \cdot |\mathcal{A}_{m_\ell}| .
	%%\end{align*}
%%Recall that $\hat{a}_{\ell,m}$ is the best arm in terms of initial reward value $\mu_0(\cdot)$ among the arms $\mc{A}_m$ subsampled for block $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$.
%%%We can decompose the regret  in the final block of the episode as
%%%\begin{equation}\label{eq:regret-decompose-block}
			%%%\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_t(a_t) = \sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell}) + \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t).
		%%%\end{equation}
%%% Then, it remains to show on event $\mc{E}_1 \cap \mc{E}_2$ that either (a) the regret of the best subsampled arm is large (indicating large variation) or (b) the subsampled bandit environment over the rounds $\ho{t_{\ell}^m}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).
%%
	%%% Then, for large enough choice of threshold $C_1>0$ in \Cref{line:cpd-test}, we have that a restart in the $\ell$-th episode corresponds to large regret for the final block $\ho{t_{\ell}^m}{t_{\ell+1}}$:
	%%% \begin{equation}\label{eq:large-regret-last-block}
	%%% 	\sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(a_s) \geq C_2 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T) \right).
	%%% \end{equation}
	%%% Now, let $\mc{E}_2$ be the high-probability event of \Cref{assumption:base} holds.
As outlined in the proof outline of \Cref{sec:blackbox}, in light of the regret lower bound \Cref{eq:large-regret-last-block} of \Cref{lem:concentration-bounds}, we consider two different cases which we recall below:
    %Then from the above display and \eqref{eq:large-regret-last-block}, one of two possible cases must hold: either
	\begin{align}
		\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell}) &\geq \frac{C_1}{4} |\mathcal{A}_{m_\ell}| \log(T) \tag{A}\label{eq:case1app} \\
		\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell}) &\leq \frac{C_1}{4} |\mathcal{A}_{m_\ell}| \log(T) \text{ and } \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t) \geq \frac{C_1}{4} |\mathcal{A}_{m_\ell}| \log(T) \tag{B}\label{eq:case2app}
	\end{align}
	Our goal is to show that in either case \Cref{eq:case1app} or \Cref{eq:case2app}, large variation must have elapsed over the episode.

	\paragraph*{$\bullet$ Best Initial Arm has Large Dynamic Regret.}
	We first consider the former case \Cref{eq:case1app}.
	First, we establish a lemma asserting the best initially subsampled arm has small inital gap with high probability.

\begin{lemma}\label{lem:best-initial-arm}
	Recall that $\mu_0(a)$ is the initial mean reward of arm $a$.
	Let $\hat{a}_{\ell,m_{\ell}}$ denote the best initial arm among the arms sampled in the last block of episode $\ho{t_{\ell}}{t_{\ell+1}}$ or $\hat{a}_{\ell,m_{\ell}} := \argmax_{a \in \mc{A}_{m_{\ell}}} \mu_0(a)$.
	Let $\mc{E}_3$ be the event that
	\[
		\forall \ell \in [\hat{L}] : 1 - \mu_0(\hat{a}_{\ell, m_{\ell}}) \leq 2^{1 - m_{\ell} \cdot \frac{1}{\beta+1}} \cdot \kappa_1^{-1/\beta}  \log(T).
	\]
	Then, $\mc{E}_3$ occurs with probability at least $1-1/T$.
\end{lemma}


	%We first consider the former case of $\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\gtrsim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $, where the regret of the best subsampled arm is large (indicating large variation).
% Let $\mu_0(a)$ denote the initial mean reward of arm $a$.
% Since
% 	\begin{align*}
% 		 \mb{P}\left(\mu_0(\hat{a}_{\ell,m_\ell}) < 1 - \jk{\log(T)} 2^{-m_{\ell}/2}\right)&=      \jk{\mb{P}\left(\max_{a\in \mathcal{A}_{m_\ell}}\mu_0(a) < 1 - \log(T) 2^{- m_{\ell}/2}\right)}    \\&\leq \left( 1 - \frac{\log(T)}{2^{m_{\ell}/2}} \right)^{|\mc{A}_{\jk{m_\ell}}|} \\
%         &\leq \exp\left( - |\mc{A}_{\jk{m_\ell}}| \cdot \frac{\log(T)}{ 2^{m_{\ell}/2}} \right) \\
% 		&\leq \frac{1}{T},
% 	\end{align*}
% 	where the last inequality follows from $|\mc{A}_{\jk{m_\ell}}| \geq 2^{m_{\ell}/2}$, we have,  with probability at least $1-1/T$,
On $\mc{E}_3$, we have
\begin{align}
\mu_0(\hat{a}_{\ell,m_\ell}) \geq 1 - \frac{2 \kappa_1^{-1/\beta} \log(T)}{2^{m_{\ell} \cdot \frac{1}{\beta+1}}} \geq 1 - \frac{2 \kappa_1^{-1/\beta} \log(T)}{ (t_{\ell+1} - t_{\ell}^{m_\ell})^{\frac{1}{\beta+1}}}.\label{eq:goodness-best-subsmapled-arm}
\end{align}
    % From the above tail probability bound, we know $1-\mu_0(\hat{a}_{\ell,m_\ell}) < \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}$.
From \eqref{eq:case1app} (with large enough $C_1 > 24 \kappa_1^{-1/\beta}$), we also know that there exists a round $t' \in \ho{t_{\ell}^{m_\ell}}{t_{\ell+1}}$ such that
	\[
		1- \mu_{t'}(\hat{a}_{\ell,m_\ell}) > \frac{C_1 \cdot |\mc{A}_{m_{\ell}}| \cdot \log(T)}{4 (t_{\ell+1} - t_{\ell}^{m_{\ell}} ) } \geq \frac{24 \kappa_1^{-1/\beta} \cdot 2^{m_{\ell} \cdot \frac{\beta}{\beta+1}} \cdot \log(T)}{ 4 \cdot 2  \cdot 2^{m_{\ell}}} \geq \frac{3 \kappa_1^{-1/\beta} \log(T)}{ (t_{\ell+1} - t_{\ell}^{m_\ell})^{\frac{1}{\beta+1}} }.
	\]
	This means the mean reward of arm $\hat{a}_{\ell,m_\ell}$ must have moved by amount at least
	\[
		\frac{\kappa_1^{-1/\beta} \log(T)}{ (t_{\ell+1} - t_{\ell}^{m_\ell})^{\frac{1}{\beta+1}} } \geq \frac{\log(T)}{ (t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}}},
	\]
	\rev{(by choosing $\kappa_1$ small enough in \Cref{ass:reservoir})}
	\jkc{<-the inequality always holds?} over the course of the block, implying
	\[
		\mu_0(\hat{a}_{\ell,m_\ell})-\mu_{t'}(\hat{a}_{\ell,m_\ell})\ge \frac{\log(T)}{ (t_{\ell+1} - t_{\ell}^{m_\ell})^{\frac{1}{\beta+1}} } \geq \frac{\log(T)}{ (t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}} }.
	\]
	Since the adversary can only modify the rewards of an arm $a_t$ after the round $t$ it is played, the movement must have occurred on rounds where $\hat{a}_{\ell,m_\ell}$ was chosen by the agent.
	Thus,
	\[
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})|\ge \sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(\hat{a}_{\ell,m_\ell}) - \mu_{t-1}(\hat{a}_{\ell,m_\ell})|\ge \mu_0(\hat{a}_{\ell,m_\ell})-\mu_{t'}(\hat{a}_{\ell,m_\ell}) \geq \frac{\log(T)}{ (t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}} }.
	\]


% 	Then, it remains to show on event $\mc{E}_1 \cap \mc{E}_2$ that either (a) the regret of the best subsampled arm is large (indicating large variation) or (b) the subsampled bandit environment over the rounds $\ho{t_{\ell}^m}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).  \textcolor{red}{**JK: Could you explain this for me?**}
% 	\joe{sorry this explanation was rushed. Using the notation from below, we can decompose the regret  in the final block of the episode as
% 		\[
% 			\sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(a_s) = \sum_s 1 - \mu_s(\hat{a}_{\ell,m}) + \sum_s \mu_s(\hat{a}_{\ell,m}) - \mu_s(a_s).
% 		\]
% 		Thus, we know from \Cref{eq:large-regret-last-block} that one of the two sums on the RHS above is large.
% 		If the first sum is large, we want to show this implies large variation must have elapsed in the episode.
% 		Our goal is to show in both situations that the variation over the episode is large or that $\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \gtrsim (t_{\ell+1} - t_{\ell})^{-1/2}$.\textcolor{red}{*jk: in the middle*}
% 	}

% 	Let $\hat{a}_{\ell,m}$ be the best arm in terms of initial reward among the arms $\mc{A}_m$ subsampled for block $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$.
% 	We first argue that with probability at least $1-1/T$,
% 	\[
% 		\mu_0(\hat{a}_{\ell,m}) > 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}.
% 	\]
% 	This is true since
% 	\begin{align*}
% 		\mb{P}(\mu_0(\hat{a}_{\ell,m}) < 1 - (t_{\ell+1} - t_{\ell}^m)^{-1/2}) &\leq \left( 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \right)^{|\mc{A}_0|} \\
% 										       &\leq \exp\left( - |\mc{A}_0| \cdot \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \right) \\
% 										       &\leq \frac{1}{T},
% 	\end{align*}
% 	where the last inequality follows from $|\mc{A}_0| \geq \sqrt{t_{\ell+1} - t_{\ell}^m}$.

% 	Now, using the regret decomposition of \Cref{eq:regret-decomp}, if
% 	\begin{equation}\label{eq:bad-reg-best}
% 		\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(\hat{a}_{\ell,m}) > 2\log(T)\sqrt{t_{\ell+1} - t_{\ell}^m},
% 	\end{equation}
% 	then we must have with probability at least $1/T$ that the variation must be at least
% 	\[
% 		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}},
% 	\]
% 	since the adversary can only modify the rewards of arms $a_t$ after the round $t$ they're played. \textcolor{red}{**JK: Could you explain this for me?**}
% 	\joe{
% 	From our earlier tail probability bound, we know $\delta_0(\hat{a}_{\ell,m}) < \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}$.
% 	We also know from (3) above that there exists a round $t \in \ho{t_{\ell}^m}{t_{\ell+1}}$ such that
% 	\[
% 		\delta_t(\hat{a}_{\ell,m}) > \frac{2\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}.
% 	\]
% 	This means the gap of arm $\hat{a}_{\ell,m}$ must have moved by amount $\frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}$ over the course of the block.
% 	Since the adversary can only modify the rewards of an arm $a_t$ after the round $t$ it is played, this must have occurred on a round where $\hat{a}_{\ell,m}$ was chosen by the agent.
% 	Thus,
% 	\[
% 		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}.
% 	\]

% }

	% Suppose, going forward that \Cref{eq:bad-reg-best} is reversed.

	\paragraph*{$\bullet$ Regret of Base Algorithm is Large.}
	Now, we consider the other case \Cref{eq:case2app}, where
	%of $\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t)\gtrsim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $, where
	the regret of the subsampled bandit environment over the rounds $\ho{t_{\ell}^{m_\ell}}{t_{\ell+1}}$ is large, while the dynamic regret of the best initial arm is small.
	In this case, we want to show a contradiction: that if the total variation over the episode is small, then the finite MAB environment experienced by the base algorithm must be mildly corrupt (\Cref{defn:mild}) which means \Cref{assumption:base} can be used to bound the regret of the last block.
	This will yield a contradiction since by virtue of \Cref{line:cpd-test} being triggered, we know the regret of the last block be large.

	Suppose for contradiction that
	\begin{equation}\label{eq:small-variation-contradiction}
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| < \frac{1}{(t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}}}.
	\end{equation}
	Then, since our adaptive adversary can only change the rewards of arms on the rounds they are played, we must have the bandit environment experienced by the base algorithm must be mildly corrupt (\Cref{defn:mild}) with respect to initial reward profile $\{\mu(a)\}_{a \in \mc{A}_{m_{\ell}}}$.

	This means we can employ \Cref{assumption:base} with $\alpha=\beta$ to bound the regret.
	In particular, our end goal here is to show that
	\begin{equation}\label{eq:blackbox-regret-small}
		\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_{\ell}}) - \mu_t(a_t) < \frac{C_1}{4} \cdot |\mc{A}_{m_{\ell}}| \log(T) ,
	\end{equation}
	which will contradict \Cref{eq:case2app}.
	%For constant $c_2$ scaling like the constant $C_1$ appearing in \Cref{line:cpd-test} of \Cref{alg:blackbox}, this will yield a contradiction since the changepoint test being triggered at the end of the block means the above cannot be true for such $C$.
	%%$\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\lesssim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $.   We want to show that the subsampled bandit environment over the last block of each episode is not mildly corrupt by a contradiction.  From \Cref{assumption:base}, if it were mildly corrupt with stationary reward profile \jk{$\{\mu_0(a)\}_{a \in \mc{A}_{m_\ell}}$ with gaps $\{ \Delta_a\}_{a \in \mc{A}_{m_\ell}}$} (Definition~\ref{defn:mild}), then we can show that:
%\begin{equation}
		%C_1 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mc{A}_{m_{\ell}}|\cdot \log(T) \right) > \sum_{t=t_\ell^m}^{t_{\ell+1}-1} 1-Y_t(a_t).
        %%\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, (t_{\ell+1} - t_{\ell}) \cdot \Delta_{(2)} \right\} \right),
	%\end{equation}
	%Given the regret decomposition of \Cref{eq:regret-decompose-block} and our assumption that the dynamic regret of the best initial arm $\sum_{t=t_{\ell}^{m_{\ell}}}^{t_{\ell+1}-1} 1 - \mu_t(\hat{a}_{\ell,m_{\ell}})$ is small, it remains to show
	%\begin{equation}\label{eq:blackbox-regret-small}
		%\sum_{t=t_{\ell}^{m_{\ell}}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_{\ell}}) - \mu_t(a_t) \leq \frac{c_2}{2} \cdot |\mc{A}_{m_{\ell}}| .
	%\end{equation}
	First, by \Cref{assumption:base} with $\alpha = \beta$, we have
	\[
		\sum_{t=t_{\ell}^{m_{\ell}}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_{\ell}}) - \mu_t(a_t) \leq C_0 \left( \sum_{i=2}^{|\mc{A}_{m_{\ell}}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1}\left\{ \frac{\Delta_{(i)}}{4} \geq \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}}} \right)^{\frac{\beta}{\beta+1}} \right\} + (t_{\ell+1} - t_{\ell}^{m_{\ell}} )^{\frac{1}{\beta+1}} \cdot \log^{\frac{\beta}{\beta+1}}(T) \right).
	\]
	Now, recall the constants $\kappa_1, \kappa_2$ from our notion of $\beta$-regular reservoir distribution \Cref{ass:reservoir}.
	By definition, we must have $\kappa_2 > \kappa_1$.
	In fact, suppose WLOG that $\kappa_2 \geq 72$ and that $2\kappa_2/\kappa_1 \geq 2$.
	Let $\rho :=   \frac{2\kappa_2}{ \kappa_1}   $.
	%Now, we will follow the argument we did above for the uniform distribution, but instead of using a dyadic grid to
	To easen notation, we now parametrize the arms in $\mc{A}_{m_{\ell}} \bs \{ \hat{a}_{\ell,m_{\ell}}\}$ via $\{2,\ldots,|\mc{A}_{m_{\ell}}|\}$ and let $\Delta_i := \mu_0(\hat{a}_{\ell,m_{\ell}}) - \mu_0(i)$.

	Now, we will partition the values of $\Delta_{i}$ based on a grid of powers of $\rho$.
	Let
	\[
		N_{j,\ell} := \sum_{i=2}^{|\mc{A}_{m_{\ell}}|} \pmb{1}\{ \Delta_{i} \in \ho{\rho^{-(j+1)}}{\rho^{-j}} \},
	\]
	where $j$ ranges from $0$ to
	\[
		J := \ceil{  1 \vee \frac{1}{\beta} \log_{\rho} \left( \frac{\kappa_1}{36} \cdot \left( \frac{t_{\ell+1} - t_{\ell}^{m_{\ell}}}{\log(T)} \right)^{\frac{\beta}{\beta+1}} \right) }
	\]
	Then, we know $N_{j,\ell}$ has mean of $|A_{m_{\ell}}| - 1$ times the reservoir mass of sampling an arm with gap in $\ho{\rho^{-(j+1)}}{\rho^{-j}}$ which is

	First, by \Cref{lem:best-initial-arm} and \Cref{eq:small-variation-contradiction}, we have that:
	\[
		\forall t \in \ho{t_{\ell}^{m_{\ell}}}{t_{\ell+1}} : \delta_t(\hat{a}_{\ell,m_{\ell}}) \leq c_4 \left( \frac{\log(T)}{ ( t_{\ell+1} - t_{\ell} )^{\frac{1}{\beta+1}} } + \frac{\log(T)}{2^{m_{\ell} \cdot \frac{1}{\beta+1}}} \right) \leq c_5 \frac{\log(T)}{(t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}} },
	\]
	where we use the fact that $2^{m_{\ell}} \geq (t_{\ell+1} - t_{\ell})/2$ because of the doubling block structure.
	This means for arm $i \in \{2,\ldots,|\mc{A}_{m_{\ell}}|\}$, the initial gap to arm $\hat{a}_{\ell,m_{\ell}}$ is:
	\[
		1 - \mu_0(i) \leq 1 - \mu_0(\hat{a}_{\ell,m_{\ell}}) + \mu_0(\hat{a}_{\ell,m_{\ell}}) - \mu_0(i) \leq c_5 \frac{\log(T)}{(t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}}} + \Delta_{i},
		%\Delta_a := \mu_0(\hat{a}_{\ell,m_{\ell}}) - \mu_0(i) \leq 1 - \mu_0(i) + \frac{\log(T)}{( t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}}}.
	\]
	Now,
	\begin{align*}
	    \mb{P}( 1 - \rho^{-j} \leq \mu_0(a) < 1 - \rho^{-(j+1)} ) &= \mb{P}(1 - \rho^{-j} < \mu_0(a)) - \mb{P}( 1 - \rho^{-(j+1)} < \mu_0(a)) \\
		&\geq \kappa_1 \rho^{-j \cdot \beta} - \kappa_2 \rho^{-(j+1) \cdot \beta} \\
		&= (\kappa_1 - \kappa_2 \cdot \rho^{-\beta}) \cdot \rho^{-j \cdot \beta}.
		%&\gtrsim (|\mc{A}_{m_{\ell}}|-1) \cdot (\rho^{-j}).
	\end{align*}
	Now, by definition of $\rho$, we have
	\[
	    \kappa_1 - \kappa_2/\rho \geq \kappa_1/2.
	\]
	Thus, we conclude
	\[
		\mb{P}( 1 - \rho^{-j} \leq \mu_0(a) < 1 - \rho^{-(j+1)} ) \geq \frac{\kappa_1}{2 \rho^{j \cdot \beta}}.
	\]
	Then, by a multiplicative Chernoff bound from, we have letting $\eta_j := \mb{P}( 1 - \rho^{-j} \leq \mu_0(a) < 1 - \rho^{-(j+1)} )$,
	\[
	    \mb{P} \left( N_{j,\ell} \geq 2 (|\mc{A}_{m_{\ell}} | - 1) \cdot \eta_j \right) \leq \exp\left( - (|\mc{A}_{m_{\ell}}| - 1 ) \cdot \eta_j / 3 \right).
	\]
	The RHS is smaller than $T^{-3}$ since:
	\begin{align*}
		(|\mc{A}_{m_{\ell}}| - 1) \cdot \eta_j / 3 &\geq 2^{m_{\ell} \cdot \frac{\beta}{\beta+1}} \cdot \log^{\frac{1}{\beta+1}}(T) \cdot \frac{\kappa_1}{2  \cdot \rho^{j \cdot \beta}} \\
							   &\geq 2^{m_{\ell} \cdot \frac{\beta}{\beta+1}} \cdot \log^{\frac{1}{\beta+1}}(T) \cdot \frac{\kappa_1}{2  \cdot \rho^{J \cdot \beta}} \\
						       &\geq 6\log(T) \cdot \left( \frac{2^{m_{\ell}}}{t_{\ell+1} - t_{\ell}^{m_{\ell}}} \right)^{\frac{\beta}{\beta+1}} \\
						       &\geq 6\log(T) \cdot \left( \half \right)^{\frac{\beta}{\beta+1}} \\
						       &\geq 3\log(T),
						       %&\geq \log(T) \iff |\mc{A}_{m_{\ell}}| \gtrsim \frac{2 \rho^J}{\kappa_1} \cdot \log(T).
	\end{align*}
	where the third inequality uses the doubling block structure to bound $t_{\ell+1} - t_{\ell}^{m_{\ell}} \leq 2^{m_{\ell}+1}$.

	Let $\mc{E}_4$ be the corresponding high-probability event that
	\[
		\{N_{j,\ell}< 2 \cdot (|\mc{A}_{m_\ell}|-1) \cdot \eta_j ; \forall j,   \forall \ell\}
	\]
	Now, refining the sum over $i = 2, \ldots, |\mc{A}_{m_{\ell}}|$ into a geometric grid based on the values of the gaps and applying concentration over the number of gaps which fall within a particular segment of said grid.
	First, suppose that
	\begin{equation}\label{eq:grid-not-enough}
		\frac{1}{\rho^{J+1}} > 4 \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}} } \right)^{\frac{\beta}{\beta+1}}.
	\end{equation}
	Then, we can separately bound the number of gaps which fall between $\rho^{-(J+1)}$ and the RHS above.
	We have
	\begin{align*}
		\mb{P} \left( 1 - \rho^{-(J+1)} \leq \mu_0(a) < 1 - 4 \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}} } \right)^{\frac{\beta}{\beta+1}} \right) &\geq \kappa_1 \rho^{- \beta \cdot (J+1)} - \kappa_2 4^{\beta}  \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}}} \right)^{\frac{\beta^2}{\beta+1}} \\
																				       &\geq \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}}} \right)^{\frac{\beta}{\beta+1}} \cdot \left( 36 \cdot\rho^{-\beta} - \kappa_2 4^{\beta} \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}} } \right)^{\frac{\beta^2-\beta}{\beta+1}} \right)
	\end{align*}
	The second term in parentheses is $\Omega(1)$ for $t_{\ell+1} - t_{\ell}^{m_{\ell}}$ large enough.
	Specifically, we need
	\[
		18 \cdot \left( \frac{2 \kappa_2}{\kappa_1} \right)^{-\beta} \geq \kappa_2 4^{\beta} \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}} } \right)^{\frac{\beta^2-\beta}{\beta+1}}  \iff t_{\ell+1} - t_{\ell}^{m_{\ell}} \geq \left( \frac{ \kappa_2^{1+\beta} 2^{3\beta}  }{ \kappa_1^{\beta} 18} \right)^{\frac{\beta+1}{\beta^2 - \beta}} \cdot \log(T).
	\]
	This can be ensured by setting $C_1$ in \Cref{line:cpd-test} of \Cref{alg:blackbox} appropriately large.
	Specifically, we have by the definition of $t_{\ell+1}$ and the fact that the $\ell$-th episode ends in a restart that:
	\[
		t_{\ell+1} - t_{\ell}^m + 1 \geq C_1 \cdot |\mc{A}_{m_{\ell}}| \cdot \log(T) \geq C_1 \log(T).
	\]
	Thus,
	\[
		(|\mc{A}_{m_{\ell}}| - 1) \cdot \mb{P}\left( 1 - \rho^{-(J+1)} \leq \mu_0(a) < 1 - 4 \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}} } \right)^{\frac{\beta}{\beta+1}} \right) \gtrsim \log(T).
	\]


	Then, we can again use a multiplicative Chernoff bound to bound
	\[
		\sum_{i=2}^{|\mc{A}_{m_{\ell}}|} \pmb{1}\left\{ 4 \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}}} \right)^{\frac{\beta}{\beta+1}} < \Delta_{(i)} \leq \rho^{-(J+1)} \right\} \cdot \log(T) \cdot \left( \frac{t_{\ell+1} - t_{\ell}^{m_{\ell}}}{ \log(T) } \right)^{\frac{\beta}{\beta+1}} \lesssim |\mc{A}_{m_{\ell}}|.
	\]
	On the other hand, if \Cref{eq:grid-not-enough} does not hold, then the argument is simpler.
	%First, we note that
	%\[
		%\frac{1}{\rho^{J+1}} \leq \frac{36 \log^{\frac{\beta}{\beta+1}}(T)}{ \kappa_1 (t_{\ell+1} - t_{\ell}^{m_{\ell}})^{\frac{\beta}{\beta+1}} \cdot (2 \kappa_2 / \kappa_1) } = \frac{18 \log^{\frac{\beta}{\beta+1}}(T)}{ \kappa_2 (t_{\ell+1} - t_{\ell}^{m_{\ell}})^{\frac{\beta}{\beta+1}} } \leq 4 \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}} } \right)^{\frac{\beta}{\beta+1}}.
	%\]
	%\com{should be a $1/\beta$ power above}
	Then, every gap $\Delta_{(i)}$ such that $\Delta_{(i)}/4 \geq \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_{\ell}} } \right)^{\frac{\beta}{\beta+1}}$ lies in some interval $[\rho^{-(j+1)} , \rho^{-j} )$ for $j \in \{0,\ldots,J\}$.

    % By our regret decomposition \Cref{eq:regret-decomp} and the restart criterion (\Cref{line:restart}) of \Cref{alg:blackbox}, for $C_1$ large enough, this must mean that:
	% \[
	% 	\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} \mu_s(\hat{a}_{\ell}^m) - \mu_s(a_s) \gtrsim \sqrt{(t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T).
	% \]


	% Then, we want to show that the subsampled bandit environment over the episode is not mildly corrupt. \textcolor{red}{**jk: <-could you explain why?**}
	% \joe{basically, I want to arrive at a contradiction: if the subsampled bandit environment was only mildly corrupt, then the restart criterion (\Cref{line:restart}) would not be triggered.
	% Taking the contrapositive of this statement, I want to show that if the restart criterion is triggered, then the subsampled bandit environment must be more heavily corrupt.
	% }
	% In other words, by \Cref{assumption:base}, we want to show by contradiction that if it were mildly corrupt with stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with gaps $\{ \Delta_a\}_{a \in \mc{A}_0}$, then:
	% \begin{equation}\label{eq:bound-gap-rate}
	% 	C_2 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T) \right) > C_0 \left( \sum_{i=3}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}}} \right\}  + \sqrt{ (t_{\ell+1} - t_{\ell}) \cdot \log(T)} \right). %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, (t_{\ell+1} - t_{\ell}) \cdot \Delta_{(2)} \right\} \right),
	% \end{equation}
	% %for any stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with ordered gaps $\Delta_{(2)} \leq \Delta_{(3)} \leq \cdots \Delta_{(|\mc{A}_0|)}$.
	% We'll show this sub-claim by refining the sum over $i = 3, \ldots, |\mc{A}_0|$ into a geometric grid based on the values of the gaps and applying concentration over the number of gaps which fall within a particular segment of said grid.

	%For $j = 0, \ldots, \ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}^{m_\ell}}{\log(T)} \right) }(=: J)$, recall $N_{j,\ell} := \sum_{\jk{i=2}}^{|\mc{A}_{m_\ell}|} \pmb{1}\left\{ \Delta_{(\jk{i})} \in [ 2^{-(j+1)}, 2^{-j} ) \right\}$.
	Thus, we bound
	\begin{align}
		\sum_{i=2}^{|\mc{A}_{m_\ell}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \frac{\Delta_{(i)}}{4} \geq \left( \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_\ell}} \right)^{\frac{\beta}{\beta+1}} \right\} &\leq \sum_{j=0}^{J} N_{j,\ell} \cdot \rho^{j+1} \cdot \log(T) . \label{eq:gap-indicator-regret-bd}
	\end{align}
	% Recall $\mu_0(\hat{a}_{\ell,m_\ell})$ is the top initial reward of the arms $\mc{A}_{m_\ell}$ subsampled for block $\ho{t_{\ell}^{m_\ell}}{t_{\ell}^{m_\ell+1}}$.
	% Since, conditional on $\mu_0(\hat{a}_{\ell,m_\ell})$, the gaps are uniform random variables with order statistics $\Delta_{(2)},\ldots,\Delta_{(|\mc{A}_{m_\ell}|)}$, it is true that $N_{j,\ell}$ has mean $(|\mc{A}_{m_\ell}|\jk{-1}) \cdot 2^{-(j+1)}$. By a multiplicative Chernoff bound, with large enough constant $C_2>0$, we have:\jk{
	% \begin{align*}
	%     \mb{P}\left( N_{j,\ell} \geq 2 \cdot (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)} \mid \mu_0(\hat{a}_{\ell,m_\ell}) \right) &\leq \exp\left( - (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)} / 3 \right)\cr &\leq \exp\left( - (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(J+1)} / 3 \right)\cr &\leq \exp\left( - (C_22^{m_\ell/2}\sqrt{\log(T)}-1) \cdot \sqrt{\frac{\log(T)}{t_{\ell+1}-t_\ell^{m_\ell}}} / 12 \right)\cr &\leq \frac{1}{T^3}.
	% \end{align*}}
	% % The RHS is less than $T^{-3}$ for $t_{\ell+1} - t_{\ell}$ sufficiently larger than a constant. \jkc{<-Why this holds? Do we need additional $\log(T)$ for $|A_m|$?}


 % %    \jk{tbd..}
	% Using tower law, the tail probability bound also holds unconditional of $\mu_0(\hat{a}_{\ell,m_\ell}) $.
	% Let $\mc{E}_3$ be the corresponding high-probability event of $\{N_{j,\ell}< 2 \cdot (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)}; \forall j,   \forall \ell\}$.
    On event $\mc{E}_1 \cap \mc{E}_2 \cap \mc{E}_4$, we have $N_{j,\ell} < 2 \cdot |\mc{A}_{m_{\ell}}| \cdot \eta_j$.
    Furthermore,
    \[
	    \eta_j = \mb{P}( 1 - \rho^{j} \leq \mu_0(a) < 1 - \rho^{-(j+1)} ) \leq \mb{P}( 1 - \rho^{-j} < \mu_0(a)) \leq \kappa_2 \cdot \rho^{-j \cdot \beta}.
	\]
	Thus,
	\[
		N_{j,\ell} \cdot \rho^{j+1} < 2 \cdot \kappa_2 \cdot |\mc{A}_{m_{\ell}}| \cdot \rho^{j \cdot (1-\beta) + 1}.
	\]
	Now, by virtue of $\beta \geq 1$, we have $\rho^{j \cdot (1-\beta)}\leq 1$.
	Plugging the above into \Cref{eq:gap-indicator-regret-bd}, we obtain a bound of
	\begin{align*}
		\sum_{j=0}^J 2 \cdot \kappa_2 \cdot |\mc{A}_{m_{\ell}}| \cdot \left( \frac{ 2 \kappa_2}{\kappa_1} \right) &\leq \frac{ 4\kappa_2^2 }{\kappa_1} \cdot |\mc{A}_{m_{\ell}}| \cdot J \\
															  &\leq \frac{4 \kappa_2^2 }{\beta \kappa_1} \log_{\rho}\left( \frac{\kappa_1}{36} \cdot \left( \frac{t_{\ell+1} - t_{\ell}^{m_{\ell}}}{ \log(T) } \right)^{\frac{\beta}{\beta+1}} \right) \cdot |\mc{A}_{m_{\ell}}|  \\
															  &\leq \frac{4 \kappa_2^2}{ \beta \kappa_1 \log(2 \kappa_2 / \kappa_1)} \left( \log\left( \frac{\kappa_1}{36} \right) + \log(T) \right) \cdot |\mc{A}_{m_{\ell}}|.
	\end{align*}
	Now, for constant $C_1$ in \Cref{line:cpd-test} of \Cref{alg:blackbox} chosen appropriately large enough to dominate the constants in the above RHS, we have that \Cref{eq:blackbox-regret-small} holds.

    %%and so
		%%$N_{j,\ell} \cdot \rho^{j+1} \leq 2 \cdot |\mc{A}_{m_{\ell}}|.$ Thus, with \eqref{eq:gap-indicator-regret-bd}, we have
	%%\[
		%%\sum_{i=2}^{|\mc{A}_{m_\ell}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_\ell}}} \right\} \leq 2 \ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}^{m_\ell}}{\log(T)} \right) } \cdot |\mc{A}_{m_{\ell}}| \leq 2\log(T) \cdot |\mc{A}_{m_{\ell}}|,
	%%\]
	%%% Now,
	%%% \[
	%%% 	|\mc{A}_{m_\ell}| \leq 2C_2\cdot2^{(m_\ell-1)/2}\sqrt{\log(T)} \leq 2C_2 \sqrt{t_{\ell}^{m_\ell}-t_{\ell}^{m_\ell-1}}\sqrt{\log(T)}\le  \ceil{\sqrt{ t_{\ell+1} - t_{\ell}}}.
	%%% \]
%%which implies, for some positive constant $C>0$,
%\begin{equation}\label{eq:bound-gap-rate}
		%C \left(  |\mc{A}_{m_{\ell}}|\cdot \log(T)+\sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)}  \right) > C_0 \left( \sum_{i=\jk{2}}^{|\mc{A}_{m_{\ell}}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - \jk{t_{\ell}^{m_\ell}}}} \right\}  + \sqrt{ (t_{\ell+1} - \jk{t_{\ell}^{m_\ell}}) \cdot \log(T)} \right). %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, (t_{\ell+1} - t_{\ell}) \cdot \Delta_{(2)} \right\} \right),
	%\end{equation}
%
%
%% Then from Assumption~\ref{assumption:base}, under the mildy corrupt environment, we have
%% \jk{
%% \begin{align}\label{eq:bound-gap-rate-lower}
%%      C_0 \left( \sum_{i={2}}^{|\mc{A}_{m_{\ell}}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - {t_{\ell}^{m_\ell}}}} \right\}  + \sqrt{ (t_{\ell+1} - {t_{\ell}^{m_\ell}}) \cdot \log(T)} \right)\ge  \max_{a \in \mc{A}_{m_\ell}} \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(a) - \mu_t(a_t).
%% \end{align}
%From \eqref{eq:bound-gap-rate}, \eqref{eq:bound-gap-rate-lower},
%we have that
%\begin{align}&\sum_{t=t_\ell^m}^{t_{\ell+1}-1} 1-Y_t(a_t)\cr &\le \sum_{t=t_\ell^m}^{t_{\ell+1}-1}1-\mu_t(a_t)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
    %&\le  \sum_{t=t_\ell^m}^{t_{\ell+1}-1}1-\mu_t(\hat{a}_{\ell,m_\ell})+\mu_t(\hat{a}_{\ell,m_\ell})-\mu_t(a_t)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)
    %\cr
    %& \lesssim  \sum_{t=t_\ell^m}^{t_{\ell+1}-1}\mu_t(\hat{a}_{\ell,m_\ell})-\mu_t(a_t)+\sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
    %&\lesssim    \max_{a\in \mc{A}_{m_\ell}}\sum_{t=t_\ell^m}^{t_{\ell+1}-1}\mu_t(a)-\mu_t(a_t)+\sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
    %&< C_1\left( \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mc{A}_{m_{\ell}}|\cdot \log(T) \right),
%\end{align}
%where the first inequality is obtained from $\mc{E}_1$ and the thrid inequality is obtained from  $\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\lesssim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $.
%
%
%% Then from Assumption~\ref{assumption:base}, under the mildy corrupt environment, we have
%% {
%% \begin{align}\label{eq:bound-gap-rate-lower}
%%      C_0 \left( \sum_{i={2}}^{|\mc{A}_{m_{\ell}}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - {t_{\ell}^{m_\ell}}}} \right\}  + \sqrt{ (t_{\ell+1} - {t_{\ell}^{m_\ell}}) \cdot \log(T)} \right)\ge  \max_{a \in \mc{A}_{m_\ell}} \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(a) - \mu_t(a_t).
%% \end{align}
%% }{From \eqref{eq:bound-gap-rate}, \eqref{eq:bound-gap-rate-lower},
%% we have that
%% \begin{align}&\sum_{t=t_\ell^m}^{t_{\ell+1}-1} 1-Y_t(a_t)\cr &\le \sum_{t=t_\ell^m}^{t_{\ell+1}-1}1-\mu_t(a_t)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
%%     &\le  \sum_{t=t_\ell^m}^{t_{\ell+1}-1}1-\mu_t(\hat{a}_{\ell,m_\ell})+\mu_t(\hat{a}_{\ell,m_\ell})-\mu_t(a_t)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)
%%     \cr
%%     & \lesssim  \sum_{t=t_\ell^m}^{t_{\ell+1}-1}\mu_t(\hat{a}_{\ell,m_\ell})-\mu_t(a_t)+\sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
%%     &\lesssim    \max_{a\in \mc{A}_{m_\ell}}\sum_{t=t_\ell^m}^{t_{\ell+1}-1}\mu_t(a)-\mu_t(a_t)+\sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
%%     &< C_1\left( \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mc{A}_{m_{\ell}}|\cdot \log(T) \right),
%% \end{align}
%% where the first inequality is obtained from $\mc{E}_1$ and the thrid inequality is obtained from  $\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\lesssim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $.
%This contradicts to $\sum_{t=t_\ell^m}^{t_{\ell+1}-1} 1-Y_t(a_t)\ge C_1\left( \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mc{A}_{m_{\ell}}|\cdot \log(T) \right)$ from \Cref{line:cpd-test} in Algorithm~\ref{alg:blackbox}.
	This implies that the subsampled bandit environment over the last block $[t_\ell^m,t_{\ell+1})$ is \textit{not} mildly corrupt (\Cref{defn:mild}). Then, for any $\mu(\cdot): \mc{A}_{m_\ell}\rightarrow [0,1]$, there always exists $t'\in[t_\ell^m,t_{\ell+1})$ and $a'\in \mc{A}_{m_\ell}$ such that
\[
	|\mu_{t'}(a')-\mu(a')|> \frac{1}{(t_{\ell+1}-t_\ell^{m_\ell})^{\frac{1}{\beta+1}}}.
\]
% This means that since the adversary can only modify the rewards of arms $a_t$ after the round $t$, we have
% 	\[
% 		\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})|\ge   \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1}|\mu_{t}(a') - \mu_{t-1}(a')|\ge |\mu_{t'}(a') - \mu_{0}(a')| \geq \frac{1}{\sqrt{t_{\ell+1} - t_{\ell}^{m_\ell}}}.
% 	\]}

% This means there exists round $t'$ and arm $a' \in \mc{A}_{m_{\ell}}$ such that:
% \[
% 	|\mu_{t'}(a')-\mu_0(a')|>\frac{1}{\sqrt{t_{\ell+1}-t_\ell^{m_\ell}}}.
% \]
This means that since the adversary can only modify the rewards of arms $a_t$ after the round $t$, we have
\begin{align*}
\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})|&\ge
	\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})|\cr &\ge   \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1}|\mu_{t}(a') - \mu_{t-1}(a')|\cr &\ge |\mu_{t'}(a') - \mu_{0}(a')| \cr & \geq \frac{1}{ (t_{\ell+1} - t_{\ell}^{m_\ell})^{\frac{1}{\beta+1}}}\cr & \geq \frac{1}{ (t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}} }.
\end{align*}

%% We first show that the variation over the episode is large, i.e. \[\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})| \gtrsim (t_{\ell+1} - t_{\ell})^{-1/2}.\]
%%For large enough choice of threshold $C_1>0$ in \Cref{line:cpd-test}, we have that a restart in the $\ell$-th episode corresponds to large regret for the final block $\ho{t_{\ell}^{m_\ell}}{t_{\ell+1}}$, so that under $\mc{E}_1$, for some constant $C>0$, we have
	%%\begin{equation}\label{eq:large-regret-last-block}
		%%\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_t(a_t) \geq C \left( \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) \right).
	%%\end{equation}
%Let $\hat{a}_{\ell,m}$ be the best arm in terms of initial reward among the arms $\mc{A}_m$ subsampled for block $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$.    We can decompose the regret  in the final block of the episode as
		%\[
			%\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_t(a_t) = \sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell}) + \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t).
		%\]
%% Then, it remains to show on event $\mc{E}_1 \cap \mc{E}_2$ that either (a) the regret of the best subsampled arm is large (indicating large variation) or (b) the subsampled bandit environment over the rounds $\ho{t_{\ell}^m}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).
%
	%% Then, for large enough choice of threshold $C_1>0$ in \Cref{line:cpd-test}, we have that a restart in the $\ell$-th episode corresponds to large regret for the final block $\ho{t_{\ell}^m}{t_{\ell+1}}$:
	%% \begin{equation}\label{eq:large-regret-last-block}
	%% 	\sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(a_s) \geq C_2 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T) \right).
	%% \end{equation}
	%% Now, let $\mc{E}_2$ be the high-probability event of \Cref{assumption:base} holds.
    %\jk{Then from \eqref{eq:large-regret-last-block}, we can consider the following two possible cases; one is $\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\gtrsim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $ and the other is $\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\lesssim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $ and $\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t)\gtrsim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $.}
%
%We first consider the former case of $\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\gtrsim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $, where the regret of the best subsampled arm is large (indicating large variation).
%% Let $\mu_0(a)$ denote the initial mean reward of arm $a$.
%% Since
%% 	\begin{align*}
%% 		 \mb{P}\left(\mu_0(\hat{a}_{\ell,m_\ell}) < 1 - \jk{\log(T)} 2^{-m_{\ell}/2}\right)&=      \jk{\mb{P}\left(\max_{a\in \mathcal{A}_{m_\ell}}\mu_0(a) < 1 - \log(T) 2^{- m_{\ell}/2}\right)}    \\&\leq \left( 1 - \frac{\log(T)}{2^{m_{\ell}/2}} \right)^{|\mc{A}_{\jk{m_\ell}}|} \\
%%         &\leq \exp\left( - |\mc{A}_{\jk{m_\ell}}| \cdot \frac{\log(T)}{ 2^{m_{\ell}/2}} \right) \\
%% 		&\leq \frac{1}{T},
%% 	\end{align*}
%% 	where the last inequality follows from $|\mc{A}_{\jk{m_\ell}}| \geq 2^{m_{\ell}/2}$, we have,  with probability at least $1-1/T$,
%From $\mc{E}_3$, we have
%\begin{align}
    	%\mu_0(\hat{a}_{\ell,m_\ell}) > 1 - \frac{\log(T)}{2^{m_{\ell}/2}} \geq 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^{m_\ell}}}.\label{eq:goodness-best-subsmapled-arm}
%\end{align}
    %From the above tail probability bound, we know $1-\mu_0(\hat{a}_{\ell,m_\ell}) < \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}$.
	%From \eqref{eq:large-regret-last-block} (with large enough $C_1>0$), we also know that there exists a round $t' \in \ho{t_{\ell}^m}{t_{\ell+1}}$ such that
	%\[
		%1- \mu_{t'}(\hat{a}_{\ell,m_\ell}) > \frac{2\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^{m_\ell}}}.
	%\]
	%This means the mean reward of arm $\hat{a}_{\ell,m_\ell}$ must have moved by amount at least $\frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^{m_\ell}}} \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}$ over the course of the block, implying \jk{
%\[\mu_0(\hat{a}_{\ell,m_\ell})-\mu_{t'}(\hat{a}_{\ell,m_\ell})\ge \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^{m_\ell}}} \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}.\]
   %}
	%Since the adversary can only modify the rewards of an arm $a_t$ after the round $t$ it is played, the movement must have occurred on rounds where $\hat{a}_{\ell,m_\ell}$ was chosen by the agent.
	%Thus,
	%\[
		%\jk{\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})|\ge \sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(\hat{a}_{\ell,m_\ell}) - \mu_{t-1}(\hat{a}_{\ell,m_\ell})|\ge \mu_0(\hat{a}_{\ell,m_\ell})-\mu_{t'}(\hat{a}_{\ell,m_\ell}) \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}.}
	%\]
%
%
%% 	Then, it remains to show on event $\mc{E}_1 \cap \mc{E}_2$ that either (a) the regret of the best subsampled arm is large (indicating large variation) or (b) the subsampled bandit environment over the rounds $\ho{t_{\ell}^m}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).  \textcolor{red}{**JK: Could you explain this for me?**}
%% 	\joe{sorry this explanation was rushed. Using the notation from below, we can decompose the regret  in the final block of the episode as
%% 		\[
%% 			\sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(a_s) = \sum_s 1 - \mu_s(\hat{a}_{\ell,m}) + \sum_s \mu_s(\hat{a}_{\ell,m}) - \mu_s(a_s).
%% 		\]
%% 		Thus, we know from \Cref{eq:large-regret-last-block} that one of the two sums on the RHS above is large.
%% 		If the first sum is large, we want to show this implies large variation must have elapsed in the episode.
%% 		Our goal is to show in both situations that the variation over the episode is large or that $\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \gtrsim (t_{\ell+1} - t_{\ell})^{-1/2}$.\textcolor{red}{*jk: in the middle*}
%% 	}
%
%% 	Let $\hat{a}_{\ell,m}$ be the best arm in terms of initial reward among the arms $\mc{A}_m$ subsampled for block $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$.
%% 	We first argue that with probability at least $1-1/T$,
%% 	\[
%% 		\mu_0(\hat{a}_{\ell,m}) > 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}.
%% 	\]
%% 	This is true since
%% 	\begin{align*}
%% 		\mb{P}(\mu_0(\hat{a}_{\ell,m}) < 1 - (t_{\ell+1} - t_{\ell}^m)^{-1/2}) &\leq \left( 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \right)^{|\mc{A}_0|} \\
%% 										       &\leq \exp\left( - |\mc{A}_0| \cdot \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \right) \\
%% 										       &\leq \frac{1}{T},
%% 	\end{align*}
%% 	where the last inequality follows from $|\mc{A}_0| \geq \sqrt{t_{\ell+1} - t_{\ell}^m}$.
%
%% 	Now, using the regret decomposition of \Cref{eq:regret-decomp}, if
%% 	\begin{equation}\label{eq:bad-reg-best}
%% 		\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(\hat{a}_{\ell,m}) > 2\log(T)\sqrt{t_{\ell+1} - t_{\ell}^m},
%% 	\end{equation}
%% 	then we must have with probability at least $1/T$ that the variation must be at least
%% 	\[
%% 		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}},
%% 	\]
%% 	since the adversary can only modify the rewards of arms $a_t$ after the round $t$ they're played. \textcolor{red}{**JK: Could you explain this for me?**}
%% 	\joe{
%% 	From our earlier tail probability bound, we know $\delta_0(\hat{a}_{\ell,m}) < \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}$.
%% 	We also know from (3) above that there exists a round $t \in \ho{t_{\ell}^m}{t_{\ell+1}}$ such that
%% 	\[
%% 		\delta_t(\hat{a}_{\ell,m}) > \frac{2\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}.
%% 	\]
%% 	This means the gap of arm $\hat{a}_{\ell,m}$ must have moved by amount $\frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}$ over the course of the block.
%% 	Since the adversary can only modify the rewards of an arm $a_t$ after the round $t$ it is played, this must have occurred on a round where $\hat{a}_{\ell,m}$ was chosen by the agent.
%% 	Thus,
%% 	\[
%% 		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}.
%% 	\]
%
%% }
%
	%% Suppose, going forward that \Cref{eq:bad-reg-best} is reversed.
%
	%Now, we consider the other case of $\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t)\gtrsim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $, where the regret of the subsampled bandit environment over the rounds $\ho{t_{\ell}^{m_\ell}}{t_{\ell+1}}$ is large, while $\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\lesssim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $.   We want to show that the subsampled bandit environment over the last block of each episode is not mildly corrupt by a contradiction.  From \Cref{assumption:base}, if it were mildly corrupt with stationary reward profile \jk{$\{\mu_0(a)\}_{a \in \mc{A}_{m_\ell}}$ with gaps $\{ \Delta_a\}_{a \in \mc{A}_{m_\ell}}$} (Definition~\ref{defn:mild}), then we can show that:
%\begin{equation}
		%C_1 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mc{A}_{m_{\ell}}|\cdot \log(T) \right) > \sum_{t=t_\ell^m}^{t_{\ell+1}-1} 1-Y_t(a_t).
        %%\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, (t_{\ell+1} - t_{\ell}) \cdot \Delta_{(2)} \right\} \right),
	%\end{equation}
    %This statement can be proven as follows. By refining the sum over $i = 2, \ldots, |\mc{A}_{m_{\ell}}|$ into a geometric grid based on the values of the gaps and applying concentration over the number of gaps which fall within a particular segment of said grid.
%
    %% By our regret decomposition \Cref{eq:regret-decomp} and the restart criterion (\Cref{line:restart}) of \Cref{alg:blackbox}, for $C_1$ large enough, this must mean that:
	%% \[
	%% 	\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} \mu_s(\hat{a}_{\ell}^m) - \mu_s(a_s) \gtrsim \sqrt{(t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T).
	%% \]
%
%
	%% Then, we want to show that the subsampled bandit environment over the episode is not mildly corrupt. \textcolor{red}{**jk: <-could you explain why?**}
	%% \joe{basically, I want to arrive at a contradiction: if the subsampled bandit environment was only mildly corrupt, then the restart criterion (\Cref{line:restart}) would not be triggered.
	%% Taking the contrapositive of this statement, I want to show that if the restart criterion is triggered, then the subsampled bandit environment must be more heavily corrupt.
	%% }
	%% In other words, by \Cref{assumption:base}, we want to show by contradiction that if it were mildly corrupt with stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with gaps $\{ \Delta_a\}_{a \in \mc{A}_0}$, then:
	%% \begin{equation}\label{eq:bound-gap-rate}
	%% 	C_2 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T) \right) > C_0 \left( \sum_{i=3}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}}} \right\}  + \sqrt{ (t_{\ell+1} - t_{\ell}) \cdot \log(T)} \right). %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, (t_{\ell+1} - t_{\ell}) \cdot \Delta_{(2)} \right\} \right),
	%% \end{equation}
	%% %for any stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with ordered gaps $\Delta_{(2)} \leq \Delta_{(3)} \leq \cdots \Delta_{(|\mc{A}_0|)}$.
	%% We'll show this sub-claim by refining the sum over $i = 3, \ldots, |\mc{A}_0|$ into a geometric grid based on the values of the gaps and applying concentration over the number of gaps which fall within a particular segment of said grid.
%
	%For $j = 0, \ldots, \ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}^{m_\ell}}{\log(T)} \right) }(=: J)$, recall $N_{j,\ell} := \sum_{\jk{i=2}}^{|\mc{A}_{m_\ell}|} \pmb{1}\left\{ \Delta_{(\jk{i})} \in [ 2^{-(j+1)}, 2^{-j} ) \right\}$.
	%Then, we bound
	%\begin{align}
		%\sum_{i=2}^{|\mc{A}_{m_\ell}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_\ell}}} \right\} &\leq \sum_{j=0}^{\ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}^{m_\ell}}{\log(T)} \right) }} N_{j,\ell} \cdot 2^{j+1}.\label{eq:gap-indicator-regret-bd}
	%\end{align}
	%% Recall $\mu_0(\hat{a}_{\ell,m_\ell})$ is the top initial reward of the arms $\mc{A}_{m_\ell}$ subsampled for block $\ho{t_{\ell}^{m_\ell}}{t_{\ell}^{m_\ell+1}}$.
	%% Since, conditional on $\mu_0(\hat{a}_{\ell,m_\ell})$, the gaps are uniform random variables with order statistics $\Delta_{(2)},\ldots,\Delta_{(|\mc{A}_{m_\ell}|)}$, it is true that $N_{j,\ell}$ has mean $(|\mc{A}_{m_\ell}|\jk{-1}) \cdot 2^{-(j+1)}$. By a multiplicative Chernoff bound, with large enough constant $C_2>0$, we have:\jk{
	%% \begin{align*}
	%%     \mb{P}\left( N_{j,\ell} \geq 2 \cdot (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)} \mid \mu_0(\hat{a}_{\ell,m_\ell}) \right) &\leq \exp\left( - (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)} / 3 \right)\cr &\leq \exp\left( - (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(J+1)} / 3 \right)\cr &\leq \exp\left( - (C_22^{m_\ell/2}\sqrt{\log(T)}-1) \cdot \sqrt{\frac{\log(T)}{t_{\ell+1}-t_\ell^{m_\ell}}} / 12 \right)\cr &\leq \frac{1}{T^3}.
	%% \end{align*}}
	%% % The RHS is less than $T^{-3}$ for $t_{\ell+1} - t_{\ell}$ sufficiently larger than a constant. \jkc{<-Why this holds? Do we need additional $\log(T)$ for $|A_m|$?}
%
%
 %% %    \jk{tbd..}
	%% Using tower law, the tail probability bound also holds unconditional of $\mu_0(\hat{a}_{\ell,m_\ell}) $.
	%% Let $\mc{E}_3$ be the corresponding high-probability event of $\{N_{j,\ell}< 2 \cdot (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)}; \forall j,   \forall \ell\}$.
%
    %On event $\mc{E}_1 \cap \mc{E}_2 \cap \mc{E}_4$, we have $N_{j,\ell} < 2 \cdot |\mc{A}_{m_{\ell}}| \cdot 2^{-(j+1)}$ and so
		%$N_{j,\ell} \cdot 2^{j+1} \leq 2 \cdot |\mc{A}_{m_{\ell}}|.$ Thus, with \eqref{eq:gap-indicator-regret-bd}, we have
	%\[
		%\sum_{i=2}^{|\mc{A}_{m_\ell}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}^{m_\ell}}} \right\} \leq 2 \ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}^{m_\ell}}{\log(T)} \right) } \cdot |\mc{A}_{m_{\ell}}| \leq 2\log(T) \cdot |\mc{A}_{m_{\ell}}|,
	%\]
	%% Now,
	%% \[
	%% 	|\mc{A}_{m_\ell}| \leq 2C_2\cdot2^{(m_\ell-1)/2}\sqrt{\log(T)} \leq 2C_2 \sqrt{t_{\ell}^{m_\ell}-t_{\ell}^{m_\ell-1}}\sqrt{\log(T)}\le  \ceil{\sqrt{ t_{\ell+1} - t_{\ell}}}.
	%% \]
%which implies, for some positive constant $C>0$,
%\begin{equation}\label{eq:bound-gap-rate}
		%C \left(  |\mc{A}_{m_{\ell}}|\cdot \log(T)+\sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)}  \right) > C_0 \left( \sum_{i=\jk{2}}^{|\mc{A}_{m_{\ell}}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - \jk{t_{\ell}^{m_\ell}}}} \right\}  + \sqrt{ (t_{\ell+1} - \jk{t_{\ell}^{m_\ell}}) \cdot \log(T)} \right). %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, (t_{\ell+1} - t_{\ell}) \cdot \Delta_{(2)} \right\} \right),
	%\end{equation}
%
%
%Then from Assumption~\ref{assumption:base}, under the mildy corrupt environment, we have
%\begin{align}\label{eq:bound-gap-rate-lower}
     %C_0 \left( \sum_{i={2}}^{|\mc{A}_{m_{\ell}}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - {t_{\ell}^{m_\ell}}}} \right\}  + \sqrt{ (t_{\ell+1} - {t_{\ell}^{m_\ell}}) \cdot \log(T)} \right)\ge  \max_{a \in \mc{A}_{m_\ell}} \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(a) - \mu_t(a_t).
%\end{align}
%From \eqref{eq:bound-gap-rate}, \eqref{eq:bound-gap-rate-lower},
%we have that
%\begin{align}&\sum_{t=t_\ell^m}^{t_{\ell+1}-1} 1-Y_t(a_t)\cr &\le \sum_{t=t_\ell^m}^{t_{\ell+1}-1}1-\mu_t(a_t)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
    %&\le  \sum_{t=t_\ell^m}^{t_{\ell+1}-1}1-\mu_t(\hat{a}_{\ell,m_\ell})+\mu_t(\hat{a}_{\ell,m_\ell})-\mu_t(a_t)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)
    %\cr
    %& \lesssim  \sum_{t=t_\ell^m}^{t_{\ell+1}-1}\mu_t(\hat{a}_{\ell,m_\ell})-\mu_t(a_t)+\sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
    %&\lesssim    \max_{a\in \mc{A}_{m_\ell}}\sum_{t=t_\ell^m}^{t_{\ell+1}-1}\mu_t(a)-\mu_t(a_t)+\sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T)+3\sqrt{3(t_{\ell+1}-t_\ell^m)\log(2T)}+6\log(2T)\cr
    %&< C_1\left( \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mc{A}_{m_{\ell}}|\cdot \log(T) \right),
%\end{align}
%where the first inequality is obtained from $\mc{E}_1$ and the third inequality is obtained from  $\sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell})\lesssim \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mathcal{A}_{m_\ell}|\log(T) $.
%% This means there exists round $t'$ and arm $a' \in \mc{A}_{m_{\ell}}$ such that:
%% \[
%% 	|\mu_{t'}(a')-\mu_0(a')|>\frac{1}{\sqrt{t_{\ell+1}-t_\ell^{m_\ell}}}.
%% \]
%
%This contradicts to $\sum_{t=t_\ell^m}^{t_{\ell+1}-1} 1-Y_t(a_t)\ge C_1\left( \sqrt{ (t_{\ell+1} - t_{\ell}^{m_\ell}) \log(T)} + |\mc{A}_{m_{\ell}}|\cdot \log(T) \right)$ from \Cref{line:cpd-test} in Algorithm~\ref{alg:blackbox}. This implies that the subsampled bandit environment over the last block $[t_\ell^m,t_{\ell+1})$ is \textit{not} mildly corrupt (\Cref{defn:mild}). Then, for any $\mu(\cdot): \mc{A}_{m_\ell}\rightarrow [0,1]$, there always exists $t'\in[t_\ell^m,t_{\ell+1})$ and $a'\in \mc{A}_{m_\ell}$ such that
%\[|\mu_{t'}(a')-\mu(a')|>\frac{1}{\sqrt{t_{\ell+1}-t_\ell^{m_\ell}}}.\]
%
%This means that since the adversary can only modify the rewards of arms $a_t$ after the round $t$, we have
%\begin{align*}
%\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})|&\ge
		%\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})|\cr &\ge   \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1}|\mu_{t}(a') - \mu_{t-1}(a')|\cr &\ge |\mu_{t'}(a') - \mu_{0}(a')| \cr & \geq \frac{1}{\sqrt{t_{\ell+1} - t_{\ell}^{m_\ell}}}\cr & \geq \frac{1}{\sqrt{t_{\ell+1} - t_{\ell}}}.
%\end{align*}

\subsection{Showing Best Initial Arm has Small Gap (Proof of \Cref{lem:best-initial-arm})}\label{subsec:proof-best-initial-arm}

%We first assert that the best initial arm $\hat{a}_{\ell,m_{\ell}}$ has small initial gap.
Let $\mu_0(a)$ denote the initial mean reward of arm $a$.
By \Cref{ass:reservoir}, we have
	\begin{align*}
		\mb{P}\left(\mu_0(\hat{a}_{\ell,m_\ell}) \leq 1 - \frac{2  \log^2(T)}{2^{m_{\ell} \cdot \frac{1}{\beta+1}}} \right) &=      \mb{P}\left(\max_{a\in \mathcal{A}_{m_\ell}}\mu_0(a) \leq 1 - \frac{2  \log^2(T)}{2^{m_{\ell} \cdot \frac{1}{\beta+1}}} \right)    \\
																		     &\leq \left( 1 - \mb{P}\left( \mu_0(a) > 1 - \frac{2  \log^2(T)}{2^{m_{\ell} \cdot \frac{1}{\beta+1}}} \right) \right)^{|\mc{A}_{m_{\ell}}|} \\
																&\leq  \left( 1 - \kappa_1 \left( \frac{2 \log^2(T)}{2^{m_{\ell} \cdot \frac{1}{\beta+1}}} \right)^{\beta} \right)^{|\mc{A}_{{m_\ell}}|} \\
																&\leq \exp\left( - |\mc{A}_{{m_\ell}}| \cdot \left( \frac{2\log(T)}{ 2^{m_{\ell} \cdot \frac{1}{\beta+1}}} \right)^{\beta} \right) \\
		&\leq \frac{1}{T^2},
	\end{align*}
	where the fourth line follows from $\log(T) \geq \kappa_1^{-1/\beta}$ and
	where the last inequality follows from $|\mc{A}_{m_\ell}| \geq 2^{m_{\ell} \cdot \frac{\beta}{\beta+1}}$.
	%\com{interestingly, the proof here only requires the lower bound of \Cref{ass:reservoir} and not the upper bound}
	%We define $\mc{E}_3$ to be the corresponding high-probability event of $ \{ \forall \ell \in [\hat{L}]: 1-\mu_0(\hat{a}_{\ell,m_\ell}) \le 2\log(T) \cdot 2^{-m_\ell \cdot \frac{1}{\beta+1}} \}$, which holds with at least probability of $1-1/T$.



\subsection{Summing Regret Over Episodes (Proof of \Cref{lem:regret-bd-nonstationarity})}

Now, we show that how to derive
\[
	\sum_{\ell=1}^{\hat{L}} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}} \leq (L+1)^{\frac{1}{\beta+1}} \cdot T^{\frac{\beta}{\beta+1}} \land (V^{\frac{1}{\beta+2}} T^{\frac{\beta+1}{\beta+2}} + T^{\frac{\beta}{\beta+1}}),
\]
from the fact that, as we have shown by \Cref{lem:variation-bound}, for all episodes $\ell\in [\hat{L}-1]$
\[
	\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})|\ge \frac{1}{ (t_{\ell+1} - t_{\ell})^{\frac{1}{\beta+1}}}.
\]
We first show the bound in terms of total variation $V$.
Let $V_{[s_1,s_2)} := \sum_{t=s_1}^{s_2-1}|\mu_t(a_{t-1})-\mu_{t-1}(a_{t-1})|$. Then, by using Hölder's inequality:
\begin{align*}
	\sum_{\ell=1}^{\hat{L}} (t_{\ell+1}-t_\ell)^{\frac{\beta}{\beta+1}} &\le T^{\frac{\beta}{\beta+1}} + \left(\sum_{\ell=1}^{\hat{L}-1} \frac{1}{(t_{\ell+1}-t_\ell)^{\frac{1}{\beta+1}}} \right)^{\frac{1}{\beta+2}} \left( \sum_{\ell=1}^{\hat{L}-1} t_{\ell+1}-t_\ell \right)^{\frac{\beta+1}{\beta+2}} \\
									    &\le T^{\frac{\beta}{\beta+1}} + \left(\sum_{\ell=1}^{\hat{L}-1} V_{[t_\ell, t_{\ell+1})} \right)^{\frac{1}{\beta+2}} T^{\frac{\beta+1}{\beta+2}} &\cr &\le T^{\frac{\beta}{\beta+1}} + V^{\frac{1}{\beta+2}} T^{\frac{\beta+1}{\beta+2}}.
\end{align*}

% Then, we also have
% \begin{align*}
%     \sum_{\ell=1}^{\hat{L}}\sqrt{t_{\ell+1}-t_\ell}&\le \left(\sum_{\ell=1}^{\hat{L}}\sqrt{\frac{1}{t_{\ell+1}-t_\ell}}\right)^{1/2}\left(\sum_{\ell=1}^{\hat{L}}t_{\ell+1}-t_\ell\right)^{1/2}\cr &\le \left(\sum_{\ell=1}^{\hat{L}}V_{[t_\ell, t_{\ell+1})}\right)^{1/3}T^{2/3}&\cr &\le V^{1/3}T^{2/3}.
% \end{align*}

To show the bound in terms of $L$, we use Jensen's inequality on the function $x \mapsto x^{\frac{\beta}{\beta+1}}$ combined with the fact that the number of episodes $\hat{L} \leq L+1$ by virtue of \Cref{lem:variation-bound}.

%\jk{Here we show that $\hat{L}\le L+1$. Let $L_{[s_1,s_2)}=\sum_{t=s_1}^{s_2-1}\textbf{1}\{\mu_t(a_{t-1})\neq \mu_{t-1}(a_{t-1})\}$.  The proof is by contradiction, assuming that episode $\ell$ is terminated at $t>t_{\ell}^{m_\ell}$ but $L_{[t_\ell^{m_\ell},t+1)}=0$. Then from the detection condition of \Cref{line:cpd-test},  under $\mc{E}_1$, for some large enough $C>0$ we have
%$\sum_{s=t_\ell^{m_\ell}}^t 1-\mu_s(a_s)\ge C(\sqrt{(t-t_{\ell}^{m_\ell}+1)\log(T)}+|\mc{A}_{m_\ell}|\cdot \log(T)).$ This contradicts the stationary condition for $L_{[t_\ell^{m_\ell},t+1)}=0$ because, under the stationary environment, we have
%\begin{align*}
%\sum_{s=t_\ell^{m_\ell}}^t 1-\mu_s(a_s)&=  \sum_{s=t_\ell^{m_\ell}}^t 1-\mu_0(\hat{a}_{\ell,m_\ell})+\mu_0(\hat{a}_{\ell,m_\ell})-\mu_0(a_s)\cr &\le  \sum_{s=t_\ell^{m_\ell}}^t\frac{\log(T)}{\sqrt{t+1-t_\ell^{m_\ell}}}+C_0 \left( \sum_{i={2}}^{|\mc{A}_{m_{\ell}}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t+1 - {t_{\ell}^{m_\ell}}}} \right\}  + \sqrt{ (t+1- {t_{\ell}^{m_\ell}}) \cdot \log(T)} \right)
%\cr &<C \left(\sqrt{(t-t_{\ell}^{m_\ell}+1)\log(T)}+|\mc{A}_{m_\ell}|\cdot \log(T)\right),
%\end{align*}
%where the first inequality is obtained from \eqref{eq:goodness-best-subsmapled-arm} and $\mc{E}_1$.
%Therefore, we have $L_{[t_\ell^{m_\ell},t_{\ell+1})}\neq 0$ (except the last episode when it ends by reaching $T$) implying $\hat{L}\le L+1$. Then, by using Jensen's inequality, we have
%\[\sum_{\ell=1}^{\hat{L}}\sqrt{t_{\ell+1}-t_\ell}\le \sqrt{\hat{L}T}\le \sqrt{(L+1)T},\]
%which concludes the proof.}

\subsection{Proof of \Cref{thm:blackbox} for $\beta < 1$}\label{subsec:beta-small}

The proof for $\beta < 1$ will follow the same steps except Lemma 4 will be based on securing an arm with gap $1/2^{m_{\ell}/2}$, Lemma 5 will instead use a bound of $(t_{\ell+1} - t_{\ell})^{-1/2}$, and Lemma 6 will use the $\beta=1$ rate.

The analogue of Lemma 4 holds for the chosen subsampling rate of $S_m \propto 2^{m\cdot \beta/2}$.
The analogue of Lemma 5 holds by following the same proof except invoking Assumption 2 using $\alpha=1$ instead of $\alpha=\beta$.


==> scrap/blackbox_old.tex <==
\section{A Blackbox for Optimally Tracking Unknown Non-Stationarity}\label{sec:blackbox}

A key idea, introduced for the stationary problem in \citet{bayati20}, is that of {\em subsampling} a finite number of arms from the reservoir.
The main algorithmic design principle is to then run a finite-armed MAB algorithm over the subsampled arms.
The choice of number of arms to subsample is key here and exhibits its own exploration-exploitation tradeoff.
This tradeoff is best exemplified through the natural regret decomposition with respect to the subsampled set of arms, which we'll denote by $\mc{A}_0 \subseteq \mc{A}$:
%For minimizing regret over $T$ rounds, the minimax optimal regret of $\sqrt{T}$ can be achieved by subsampling $\sqrt{T}$ arms.

%In particular, within a sample of $\sqrt{T}$ arms, with high probability at least one arm will have reward at least $1-1/\sqrt{T}$.
%Then, it turns out one can reduce the problem to finite-armed bandits by subsampling $\sqrt{T}$ arms and then bounding regret between the subsampled arms:
%Thentural regret decomposition induced by a subsampled set of arms $\mc{A}_0$:
\begin{equation}\label{eq:regret-decomp}
	\sum_{t=1}^T \delta(a_t) = \underbrace{ \sum_{t=1}^T  1 - \max_{a \in \mc{A}_0} \mu(a)}_{\text{Regret of best subsampled arm}}  + \underbrace{ \sum_{t=1}^T  \max_{a \in \mc{A}_0} \mu(a) - \mu(a_t)}_{\text{Regret of played arms to best subsampled arm}}.
\end{equation}
Let's suppose there are $K := |\mc{A}_0|$ subsampled arms.
Then, a sample of $K$ arms drawn from $\Unifu$ contains, with high probability, an arm with reward at least $1-1/K$ and, thus, gap at most $1/K$.
Thus, the first sum in \Cref{eq:regret-decomp} is at most $T/K$.

Then, plugging in the classical gap-dependent regret bounds for finite-armed MAB, the second term in \Cref{eq:regret-decomp} is $\tilde{O}\left( \sum_{a \in \mc{A}_0 \bs \argmax_{a' \in \mc{A}_0} \mu(a')} \Delta_{a}^{-1} \right)$ where $\Delta_{a}$ is the (random) gap of $a$ to the best subsampled arm.
Then, it is further shown \citep[Section A.2]{bayati20} that this gap-dependent quantity scales like $K\log(T)$ in expectation.

Then, we may choose $K$ to balance the bounds $T/K$ and $K \cdot \log(T)$ for which $K \propto \sqrt{T}$ is optimal giving a regret bound of $\sqrt{T}$.
As it turns out, the $\sqrt{T}$ regret rate is minimax.

Extending this to the non-stationary problem, it is first natural to ask whether we can follow the same strategy using a reduction to finite-armed non-stationary bandits.
However, this strategy poses two key difficulties:
\begin{enumerate}[(a)]
	\item Firstly, it's quite crucial in the above argument that the logarithmic gap-dependent regret bound was plugged in and not the gap-independent worst-case bound of $\sqrt{K T}$ (which would only lead to a suboptimal $T^{2/3}$ bound when optimizing $K$).

	As our goal in the non-stationary problem is to achieve {\em adaptive} regret bounds, free of parameter knowledge, a natural proposal is to reduce to $K$-armed non-stationary bandits and employ the known adaptive algorithms for this setting \citep{auer2019,wei2021,suk22,abbasi22}.
	However, it's long been known in this literature that no algorithm can adaptively secure a gap-dependent regret of $\sum_{\ell=1}^L \frac{K}{\Delta_{\ell,\min}}$ over $L$ stationary phases with minimal gaps $\Delta_{\ell,\min}$ \citep{garivier2011,lattimore}.
	This suggests we cannot do a full blackbox reduction to finite-armed non-stationary bandits.
	\item Secondly, we observe that upon experiencing changes, it may be necessary to {\em re-sample} arms from the reservoir distribution or else the first sum in \Cref{eq:regret-decomp} can become large if the rewards of all arms in $\mc{A}_0$ degrade over time.
	Thus, we require a more refined subsampling strategy which works in tandem with non-stationarity detection.
\end{enumerate}

We handle both of the above issues with the new idea of tracking the empirical regret $1 - Y_t(a_t)$ as a proxy for tracking non-stationarity.
The key observation is that the empirical cumulative regret of played actions up to round $t$, $\sum_{s=1}^t 1 - Y_s(a_s)$, concentrates around $\sum_{s=1}^t 1 - \mu_s(a_s)$ at a rate of $\sqrt{t}$ by Freedman's inequality.

This means, so long as $\sum_{s=1}^t 1 - Y_s(a_s) \lesssim \sqrt{t}$, our regret will be safe up to stationary rates.
On the other hand, if $\sum_{s=1}^t 1 - Y_s(a_s) \gg \sqrt{t}$, then the learner must be experiencing large regret.

On the other side, if the agent is playing according to an optimal algorithm for stationary infinite-armed bandits, then the only way large empirical regret is observed is if large non-stationarity has occurred.
Hence, checking empirical regret is a valid changepoint detection test.

Putting these observations together, our procedure (\Cref{alg:blackbox}), similar to the adaptive algorithms for the finite-armed setting \citep{auer2019,wei2021,suk22,abbasi22}, proceeds in episodes and restarts upon detecting non-stationarity.
A restart, or new episode, is triggered when the empirical regret over the current episode becomes too large.
Within each episode, we further employ doubling epochs, termed {\em blocks}, to account for unknown horizons and changepoints.


Going into more detail, our blackbox will rely on a stochastic finite-armed MAB base algorithm designed for stochastic environments, which we'll denote by $\base(t,\mc{A}_0)$, taking as input a horizon $t$ and finite subsample $\mc{A}_0$.

Our only requirement of $\base$ is that it attains a standard logarithmic regret bound in so-called mildly corrupt environments, defined below.
It's straightforward to show this is satisfied by classical stochastic MAB algorithms such as UCB \citep{LaiRo85} and Successive Elimination \citep{Even-Dar+02}.
We give proofs of these facts in \Cref{app:base}.

\begin{defn}\label{defn:mild}
	We say a finite-armed non-stationary bandit environment $\{ \mu_t(a)\}_{t \in [T], a \in \mc{A}_0}$ over horizon $T$ with armset $\mc{A}_0$ is {\bf mildly corrupt} if there exists a {\bf stationary reward profile} $\{ \mu(a)\}_{a \in \mc{A}_0}$ such that
\[
	\forall t \in [T] , a \in \mc{A}_0: |\mu_t(a) - \mu(a) | \leq \frac{1}{\sqrt{T}}.
\]
\end{defn}



\begin{assumption}\label{assumption:base}
	$\base(T,\mc{A}_0)$ attains, with probability at least $1-1/T$, for all $t \in [T]$, a $t$-round regret bound of
	\[
		\max_{a' \in \mc{A}_0} \sum_{s=1}^t \mu_s(a') - \mu_s(a_s) \leq C_0 \left( \sum_{i=2}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1}\{ \Delta_{(i)} \geq \sqrt{\log(T) / t} \} + \sqrt{t \log(T)} \right) . %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, T \cdot \Delta_{(2)} \right\} \right).
	\]
	in any $T$-round environment which is mildly corrupt with stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with ordered gaps $\Delta_{(2)} \leq \Delta_{(3)} \leq \cdots \Delta_{(|\mc{A}_0|)}$.
	%minimal gap
	%\[
		%\Delta_{\min} := \min_{a \in \mc{A}_0 \bs \{ \argmax_{a' \in \mc{A}_0} \mu(a') \} } \max_{a' \in \mc{A}_0} \mu(a') - \mu(a).
	%\]
\end{assumption}

%Next, our blackbox is surprisingly simple.
%In doubling epochs, we'll run $\base$ with a doubling set of subsampled arms and then restart the entire procedure based on checking the cumulative empirical regret $\sum_{s=1}^t 1 - Y_s(a_s) \gg \sqrt{t}$.
%This is captured in \Cref{alg:blackbox}.


\IncMargin{1em}
\begin{algorithm2e}[h]
 	\caption{{Blackbox Non-Stationary Algorithm}}
 \label{alg:blackbox}
 \bld{Input}: finite-armed MAB algorithm robust to mildly non-stationary environments $\base$. \\
 \bld{Initialize}: episode count $\ell \leftarrow 1$, first episode start round $t_1 \leftarrow 1$.\\
 \For{$m=1,2,\ldots,\ceil{\log(T)}$}{ \label{line:doubling}
		 Subsample $\ceil{2^{m/2}}$ arms $\mc{A}_m$ from the reservoir distribution.\\
		 Initiate a new instance of $\base(2^m,\mc{A}_m)$ with horizon $2^m$ and arm-set $\mc{A}_m$.\\
		 Let $t_{\ell}^m := t_{\ell} + 2^{m-1} - 1$ be the start of the $m$-th {\em block} in the $\ell$-th episode.\\
		 \For{$t = t_{\ell}^m,\ldots,t_{\ell}^m + 2^m$}{
			 Play arm $a_t$ as chosen by $\base(2^m,\mc{A}_m)$.\\
			 Obtain reward $Y_t(a_t)$ from $\base(2^m,\mc{A}_m)$.\\
			 \bld{Changepoint Test:} \uIf{$\sum_{s = t_{\ell}^m}^t 1 - Y_s(a_s) \geq C_1 \left( \sqrt{(t - t_{\ell}^m + 1) \log(T)} + \log(T) \right) $}{ \label{line:cpd-test}
				 Restart: $t_{\ell} \leftarrow t+1$, $\ell \leftarrow \ell+1$. \label{line:restart}\\
				 Return to \Cref{line:doubling} \jk{(Restart from $m=1$)}. 
                 % \textcolor{red}{**JK: This may mean starting from $m=1$?**} \joe{yes, one must restart from $m=1$}
		}
	}
}
		 %\Indp $\mc{A}_{t} \leftarrow \mc{A}_{t} \bs \left\{a\in [K]:\text{$\exists $ round $t_0 \leq t$ s.t. $\underset{a' \in \mc{A}_t}{\max} \sum_{s=t_0}^{t} \hat{\delta}_s(a',a) > C_5\sqrt{\sum_{s=t_0}^t \frac{\log(T)}{|\mc{A}_s|} }$ holds}\right\}$. \label{line:evict-At}\\
 		%\Indm
\end{algorithm2e}
\DecMargin{1em}


The main result of this section is that \Cref{alg:blackbox} in fact attains the optimal regret in terms of number of changes $L$ and total-variation $V$.
The proof is surprisingly simple with much of the difficulty of non-stationarity handled by our \Cref{assumption:base} on the base algorithm.

\begin{thm}\label{thm:blackbox}
	\Cref{alg:blackbox} satisfies, with probability at least $1-1/T$:
	\[
		{\normalfont \bld{R}}_T \leq \tilde{O} \left( \sqrt{(L+1) T} \land V^{1/3} T^{2/3} \right) .
	\]
\end{thm}

\begin{proof}
	Let $t_{\ell}$ be the the $\ell$-th restart round per \Cref{line:restart} of \Cref{alg:blackbox} so that $\ho{t_{\ell}}{t_{\ell+1}}$ is the $\ell$-th episode.
	Let $\hat{L}$ be the (random) number of restarts triggered over $T$ rounds.

	\paragraph*{$\bullet$ Using Empirical Regret Bound to get Regret Bound.}
	Next, we establish a high-probability event over which our empirical regret concentrates around its mean. First, fix an interval of rounds $[s_1,s_2]$.
	Then, we note that
	\[
		\sum_{s=s_1}^{s_2} Y_s(a_s) - \mb{E}[ Y_s(a_s) \mid \mc{H}_{s-1}],
	\]
	is a martingale difference sequence with respect to the natural filtration $\{\mc{H}_t\}_t$ of $\sigma$-algebras $\mc{H}_{t}$, generated by the observations and decisions (of both decision-maker and adversary) up to round $t-1$. Now, since the choice of arm $a_t$ at round $t$ is fixed conditional on $\mc{H}_{t-1}$, we have $\mb{E}[ Y_t(a_t) \mid \mc{H}_{t-1}] = \mu_t(a_t)$.
	% \textcolor{red}{**JK: I was just wondering the reason to use Freedman inequality.**} \joe{I need martingale concentration since R.V.'s are not iid, variance scaling is not important here and Azuma or Bernstein would have also sufficed. Later on, in proof of \Cref{thm:regret-episodes}, Freedman's variance scaling is important}
	Then, by Freedman's inequality (\Cref{lem:freedman}) we have with probability at least $1 - 1/T^3$,
	\[
		\left| \sum_{s=s_1}^{s_2} Y_s(a_s) - \mu_s(a_s)  \right| \leq 3 \sqrt{ (s_2-s_1+1) \cdot \log\left(2 T^3 \right) } + 2 \log\left( 2 T^3 \right) .
	\]
Let $t_{\ell}^m := t_{\ell+1}$ if the $(m-1)$-th block resulted in a restart, \jk{$m_\ell$ be the last block in the $\ell$-th episode, and $\hat{L}$ be the index of the last episode up to $T$.}	 Taking a further union bound over all choices of intervals $[s_1,s_2] \jk{\subseteq [T]}$, we have that, with probability at least $1 - 1/T$, 
     \jk{for all blocks of $[t_\ell^{m},t_\ell^{m+1})$ for $l\in[\hat{L}]$ and $m\in[m_\ell]$:}
     % for all final blocks $\ho{t_{\ell}^m}{t_{\ell+1}}$:
     \begin{align}
         	\left| \sum_{s=t_{\ell}^m}^{\jk{t_{\ell}^{m+1}-1}} (1 - Y_s(a_s)) - (1 - \mu_s(a_s)) \right| \leq 3\sqrt{ 3 (\jk{t_{\ell}^{m+1}}   - t_{\ell}^m) \log(2T)} + 6\log(2T).\label{eq:good_event1}
     \end{align}
	Let $\mc{E}_1$ be the good event on which this concentration of \eqref{eq:good_event1} holds for all episodes $\ell$ and blocks $m$.
    
	\jk{In what follows we show that}, summing over blocks and episodes, a regret bound of $\log(T) \sum_{\ell=1}^{\hat{L}} \sqrt{t_{\ell+1} - t_{\ell}}$ is evident on $\mc{E}_1$. 
    % \textcolor{red}{**JK: Could you explain this for me?**
		% Recall $t_{\ell}^m$ denote the start round of the $m$-th block in the $\ell$-th episode and let $t_{\ell}^m := t_{\ell+1}$ if the $(m-1)$-th block resulted in a restart.
		% Then,
     
\begin{lemma} \jk{Under $\mc{E}_1$, we have
    \[\sum_{t=1}^T 1-\mu_t(a_t)=\tilde{O}\left(\sum_{\ell\in[\hat{L}]}\sqrt{t_{\ell+1}-t_\ell}\right).\]}
\end{lemma}
    \begin{proof}
        
        We first decompose the regret along episodes and blocks contained therein:
		\[
			\sum_{t=1}^T 1 - \mu_t(a_t) = \jk{\sum_{\ell = 1}^{\hat{L}} \sum_{m\in [m_\ell]}} \sum_{t = t_{\ell}^m}^{t_{\ell}^{m+1}-1} 1 - \mu_t(a_t).
		\]
		% Then, on event $\mc{E}_1$, by Freedman, each inner sum $\sum_t 1 - \mu_t(a_t)$ concentrates around its mean $\sum_t 1 - Y_t(a_t)$ with concentration error
		% \[
		% 	\sqrt{(t_{\ell}^{m+1} - t_{\ell}^m) \cdot \log(T)} + \log(T).
		% \]
		Then, on event $\mc{E}_1$, we have:
        \begin{align*}
            \sum_{t=1}^T 1 - \mu_t(a_t)  &\lesssim
  \sum_{\ell\in [\hat{L}]} \sum_{m\in[m_\ell]}\left[ \sqrt{(t_{\ell}^{m+1} - t_{\ell}^m) \cdot \log(T)} + \log(T) + \sum_{t=t_{\ell}^m}^{t_{\ell}^{m+1} - 1} 1 - Y_t(a_t)\right].
        \end{align*}
		Then, we upper bound the last inner sum over $t$ on the RHS as follows
        \jk{\begin{align*}
            &\sum_{\ell\in [\hat{L}]}\sum_{m\in [m_\ell]} \sum_{t=t_\ell^m}^{t_\ell^{m+1}-1}1-Y_t(a_t)\cr &=\sum_{\ell\in [\hat{L}]}\sum_{m\in [m_\ell-1]} \sum_{t=t_\ell^m}^{t_\ell^{m+1}-1}1-Y_t(a_t)+\sum_{\ell\in [\hat{L}]} \sum_{t=t_\ell^{m_\ell}}^{t_\ell^{m_\ell+1}-2}1-Y_t(a_t)+\sum_{\ell\in [\hat{L}]} 1-Y_{t_\ell^{m_\ell+1}-1}(a_{t_\ell^{m_\ell+1}-1})
            \cr &\lesssim \sum_{\ell \in[\hat{L}]}\sum_{m\in [m_{\ell}]}\sqrt{(t_\ell^{m+1}-t_\ell^m)\log(T)}+ \hat{L}
             \cr &\lesssim \sum_{\ell \in[\hat{L}]}\sum_{m\in [m_{\ell}]}\sqrt{(t_\ell^{m+1}-t_\ell^m)\log(T)},
        \end{align*}
        where the first inequality is obtained from  the condition of \Cref{line:cpd-test} in Algorithm~\ref{alg:blackbox}.} Since
	the periods $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$ are doubling blocks for the  episode $\ho{t_{\ell}}{t_{\ell+1}}$, using Jensen's inequality, we can show that 
    \begin{align*}
        \sum_{m\in[m_\ell]}\sqrt{t_\ell^{m+1}-t_\ell^m}\le \sqrt{m_\ell \sum_{m\in[m_l]}(t_\ell^{m+1}-t_\ell^m)}=\tilde{O}(\sqrt{t_{\ell+1}-t_\ell}),
    \end{align*}
    which concludes the proof.
	\end{proof}

	\paragraph*{$\bullet$ Showing \Cref{line:cpd-test} is a Valid Changepoint Detection Test.}
	It then remains to show
	\[
		\sum_{\ell=1}^{\hat{L}} \sqrt{t_{\ell+1} - t_{\ell}} \leq \sqrt{(L+1) \cdot T} \land V^{1/3} T^{2/3},
	\]
	which amounts to showing \Cref{line:cpd-test} of \Cref{alg:blackbox} is a valid changepoint detection test which doesn't restart unnecessarily.



	Then, for large enough choice of threshold $C_1>0$ in \Cref{line:cpd-test}, we have that a restart in the $\ell$-th episode corresponds to large regret for the final block $\ho{t_{\ell}^m}{t_{\ell+1}}$:
	\begin{equation}\label{eq:large-regret-last-block}
		\sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(a_s) \geq C_2 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T) \right).
	\end{equation}
	Now, let $\mc{E}_2$ be the high-probability event of \Cref{assumption:base} holds.
	Then, it remains to show on event $\mc{E}_1 \cap \mc{E}_2$ that either (a) the regret of the best subsampled arm is large (indicating large variation) or (b) the subsampled bandit environment over the rounds $\ho{t_{\ell}^m}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).  \textcolor{red}{**JK: Could you explain this for me?**}
	\joe{sorry this explanation was rushed. Using the notation from below, we can decompose the regret  in the final block of the episode as
		\[
			\sum_{s=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(a_s) = \sum_s 1 - \mu_s(\hat{a}_{\ell,m}) + \sum_s \mu_s(\hat{a}_{\ell,m}) - \mu_s(a_s).
		\]
		Thus, we know from \Cref{eq:large-regret-last-block} that one of the two sums on the RHS above is large.
		If the first sum is large, we want to show this implies large variation must have elapsed in the episode.
		Our goal is to show in both situations that the variation over the episode is large or that $\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \gtrsim (t_{\ell+1} - t_{\ell})^{-1/2}$.\textcolor{red}{*jk: in the middle*}
	}

	Let $\hat{a}_{\ell,m}$ be the best arm in terms of initial reward among the arms $\mc{A}_m$ subsampled for block $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$.
	We first argue that with probability at least $1-1/T$,
	\[
		\mu_0(\hat{a}_{\ell,m}) > 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}.
	\]
	This is true since
	\begin{align*}
		\mb{P}(\mu_0(\hat{a}_{\ell,m}) < 1 - (t_{\ell+1} - t_{\ell}^m)^{-1/2}) &\leq \left( 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \right)^{|\mc{A}_0|} \\
										       &\leq \exp\left( - |\mc{A}_0| \cdot \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \right) \\
										       &\leq \frac{1}{T},
	\end{align*}
	where the last inequality follows from $|\mc{A}_0| \geq \sqrt{t_{\ell+1} - t_{\ell}^m}$.

	Now, using the regret decomposition of \Cref{eq:regret-decomp}, if
	\begin{equation}\label{eq:bad-reg-best}
		\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} 1 - \mu_s(\hat{a}_{\ell,m}) > 2\log(T)\sqrt{t_{\ell+1} - t_{\ell}^m},
	\end{equation}
	then we must have with probability at least $1/T$ that the variation must be at least
	\[
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}},
	\]
	since the adversary can only modify the rewards of arms $a_t$ after the round $t$ they're played. \textcolor{red}{**JK: Could you explain this for me?**}
	\joe{
	From our earlier tail probability bound, we know $\delta_0(\hat{a}_{\ell,m}) < \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}$.
	We also know from (3) above that there exists a round $t \in \ho{t_{\ell}^m}{t_{\ell+1}}$ such that
	\[
		\delta_t(\hat{a}_{\ell,m}) > \frac{2\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}}.
	\]
	This means the gap of arm $\hat{a}_{\ell,m}$ must have moved by amount $\frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^m}} \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}$ over the course of the block.
	Since the adversary can only modify the rewards of an arm $a_t$ after the round $t$ it is played, this must have occurred on a round where $\hat{a}_{\ell,m}$ was chosen by the agent.
	Thus,
	\[
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}}}.
	\]

}

	Suppose, going forward that \Cref{eq:bad-reg-best} is reversed.
	By our regret decomposition \Cref{eq:regret-decomp} and the restart criterion (\Cref{line:restart}) of \Cref{alg:blackbox}, for $C_1$ large enough, this must mean that:
	\[
		\sum_{t=t_{\ell}^m}^{t_{\ell+1}-1} \mu_s(\hat{a}_{\ell}^m) - \mu_s(a_s) \gtrsim \sqrt{(t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T).
	\]


	Then, we want to show that the subsampled bandit environment over the episode is not mildly corrupt. \textcolor{red}{**jk: <-could you explain why?**}
	\joe{basically, I want to arrive at a contradiction: if the subsampled bandit environment was only mildly corrupt, then the restart criterion (\Cref{line:restart}) would not be triggered.
	Taking the contrapositive of this statement, I want to show that if the restart criterion is triggered, then the subsampled bandit environment must be more heavily corrupt.
	}
	In other words, by \Cref{assumption:base}, we want to show by contradiction that if it were mildly corrupt with stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with gaps $\{ \Delta_a\}_{a \in \mc{A}_0}$, then:
	\begin{equation}\label{eq:bound-gap-rate}
		C_2 \left( \sqrt{ (t_{\ell+1} - t_{\ell}^m) \log(T)} + \log(T) \right) > C_0 \left( \sum_{i=3}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}}} \right\}  + \sqrt{ (t_{\ell+1} - t_{\ell}) \cdot \log(T)} \right). %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, (t_{\ell+1} - t_{\ell}) \cdot \Delta_{(2)} \right\} \right),
	\end{equation}
	%for any stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with ordered gaps $\Delta_{(2)} \leq \Delta_{(3)} \leq \cdots \Delta_{(|\mc{A}_0|)}$.
	We'll show this sub-claim by refining the sum over $i = 3, \ldots, |\mc{A}_0|$ into a geometric grid based on the values of the gaps and applying concentration over the number of gaps which fall within a particular segment of said grid.

	For $j = 0, \ldots, \ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}}{\log(T)} \right) }$, let $N_j := \sum_{j=3}^{|\mc{A}_0|} \pmb{1}\left\{ \Delta_{(j)} \in [ 2^{-(j+1)}, 2^{-j} ) \right\}$.
	Then, we bound
	\begin{align*}
		\sum_{i=3}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}}} \right\} &\leq \sum_{j=0}^{\ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}}{\log(T)} \right) }} N_j \cdot 2^{j+1}.
	\end{align*}
	Let $\mu_{m,(1)}$ be the top initial reward of the arms $\mc{A}_m$ subsampled during block $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$.
	Next, by a multiplicative Chernoff bound, since, conditional on $\mu_{m,(1)}$, the gaps are uniform random variables with order statistics $\Delta_{(2)},\ldots,\Delta_{(|\mc{A}_0|)}$.
	This means $N_j$ has mean $|\mc{A}_0| \cdot 2^{-(j+1)}$ so that:
	\[
		\mb{P}\left( N_j \geq 2 \cdot |\mc{A}_0| \cdot 2^{-(j+1)} \mid \mu_{m,(1)} \right) \leq \exp\left( - |\mc{A}_0| \cdot 2^{-(j+1)} / 3 \right).
	\]
	The RHS is less than $T^{-3}$ for $t_{\ell+1} - t_{\ell}$ sufficiently larger than a constant.
	Using tower law, the tail probability upper bound also holds unconditional of $\mu_{m,(1)}$, for all $j$.
	Let $\mc{E}_3$ be the corresponding high-probability event.

	Thus, on event $\mc{E}_1 \cap \mc{E}_2 \cap \mc{E}_3$, we have $N_j < 2 \cdot |\mc{A}_0| \cdot 2^{-(j+1)}$ and so
	\[
		N_j \cdot 2^{j+1} \leq 2 \cdot |\mc{A}_0|.
	\]
	Thus,
	\[
		\sum_{i=3}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1} \left\{ \Delta_{(i)} \geq \sqrt{ \frac{\log(T)}{t_{\ell+1} - t_{\ell}}} \right\} \leq 2 \ceil{ \half \log_2\left( \frac{t_{\ell+1} - t_{\ell}}{\log(T)} \right) } \cdot |\mc{A}_0| \leq 2\log(T) \cdot |\mc{A}_0|.
	\]
	Now,
	\[
		|\mc{A}_0| \leq \ceil{2^{m/2}} \leq \ceil{\sqrt{ t_{\ell+1} - t_{\ell}}}.
	\]

	Thus, \Cref{eq:bound-gap-rate} is shown which shows that the bandit environment over the rounds $\ho{t_{\ell}}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).

	This means that since the adversary can only modify the rewards of arms $a_t$ after the round $t$ they're played, the variation of change in each episode $\ho{t_{\ell}}{t_{\ell+1}}$ concluding with a restart must be at least
	\[
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{1}{\sqrt{t_{\ell+1} - t_{\ell}}}.
	\]
 
\jk{I'm currently struggling to understand that the left hand side above is increasing when the gap between $t_l$ and $t_{l+1}$ increases while the right hand side decreases. Could you provide some insights for it?}
\joe{Yes, this is a correct observation. The LHS increases as the episode duration $t_{\ell+1} - t_{\ell}$ increases while the RHS decreases.
	My intuition for this is as follows: if the episode $\ho{t_{\ell}}{t_{\ell+1}}$ is longer than that means we haven't detected a change over a longer period.
	This means the safe amount of total variation that can be accounted for in the episode is {\bf smaller} because our guarantees are more sensitive to small changes (i.e., finding a $T^{-1/2}$ optimal arm will be sensitive to $T^{-1/2}$ magnitude changes and thus sensitivitiy increases as $T$ increases).
	Viewed another way, \Cref{defn:mild} becomes more restrictive as $T$ increases.

	I think we can also view it the following way: if our \Cref{alg:blackbox} experiences a longer episode $\ho{t_{\ell}}{t_{\ell+1}}$, then that means it's very confident about the environment being stationary and finding the best arm over that episode.
	That higher confidence is more sensitive to a slight perturbation in the rewards which is why the threshold $(t_{\ell+1} - t_{\ell})^{-1/2}$ is smaller.
}

    This allows us to further bound the rate
	\[
		\sum_{\ell=1}^{\hat{L}} \sqrt{t_{\ell+1} - t_{\ell}} \leq \sqrt{(L+1) \cdot T} \land V^{1/3} T^{2/3}.
	\]
	In particular, the above is achieved using standard arguments seen in prior works \citep[Lemma 26]{wei2021} \citep[Corollary 2]{suk22}.
	%If we restart $\sum_{s=1}^t 1 - Y_s(a_s) \gtrsim \sqrt{t}$, then this means $\sum_{s=1}^t 1 - \mu_s(a_s) \gtrsim \sqrt{t}$.
	%This means large total variation must have elapsed in the environment so long as we have the base algorithm guarantee:
	%\[
		%\sum_{s=1}^t 1 - \mu_s(a_s) \lesssim \sqrt{t},
	%\]
	%in all environments with small total variation (at most $t^{-1/2}$ over $t$ rounds).
\end{proof}


\begin{rmk}
	At first glance, our base algorithm assumption (\Cref{assumption:base}) seems similar to Assumption 1 of \citet{wei2021}, but our base algorithm needs to maintain {\bf gap-dependent regret bounds} in environments with variation at most $T^{-1/2}$ which is stronger than their requirement of maintaining $\sqrt{KT}$ regret in nearly stationary $T$-round environments for $K$-armed bandits.
\end{rmk}

\begin{rmk}
	Bandit algorithm with optimal regret guarantees in {\bf stochastic regimes with adversarial corruption} \citep{lykouris18,zimmert19,ito21,ito23,dann23} would suffice for \Cref{assumption:base} as one can view our ``mildly corrupt'' regime as falling under these works' setting with corruption parameter of $T^{-1/2}$.
\end{rmk}


==> scrap/blackbox_v2_oldkappa.tex <==
\section{A Blackbox for Optimally Tracking Unknown Non-Stationarity}\label{sec:blackbox}

A key idea, introduced for the stationary problem in \citet{bayati20}, is that of {\em subsampling} a finite number of arms from the reservoir.
The main algorithmic design principle is to then run a finite-armed MAB algorithm over the subsampled arms.
The choice of number of arms to subsample is key here and exhibits its own exploration-exploitation tradeoff.
This tradeoff is best exemplified through the natural regret decomposition with respect to the subsampled set of arms, which we'll denote by $\mc{A}_0 \subseteq \mc{A}$:
%For minimizing regret over $T$ rounds, the minimax optimal regret of $\sqrt{T}$ can be achieved by subsampling $\sqrt{T}$ arms.

%In particular, within a sample of $\sqrt{T}$ arms, with high probability at least one arm will have reward at least $1-1/\sqrt{T}$.
%Then, it turns out one can reduce the problem to finite-armed bandits by subsampling $\sqrt{T}$ arms and then bounding regret between the subsampled arms:
%Thentural regret decomposition induced by a subsampled set of arms $\mc{A}_0$:
\begin{equation}\label{eq:regret-decomp}
	\sum_{t=1}^T \delta_t(a_t) = \underbrace{ \sum_{t=1}^T  1 - \max_{a \in \mc{A}_0} \mu(a)}_{\text{Regret of best subsampled arm}}  + \underbrace{ \sum_{t=1}^T  \max_{a \in \mc{A}_0} \mu(a) - \mu(a_t)}_{\text{Regret of played arms to best subsampled arm}}.
\end{equation}
Let's suppose there are $K := |\mc{A}_0|$ subsampled arms.
In what follows, we'll provide intuition for the $\beta=1$ case.
In fact, let's simplify matters by assuming the reservoir distribution is $\Unifu$.
Now, a sample of $K$ arms drawn from $\Unifu$ contains, with high probability, an arm with reward at least $1-1/K$ and, thus, gap at most $1/K$.
Thus, the first sum in \Cref{eq:regret-decomp} is at most $T/K$.

Then, plugging in the classical gap-dependent regret bounds for finite-armed MAB, the second term in \Cref{eq:regret-decomp} is $\tilde{O}\left( \sum_{a \in \mc{A}_0 \bs \argmax_{a' \in \mc{A}_0} \mu(a')} \Delta_{a}^{-1} \right)$ where $\Delta_{a}$ is the (random) gap of $a$ to the best subsampled arm.
Then, it is further shown \citep[Section A.2]{bayati20} that this gap-dependent quantity scales like $K\log(T)$ in expectation.

Then, we may choose $K$ to balance the bounds $T/K$ and $K \cdot \log(T)$ for which $K \propto \sqrt{T}$ is optimal giving a regret bound of $\sqrt{T}$.
As it turns out, the $\sqrt{T}$ regret rate is minimax.

Extending this to the non-stationary problem, it is first natural to ask whether we can follow the same strategy using a reduction to finite-armed non-stationary bandits.
However, this strategy poses two key difficulties:
\begin{enumerate}[(a)]
	\item Firstly, it's quite crucial in the above argument that the logarithmic gap-dependent regret bound was plugged in and not the gap-independent worst-case bound of $\sqrt{K T}$ (which would only lead to a suboptimal $T^{2/3}$ bound when optimizing $K$).

	As our goal in the non-stationary problem is to achieve {\em adaptive} regret bounds, free of parameter knowledge, a natural proposal is to reduce to $K$-armed non-stationary bandits and employ the known adaptive algorithms for this setting \citep{auer2019,wei2021,suk22,abbasi22}.
	However, it's long been known in this literature that no algorithm can adaptively secure a gap-dependent regret of $\sum_{\ell=1}^L \frac{K}{\Delta_{\ell,\min}}$ over $L$ stationary phases with minimal gaps $\Delta_{\ell,\min}$ \citep{garivier2011,lattimore}.
	This suggests we cannot do a full blackbox reduction to finite-armed non-stationary bandits.
	\item Secondly, we observe that upon experiencing changes, it may be necessary to {\em re-sample} arms from the reservoir distribution or else the first sum in \Cref{eq:regret-decomp} can become large if the rewards of all arms in $\mc{A}_0$ degrade over time.
	Thus, we require a more refined subsampling strategy which works in tandem with non-stationarity detection.
\end{enumerate}

We handle both of the above issues with the new idea of tracking the empirical regret $1 - Y_t(a_t)$ as a proxy for tracking non-stationarity.
The key observation is that the empirical cumulative regret of played actions up to round $t$, $\sum_{s=1}^t 1 - Y_s(a_s)$, concentrates around $\sum_{s=1}^t 1 - \mu_s(a_s)$ at a rate of $\sqrt{t}$ by Freedman's inequality.

This means, so long as $\sum_{s=1}^t 1 - Y_s(a_s) \lesssim \sqrt{t}$, our regret will be safe up to stationary rates.
On the other hand, if $\sum_{s=1}^t 1 - Y_s(a_s) \gg \sqrt{t}$, then the learner must be experiencing large regret.

On the other side, if the agent is playing according to an optimal algorithm for stationary infinite-armed bandits, then the only way large empirical regret is observed is if large non-stationarity has occurred.
Hence, checking empirical regret is a valid changepoint detection test.

Putting these observations together, our procedure (\Cref{alg:blackbox}), similar to the adaptive algorithms for the finite-armed setting \citep{auer2019,wei2021,suk22,abbasi22}, proceeds in episodes and restarts upon detecting non-stationarity.
A restart, or new episode, is triggered when the empirical regret over the current episode becomes too large.
Within each episode, we further employ doubling epochs, termed {\em blocks}, to account for unknown horizons and changepoints.


Going into more detail, our blackbox will rely on a stochastic finite-armed MAB base algorithm designed for stochastic environments, which we'll denote by $\base(t,\mc{A}_0)$, taking as input a horizon $t$ and finite subsample $\mc{A}_0$.

Our only requirement of $\base$ is that it attains a standard logarithmic regret bound in so-called mildly corrupt environments, defined below.
It's straightforward to show this is satisfied by classical stochastic MAB algorithms such as UCB \citep{lai} and Successive Elimination \citep{Even-Dar+02}.
We give proofs of these facts in \Cref{app:base}.

\begin{defn}\label{defn:mild}
	We say a finite-armed non-stationary bandit environment $\{ \mu_t(a)\}_{t \in [T], a \in \mc{A}_0}$ over horizon $T$ with armset $\mc{A}_0$ is {\bf $\alpha$-mildly corrupt} for $\alpha>0$ if there exists a {\bf stationary reward profile} $\{ \mu(a)\}_{a \in \mc{A}_0}$ such that
\[
	\forall t \in [T] , a \in \mc{A}_0: |\mu_t(a) - \mu(a) | \leq T^{- \frac{\alpha}{\alpha + 1}}.
\]
\end{defn}

\begin{assumption}\label{assumption:base}
	$\base(T,\mc{A}_0)$ attains, with probability at least $1-1/T$, for all $t \in [T]$, a $t$-round regret bound of
	\[
		\max_{a\in \mc{A}_0} \sum_{s=1}^t \mu_s(a) - \mu_s(a_s) \leq C_0 \left( \sum_{i=2}^{|\mc{A}_0|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1}\left\{ \frac{\Delta_{(i)}}{4} \geq \left(\frac{\log(T)}{t}\right)^{\frac{\alpha}{\alpha + 1}} \right\} + t^{\frac{1}{\alpha + 1}} \cdot \log^{\frac{\alpha}{\alpha+1}}(T) \right) . %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, T \cdot \Delta_{(2)} \right\} \right).
	\]
	in any $T$-round environment which is $\alpha$-mildly corrupt, for any $\alpha > 0$, with stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with ordered gaps $\Delta_{(2)} \leq \Delta_{(3)} \leq \cdots \Delta_{(|\mc{A}_0|)}$.
	%minimal gap
	%\[
		%\Delta_{\min} := \min_{a \in \mc{A}_0 \bs \{ \argmax_{a' \in \mc{A}_0} \mu(a') \} } \max_{a' \in \mc{A}_0} \mu(a') - \mu(a).
	%\]
\end{assumption}

\begin{rmk}
	At first glance, our base algorithm assumption (\Cref{assumption:base}) seems similar to Assumption 1 of \citet{wei2021}, but our base algorithm needs to maintain {\bf gap-dependent regret bounds} in environments with variation at most $T^{-1/2}$ which is stronger than their requirement of maintaining $\sqrt{KT}$ regret in nearly stationary $T$-round environments for $K$-armed bandits.
\end{rmk}

\begin{rmk}
	Bandit algorithm with optimal regret guarantees in {\bf stochastic regimes with adversarial corruption} \citep{lykouris18,zimmert19,ito21,ito23,dann23} would suffice for \Cref{assumption:base} as one can view our ``mildly corrupt'' regime as falling under these works' setting with corruption parameter of $T^{-1/2}$.
\end{rmk}
%Next, our blackbox is surprisingly simple.
%In doubling epochs, we'll run $\base$ with a doubling set of subsampled arms and then restart the entire procedure based on checking the cumulative empirical regret $\sum_{s=1}^t 1 - Y_s(a_s) \gg \sqrt{t}$.
%This is captured in \Cref{alg:blackbox}.


\IncMargin{1em}
\begin{algorithm2e}[H]
 	\caption{{Blackbox Non-Stationary Algorithm}}
 \label{alg:blackbox}
 \bld{Input}: Finite-armed MAB algorithm $\base$ satisfying \Cref{ass:reservoir}. Subsampling rate $S_m$.\\
 \bld{Initialize}: Episode count $\ell \leftarrow 1$, Starting time $t_1^1 \leftarrow 1$.\\
 \For{$m=1,2,\ldots,\ceil{\log(T)}$}{ \label{line:doubling}
	 Subsample $S_m$  arms $\mc{A}_m$ from the reservoir distribution.\\
		 Initiate a new instance of $\base(2^m,\mc{A}_m)$ with horizon $2^m$ and arm-set $\mc{A}_m$.\\
		 \For{$t = t_{\ell}^m,\ldots,(t_{\ell}^m + 2^m-1) \land T$}{
			 Play arm $a_t$ as chosen by $\base(2^m,\mc{A}_m)$.\\
			 Obtain reward $Y_t(a_t)$ from $\base(2^m,\mc{A}_m)$.\\

		 \bld{Changepoint Test:} \If{$\sum_{s = t_{\ell}^m}^t 1 - Y_s(a_s) \geq C_1 \cdot |\mc{A}_m| \cdot \log(T) $}{ \label{line:cpd-test}
				 Restart: $t_{\ell+1}^1 \leftarrow t+1$, $\ell \leftarrow \ell+1$. \label{line:restart}\\
				 Return to \Cref{line:doubling} (Restart from $m=1$).
                 % \textcolor{red}{**JK: This may mean starting from $m=1$?**} \joe{yes, one must restart from $m=1$}
		}
        \ElseIf{ $t=t_\ell^m+2^m-1$}{$t_{\ell}^{m+1}\leftarrow t+1$ (Start of the $(m+1)$-th {\em block} in the $\ell$-th episode).}
	}
}
		 %\Indp $\mc{A}_{t} \leftarrow \mc{A}_{t} \bs \left\{a\in [K]:\text{$\exists $ round $t_0 \leq t$ s.t. $\underset{a' \in \mc{A}_t}{\max} \sum_{s=t_0}^{t} \hat{\delta}_s(a',a) > C_5\sqrt{\sum_{s=t_0}^t \frac{\log(T)}{|\mc{A}_s|} }$ holds}\right\}$. \label{line:evict-At}\\
 		%\Indm
\end{algorithm2e}
\DecMargin{1em}


The main result of this section is that \Cref{alg:blackbox} in fact attains the optimal regret in terms of number of changes $L$ and total-variation $V$.
The proof is surprisingly simple with much of the difficulty of non-stationarity handled by our \Cref{assumption:base} on the base algorithm.

\begin{thm}\label{thm:blackbox}
	Under \Cref{ass:reservoir} with $\beta \geq 1$, \Cref{alg:blackbox} with $S_m := \ceil{C_2 2^{m \cdot \frac{\beta}{\beta+1}} \log(T)} \land 2^m$ satisfies, with probability at least $1-O(1/T)$:
	\[
		{\normalfont \bld{R}}_T \leq \tilde{O} \left( (L+1)^{\frac{1}{\beta+1}}  T^{\frac{\beta}{\beta+1}} \land (V^{\frac{1}{\beta+2}} T^{\frac{\beta+1}{\beta+2}} + T^{\frac{\beta}{\beta+1}}) \right) .
	\]
	If $\beta < 1$, \Cref{alg:blackbox} with $S_m := \ceil{ C_2 2^{m \cdot \beta/2} \log(T) } \land 2^m$ satisfies with probability at least $1 - O(1/T)$:
	\[
		{\normalfont \bld{R}}_T \leq \tilde{O} \left( \sqrt{(L+1) \cdot T} \land ( V^{1/3} T^{2/3} + \sqrt{T} ) \right).
	\]
\end{thm}

\begin{proof}{(Outline)}
	In this outline, we focus on the setting of $\beta \geq 1$.
	Modifications of the argument for $\beta < 1$ are detailed in \Cref{subsec:beta-small}.

	Let $t_{\ell} := t_{\ell}^1$ be the start round after the $\ell$-th restart in \Cref{alg:blackbox} so that $\ho{t_{\ell}}{t_{\ell+1}}$ is the $\ell$-th episode.
	Let $\hat{L}$ be the (random) number of restarts triggered over $T$ rounds. Let $m_\ell$ be the index of the last block in $\ell$-th episode.

	\paragraph*{$\bullet$ Converting Empirical Regret Bound to Per-Episode Regret Bound.}
	Next, we establish a high-probability event over which our empirical regret concentrates around its mean and so the changepoint test (\Cref{line:cpd-test} of \Cref{alg:blackbox}) can be related to the regret over each block.

	\begin{lemma}{(Proof in \Cref{subsec:proof-concentration-bounds})}\label{lem:concentration-bounds}
		Let $\mc{E}_1$ be the event that (1) for all blocks $\ho{t_{\ell}^m}{t_{\ell}^{m+1}}$,
		\begin{equation}\label{eq:block-bound}
			\sum_{s=t_{\ell}^m}^{t_{\ell}^{m+1}-1} \delta_s(a_s) < 3 C_1 \cdot |\mc{A}_m| \cdot \log(T).
		\end{equation}
		and (2) for the last block $\ho{t_{\ell}^{m_{\ell}}}{t_{\ell+1}}$ of episodes $\ho{t_{\ell}}{t_{\ell+1}}$ concluding in a restart, we have:
		\begin{equation}\label{eq:large-regret-last-block}
			\sum_{s=t_{\ell}^{m_{\ell}}}^{t_{\ell+1} - 1} \delta_s(a_s) \geq \frac{C_1}{2} \cdot |\mc{A}_{m_{\ell}}| \cdot \log(T).
		\end{equation}
		Then, $\mc{E}_1$ occurs with probability at least $1-1/T$.
	\end{lemma}

	Now, on event $\mc{E}_1$, we obtain a total regret bound of
	$\log^{2}(T) \sum_{\ell=1}^{\hat{L}} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}}$ on $\mc{E}_1$, by summing \Cref{eq:block-bound} over blocks and episodes .
    % \textcolor{red}{**JK: Could you explain this for me?**
		% Recall $t_{\ell}^m$ denote the start round of the $m$-th block in the $\ell$-th episode and let $t_{\ell}^m := t_{\ell+1}$ if the $(m-1)$-th block resulted in a restart.
		% Then,

\begin{lemma}{(Proof in \Cref{subsec:proof-regret-bd-ep-length})}\label{lem:regret-bd-episode-length}
	Under $\mc{E}_1$, we have
    	\[
		\sum_{t=1}^T \delta_t(a_t) \leq c_3  \log^2(T) \sum_{\ell\in[\hat{L}]} (t_{\ell+1}-t_\ell)^{\frac{\beta}{\beta+1}} .
	\]
\end{lemma}
\vspace{-2em}
\paragraph*{$\bullet$ Showing \Cref{line:cpd-test} is a Valid Changepoint Detection Test.}
Given \Cref{lem:regret-bd-episode-length}, it remains to %show a high probability bound for
	relate
	$
		\sum_{\ell=1}^{\hat{L}} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}}
	$
	to the total count $L$ of changes and total-variation $V$.
	To this end, we show there is sufficient variation in each episode $\ho{t_{\ell}}{t_{\ell+1}}$ which will allow us to conclude the total regret bound using standard arguments (\Cref{lem:regret-bd-nonstationarity}).

	%\Cref{line:cpd-test} of \Cref{alg:blackbox} is a valid changepoint detection test which doesn't restart unnecessarily.


    %In what follows, we define several high-probability events required for the bound. First of all, let $\mc{E}_2$ be the high-probability event that \Cref{assumption:base} holds.
	%% \[
	%% 	\mu_0(\hat{a}_{\ell,m_\ell}) > 1 - \frac{\log(T)}{2^{m_{\ell}/2}} \geq 1 - \frac{\log(T)}{\sqrt{t_{\ell+1} - t_{\ell}^{m_\ell}}}.
	%% \]
%Now, consider a stationary reward profile $\{\mu_0(a)\}_{a \in \mc{A}_{m_\ell}}$ with gaps $\{ \Delta_a\}_{a \in \mc{A}_{m_\ell}}$.
%
%
%For $j = 0, \ldots, \ceil{ \half \log_2\left( \frac{\jk{2^{m_\ell}}}{\log(T)} \right) }(:=J)$, let $N_{j,\ell} := \sum_{\jk{i=2}}^{|\mc{A}_{m_\ell}|} \pmb{1}\left\{ \Delta_{(\jk{i})} \in [ 2^{-(j+1)}, 2^{-j} ) \right\}$. Recall $\mu_0(\hat{a}_{\ell,m_\ell})$ is the top initial reward of the arms $\mc{A}_{m_\ell}$ subsampled for block $\ho{t_{\ell}^{m_\ell}}{t_{\ell}^{m_\ell+1}}$.
	%Since, conditional on $\mu_0(\hat{a}_{\ell,m_\ell})$, the gaps are uniform random variables with order statistics $\Delta_{(2)},\ldots,\Delta_{(|\mc{A}_{m_\ell}|)}$, it is true that $N_{j,\ell}$ has mean $(|\mc{A}_{m_\ell}|\jk{-1}) \cdot 2^{-(j+1)}$. By a multiplicative Chernoff bound, with large enough constant $C_2>0$, we have:\jk{
	%\begin{align*}
	    %\mb{P}\left( N_{j,\ell} \geq 2 \cdot (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)} \mid \mu_0(\hat{a}_{\ell,m_\ell}) \right) &\leq \exp\left( - (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)} / 3 \right)\cr &\leq \exp\left( - (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(J+1)} / 3 \right)\cr &\leq \exp\left( - (C_22^{m_\ell/2}\sqrt{\log(T)}-1) \cdot \sqrt{\frac{\log(T)}{2^{m_\ell}}} / 12 \right)\cr &\leq \frac{1}{T^3}.
	%\end{align*}}
	%% The RHS is less than $T^{-3}$ for $t_{\ell+1} - t_{\ell}$ sufficiently larger than a constant. \jkc{<-Why this holds? Do we need additional $\log(T)$ for $|A_m|$?}
%
%
 %%    \jk{tbd..}
	%Using tower law, the tail probability bound also holds unconditional of $\mu_0(\hat{a}_{\ell,m_\ell}) $.
	%Let $\mc{E}_4$ be the corresponding high-probability event of $\{N_{j,\ell}< 2 \cdot (|\mc{A}_{m_\ell}|-1) \cdot 2^{-(j+1)}; \forall j,   \forall \ell\}$.
%\jkc{Need the definition of $\mc{E}_3$ for the main.}
% , i.e. \[\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})| \gtrsim (t_{\ell+1} - t_{\ell})^{-1/2}.\]
We first introduce a regret decomposition, alluded to earlier in \Cref{eq:regret-decomp}, based on the ``best subsampled arm'', $\widehat{a}_{\ell,m_\ell}$: we decompose the regret in the last block $\ho{t_{\ell}^{m_{\ell}},t_{\ell+1}}$ of the $\ell$-th episode as
\begin{equation}\label{eq:regret-decompose-block}
			\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \delta_t(a_t) = \sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} \delta_{t}(\hat{a}_{\ell,m_\ell}) + \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t).
\end{equation}
    Then from the above display and \eqref{eq:large-regret-last-block}, one of two possible cases must hold: either
    \begin{align*}
	    \underbrace{ \sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} \delta_{t}(\hat{a}_{\ell,m_\ell}) \geq \frac{C_1}{4} |\mathcal{A}_{m_\ell}| \log(T) }_{ \mytag{(A)}{case1}} \text{ or } \\
	    \underbrace{ \sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} \delta_{t}(\hat{a}_{\ell,m_\ell}) < \frac{C_1}{4} |\mathcal{A}_{m_\ell}| \log(T) \text{ and } \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t) \geq \frac{C_1}{4} |\mathcal{A}_{m_\ell}| \log(T) }_{ \mytag{(B)}{case2}}.
	\end{align*}
	Our goal is to show that in either case \ref{case1} or \ref{case2}, large variation must have elapsed over the episode:
	\begin{equation}\label{eq:large-variation-ep}
		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq (t_{\ell+1} - t_{\ell})^{-\frac{1}{\beta+1}}.
	\end{equation}
%\[
	%\sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_t(a_t) = \sum_{t=t_\ell^{m_\ell}}^{t_{\ell+1}-1} 1 - \mu_{t}(\hat{a}_{\ell,m_\ell}) + \sum_{t=t_{\ell}^{m_\ell}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_\ell}) - \mu_t(a_t).
%\]
We first consider the former case \ref{case1}.
In this case, we know due to our subsampling rate $S_m$ that $\hat{a}_{\ell, m_{\ell}}$ will w.h.p. have an initial gap of $\tilde{O}( 2^{- m_{\ell} \cdot \frac{1}{\beta+1}})$.
On the other hand, \ref{case1} implies there is a round $t' \in \ho{t_{\ell}^m}{t_{\ell+1}}$ such that $\delta_{t'}(\hat{a}_{\ell,m_{\ell}}) \gtrsim |\mc{A}_{m_{\ell}}| / (t_{\ell+1} - t_{\ell}^{m_{\ell}}) \gtrsim 2^{- m_{\ell} \frac{1}{\beta+1}}$.
Thus, from $2^{- m_{\ell} \frac{1}{\beta+1}} \geq (t_{\ell+1} - t_{\ell})^{-\frac{1}{\beta+1}}$, \Cref{eq:large-variation-ep} holds.

Now, addressing case \ref{case2}, we suppose for contradiction that \Cref{eq:large-variation-ep} is reversed.
Then, this means the finite MAB environment experienced by the base algorithm is $\beta$-mildly corrupt (\Cref{defn:mild}).
Thus, we can use \Cref{assumption:base} to bound the regret of the base
\begin{equation}\label{eq:subsample-bound-block}
	\sum_{t=t_{\ell}^{m_{\ell}}}^{t_{\ell+1}-1} \mu_t(\hat{a}_{\ell,m_{\ell}}) - \mu_t(a_t) \leq C_0 \left( \sum_{i=2}^{|\mc{A}_{m_{\ell}}|} \frac{\log(T)}{\Delta_{(i)}} \cdot \pmb{1}\left\{ \frac{\Delta_{(i)}}{4} \geq \left(\frac{\log(T)}{t}\right)^{\frac{\beta}{\beta + 1}} \right\} + t^{\frac{1}{\beta + 1}} \cdot \log^{\frac{\beta}{\beta+1}}(T) \right) ,
\end{equation}
where $\{\Delta_{(i)}\}_{i = 1}^{|\mc{A}_{m_{\ell}}|}$ are the ordered gaps of the initial subsampled rewards.
Our goal is then to bound the RHS of \Cref{eq:subsample-bound-block} by $\frac{C}{2} |\mc{A}_{m_{\ell}}|$ to contradict \ref{case2}, which will imply \Cref{eq:large-variation-ep}.

\citet[Lemma D.4]{bayati20} also bound \Cref{eq:subsample-bound-block} by carefully integrating the densities of each $\Delta_{(i)}$.
However, this argment only works for bounding \Cref{eq:subsample-bound-block} in expectation and further requires additional regularity conditions on an assumed density for the reservoir distribution when $\beta \neq 1$ (op. cit. Section 6.1).
To contrast, we don't assume a density on the reservoir and bound \Cref{eq:subsample-bound-block} in high probability by using a novel binning argument on the values of the $\Delta_{(i)}$'s and using concentration on the number of arms whose gaps fall within each bin.

%We now show that the variation over the episode is large as follows using the following lemma whose proof is found in \Cref{subsec:proof-variation-bound}.\jkc{We may need the definition of $\mc{E}_4$ for the main part?}
The following lemma (proof in \Cref{subsec:proof-variation-bound}) summarizes our above discussion.

\begin{lemma}\label{lem:variation-bound}
	With probability at least $1-4/T$, for all $\ell\in [\hat{L}-1]$,
    \[
	    \sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_{t}(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq (t_{\ell+1} - t_{\ell})^{-\frac{1}{\beta+1}}.
	 \]
\end{lemma}

% Therefore, we have
% \begin{align}
%     \sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{1}{\sqrt{t_{\ell+1} - t_{\ell}}}.
% \end{align}


% Now we show that under Assumption~\ref{assumption:base} \Cref{eq:bound-gap-rate} is contradiction, which implies that the subsampled

% 	Thus, \Cref{eq:bound-gap-rate} is shown which shows that the bandit environment over the rounds $\ho{t_{\ell}}{t_{\ell+1}}$ is not mildly corrupt (\Cref{defn:mild}).

% This means that since the adversary can only modify the rewards of arms $a_t$ after the round $t$ they're played, the variation of change in each episode $\ho{t_{\ell}}{t_{\ell+1}}$ concluding with a restart must be at least
% 	\[
% 		\sum_{t=t_{\ell}}^{t_{\ell+1}-1} |\mu_t(a_{t-1}) - \mu_{t-1}(a_{t-1})| \geq \frac{1}{\sqrt{t_{\ell+1} - t_{\ell}}}.
% 	\]

% \jk{I'm currently struggling to understand that the left hand side above is increasing when the gap between $t_l$ and $t_{l+1}$ increases while the right hand side decreases. Could you provide some insights for it?}
% \joe{Yes, this is a correct observation. The LHS increases as the episode duration $t_{\ell+1} - t_{\ell}$ increases while the RHS decreases.
% 	My intuition for this is as follows: if the episode $\ho{t_{\ell}}{t_{\ell+1}}$ is longer than that means we haven't detected a change over a longer period.
% 	This means the safe amount of total variation that can be accounted for in the episode is {\bf smaller} because our guarantees are more sensitive to small changes (i.e., finding a $T^{-1/2}$ optimal arm will be sensitive to $T^{-1/2}$ magnitude changes and thus sensitivitiy increases as $T$ increases).
% 	Viewed another way, \Cref{defn:mild} becomes more restrictive as $T$ increases.

% 	I think we can also view it the following way: if our \Cref{alg:blackbox} experiences a longer episode $\ho{t_{\ell}}{t_{\ell+1}}$, then that means it's very confident about the environment being stationary and finding the best arm over that episode.
% 	That higher confidence is more sensitive to a slight perturbation in the rewards which is why the threshold $(t_{\ell+1} - t_{\ell})^{-1/2}$ is smaller.
% }



 %    This allows us to further bound the rate
	% \[
	% 	\sum_{\ell=1}^{\hat{L}} \sqrt{t_{\ell+1} - t_{\ell}} \leq \sqrt{(L+1) \cdot T} \land V^{1/3} T^{2/3}.
	% \]
	% In particular, the above is achieved using standard arguments seen in prior works \citep[Lemma 26]{wei2021} \citep[Corollary 2]{suk22}.\end{proof}

	%If we restart $\sum_{s=1}^t 1 - Y_s(a_s) \gtrsim \sqrt{t}$, then this means $\sum_{s=1}^t 1 - \mu_s(a_s) \gtrsim \sqrt{t}$.
	%This means large total variation must have elapsed in the environment so long as we have the base algorithm guarantee:
	%\[
		%\sum_{s=1}^t 1 - \mu_s(a_s) \lesssim \sqrt{t},
	%\]
	%in all environments with small total variation (at most $t^{-1/2}$ over $t$ rounds).
Using the above lemma, we can relate $\sum_{\ell=1}^{\hat{L}} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}}$ to $L$ and $V$ via standard arguments similar to Corollary 2 of \citet{suk22}, allowing us to conclude the proof when combining with \Cref{lem:regret-bd-episode-length}.

\begin{lemma}
%Under  $\mc{E}_1 \cap \mc{E}_2\cap \mc{E}_3\cap \mc{E}_4$
With probability at least $1-4/T$, we have
\[
	\sum_{\ell=1}^{\hat{L}} (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}} \lesssim (L+1)^{\frac{1}{\beta+1}} \cdot T^{\frac{\beta}{\beta+1}} \land ( T^{\frac{\beta}{\beta+1}} + V^{\frac{1}{\beta+2}} T^{\frac{\beta+1}{\beta+2}}).
\]
\label{lem:regret-bd-nonstationarity}
\end{lemma}
%Finally, we can conclude the proof for the regret bound from Lemmas~\ref{lem:regret-bd-episode-length} and \ref{lem:regret-bd-nonstationarity}
\end{proof}


==> scrap/constants.tex <==
{\color{Periwinkle}

\section*{\color{Periwinkle} Remarks on Algorithmic Knowledge of $\kappa_1,\kappa_2$}

\Cref{alg:blackbox} needs to know both $\kappa_1$ and $\kappa_2$ to achieve its regret bound (\Cref{thm:blackbox}).
Specifically, the constant $C_1$ in \Cref{line:cpd-test} needs to scale like $\Omega(\kappa_2^2/\kappa_1)$.

Meanwhile, \Cref{alg:elim} needs to know $\kappa_1$ to achieve its regret bound (\Cref{cor:elim-bounds}).
Specifically, the constant $C_3$ in \Cref{line:elim} needs to scale like $\Omega(1/\kappa_1^{1/\beta})$.

Intuitively, this is because in order to do changepoint detection (either through \Cref{line:cpd-test} of \Cref{alg:blackbox} or \Cref{line:elim} of \Cref{alg:elim}), we need to {\em know} what is the acceptable regret to pay over $T$ rounds which scales (for $\beta=1$) like $\sqrt{T}/\kappa_1$.
Therefore, the constants $C_1$ and $C_3$ need to scale like $\kappa_1^{-1}$.

Note that if, instead, we wanted to target a regret rate of $\sqrt{T}$ instead of $\sqrt{T}/\kappa_1$, then our subsampling rate $S_m$ or $|\mc{A}_m|$ would need to scale with $\kappa_1^{-1}$ instead.

If we wanted to avoid algorithmic knowledge of $\kappa_1$ entirely for \Cref{alg:elim}, we could just assume that $\log(T) > \kappa_1^{-1}$ and then not worry about $\kappa_1$ in the regret analysis.
However, this will lead to an additive $2^{1/\kappa_1}$ factor in the regret upper bound which could be much worse than a multiplicative scaling of $1/\kappa_1$. \jkc{we may say that $2^{1/\kappa_1}$ is a constant?}

In the previous works in stationary infinite-armed bandits, a similar phenomenon is observed in that we either need to know $\kappa_1$ or pick up a dependence on $\kappa_1^{-1}$ in the regret bound.

\begin{itemize}
	\item In Theorem 2 of \citet{carpentier15} , the constant $E$ needs to scale like $\kappa_1^{-1/\beta}$ and the constant $A$ in their definition of $\ol{T}_{\beta}$ (bottom of p. 4 therein) needs to depend on $\kappa_1$ for Theorem 2 to hold.
	\item The UCB-V algorithm of \citet{wang08} doesn't need to know $\kappa_1$ but has a $\kappa_1^{-1}$ dependence in the regret upper bound (Theorem 1 therein).
	\item The SS-UCB algorithm of \citet{bayati20} does not need to know $\kappa_1$, but also picks up a $\kappa_1^{-1}$ dependence in the regret upper bound of their Theorem 3.3.
	\item AUCBT \citep{kim24} does not seem to need to know $\kappa_1$?
\end{itemize}









}


==> scrap/tighter.tex <==
\section{Tighter Regret Bound for $\beta \in (0,1)$}

\com{this section is now outdated. All of the results here can be obtained through the results of \Cref{app:beta} instead.}


In this section, we show how to get a tighter $T^{\frac{\beta}{\beta+1}}$ regret bound in the stationary setting with $\beta \in (0,1)$.
We do this using the blackbox approach of \Cref{alg:blackbox} with some key modifications.

First, we give the necessary requirements for our finite MAB base algorithm.

\begin{assumption}\label{assumption:fixed-variance}
	Suppose the variane $\sigma_a^2$ of the random reward of each arm $a$ sampled from the reservoir remains the same across all rounds.
\end{assumption}


\begin{defn}\label{defn:mild-beta-small}
	We say a finite-armed non-stationary bandit environment $\{ \mu_t(a)\}_{t \in [T], a \in \mc{A}_0}$ over horizon $T$ with armset $\mc{A}_0$ is {\bf mildly corrupt} if there exists a {\bf stationary reward profile} $\{ \mu(a)\}_{a \in \mc{A}_0}$ such that
\[
	\forall t \in [T] , a \in \mc{A}_0: |\mu_t(a) - \mu(a) | \leq \frac{1}{T^{\frac{1}{\beta+1}}}.
\]
\end{defn}


\begin{assumption}\label{assumption:base-beta-small}
	$\base(T,\mc{A}_0)$ attains, with probability at least $1-1/T$, for all $t \in [T]$, a $t$-round regret bound of
	\[
		\max_{a' \in \mc{A}_0} \sum_{s=1}^t \mu_s(a') - \mu_s(a_s) \leq C_0 \left( \sum_{i=2}^{|\mc{A}_0|} \frac{\sigma_i^2 \log(T)}{\Delta_{(i)}} \cdot \pmb{1}\left\{ \Delta_{(i)} \geq \frac{\log(T)}{t^{\frac{1}{\beta+1}}} \right\} + t^{\frac{\beta}{\beta+1}} \log(T) \right) . %\min\left\{ \frac{\log(T)}{\Delta_{(2)}}, T \cdot \Delta_{(2)} \right\} \right).
	\]
	in any $T$-round environment which is mildly corrupt with stationary reward profile $\{\mu(a)\}_{a \in \mc{A}_0}$ with ordered gaps $\Delta_{(2)} \leq \Delta_{(3)} \leq \cdots \Delta_{(|\mc{A}_0|)}$ and with respective reward variances $\sigma_i^2$.
\end{assumption}

I believe the above assumption should hold for example with UCB-V \citep{audibert2007TuningBA}.
The assumption is definitely satisfied for the corruption-robust algorithm LB-INF \citep[Prop. 3]{ito22}\footnote{
Note these best-of-both-world algorithms like LB-INF also assume a unique optimal arm which shouldn't be a problem for us since this happens almost surely when subsampling from a continuous distribution.}

Now, consider running a blackbox algorithm where, in each doubling block of length $2^m$, we sample a set $\mc{A}_m$ of $\ceil{2^{m \cdot \frac{\beta}{\beta+1}}}$ arms from the reservoir and run $\base(2^m,\mc{A}_m)$.

\begin{prop}\label{prop:small-beta}
	For $\beta \in (0,1)$, the aforementioned blackbox algorithm gets a regret bound of $\tilde{O}(T^{\frac{\beta}{\beta+1}})$ in any $T$-round stationary environment.
\end{prop}

\begin{proof}{(Sketch)}
	First note that, over $T$ rounds, sampling $K = T^{\frac{\beta}{\beta+1}}$ arms is enough to secure an arm with gap $o(\log(T) \cdot T^{-\frac{1}{\beta+1}})$ whp.
	This is true since
	\[
		\mb{P}(\forall a \in [K]: \mu(a) \leq 1 - \log(T) \cdot T^{-\frac{1}{\beta+1}} ) = (1 - O(\log(T) \cdot T^{-\frac{\beta}{\beta+1}}))^K \leq \exp\left( - K \cdot \frac{O(\log(T))}{T^{\frac{\beta}{\beta+1}}} \right) = O(T^{-1}).
	\]
	Thus, it suffices to bound the plug-in regret bound from \Cref{assumption:base-beta-small}.

	The key idea in employing the variance $\sigma_i^2$ of the $i$-th best subsampled arm is that it will be small and cancel out the inverse gaps $\Delta_{(i)}^{-1}$.

	We start by noting that since the rewards are bounded in $[0,1]$: for $Y_{(i)}$ the random reward of $i$-th best subsampled arm: with mean $\mu_{(i)}$:
	\[
		\sigma_i^2 = \mb{E}[Y_{(i)}^2] - \mb{E}[Y_{(i)}]^2 \leq \mb{E}[ \mu_{(i)}^2 - \mu_{(i)} ] \leq \mb{E}[1 - \mu_{(i)}] = \mb{E}[ 1 - \mu_{(1)} ] + \Delta_{(i)}.
	\]
	Plugging this bound into the guarantee of \Cref{assumption:base-beta-small}, it remains to bound
	\[
		\sum_{i=2}^{K} \frac{1-\mu_{(1)}}{\Delta_{(i)}} \cdot \pmb{1}\left\{ \Delta_{(i)} \geq \frac{\log(T)}{T^{\frac{1}{\beta+1}}} \right\} + \sum_{i=2}^K \frac{\Delta_{(i)}}{\Delta_{(i)}} \cdot \pmb{1}\left\{ \Delta_{(i)} \geq \frac{\log(T)}{T^{\frac{1}{\beta+1}}} \right\} .
	\]
	As we already asserted that $1 - \mu_{(1)} \leq T^{-\frac{1}{\beta+1}}$ whp, we have the first sum above is $K \cdot T^{\frac{1}{\beta+1}} \cdot T^{-\frac{1}{\beta+1}} = K$.
	Meanwhile, the second sum is also order $K$.
	Thus, we have established a $T^{\frac{\beta}{\beta+1}}$ regret bound.
\end{proof}

\begin{rmk}
	I believe we can get rid of the fixed variance assumption (\Cref{assumption:fixed-variance}) by defining $\sigma_i^2$ more generally as $\min_{x \in [0,1]} \frac{1}{T} \sum_{t=1}^T \mb{E}[(Y_{t,i} - x)^2 ]$ os something similar.
	If defining $\sigma_i^2$ in this way is allowed in \Cref{assumption:base-beta-small}, then the proof of \Cref{prop:small-beta} should still go through as one can still show $\sigma_i^2 \leq 1 - \mu_i$.

	Thus, the main thing to check is whether \Cref{assumption:base-beta-small} holds for theteroscedastic rewards and this general notion of $\sigma_i^2$.
	Intuitively, I believe this to be true since UCB-V analysis relies on empirical Bernstein inequality which does not require identically distributed rewards.
	But, I need to check the proof more careefully.
\end{rmk}

%\section{Tighter Nonstationary Bound for $\beta\in(0,1)$ using Elimination}
%
%Here, I'll describe how to get optimal dynamic regret bound of
%\[
	%\tilde{O}\left( \min\{ T^{\frac{\beta+1/2}{\beta+1}} \cdot (\Lsig + 1)^{\frac{1/2}{\beta+1}}, (L+1)^{\frac{1}{\beta+1}} \cdot T^{\frac{\beta}{\beta+1}} , V^{\frac{1}{\beta+2}} \cdot T^{\frac{1+\beta}{\beta+2}} + T^{\frac{\beta}{\beta+1}}  \} \right),
%\]
%for $\beta \in (0,1)$ using a variant of \Cref{alg:elim}.
%The advantage of this over the previous approach is that we don't need to use any blackbox algorithm guarantees which may require homoscedastic rewards.
%
%We'll state the algorithm first.
%Notice the key substitutions (in blue) are respectively the number of subsampled arms per block and the elimination threshold.
%
%\IncMargin{1em}
%\begin{algorithm2e}[h]%\small
 	%\caption{{Elimination for Tracking Significant Shifts}}
 %\label{alg:elim-beta-small}
 %\bld{Initialize}: episode start round $t_0 \leftarrow 1$.\\
 %\For{$m=1,2,\ldots,\ceil{\log(T)}$}{ \label{line:restart}
	 %Subsample ${\color{blue} \ceil{2^{(m+1) \cdot \frac{\beta}{\beta+1}}}}$ arms $\mc{A}_m$ and let $\mc{G}_{t_0 + 2^{m-1} - 1} \leftarrow \mc{A}_m$.\\
		 %\For{$t = t_0 + 2^{m-1} - 1,\ldots,t_0 + 2^m$}{
			 %Play arm $a_t$ as $\Unif\{\mc{G}_t\}$ and observe reward $Y_t(a_t)$.\\
			 %Eliminate arms: $\mc{G}_{t+1} \leftarrow \mc{G}_t \bs \left\{ a \in \mc{A}_m  : \ds\sum_{s=t_0 + 2^{m-1} - 1}^t \hat{\delta}_s(a) \geq C \cdot {\color{blue} \ceil{ 2^{(m+1)\cdot \frac{\beta}{\beta+1}}}} \right\}$. \label{line:elim} \\
			 %\bld{Restart Test:} \uIf{$\mc{G}_{t+1} = \emptyset$}{
		 %Restart: $t_0 \leftarrow t+1$.\\
		 %Return to \Cref{line:restart}.
		%}
	%}
%}
		 %%\Indp $\mc{A}_{t} \leftarrow \mc{A}_{t} \bs \left\{a\in [K]:\text{$\exists $ round $t_0 \leq t$ s.t. $\underset{a' \in \mc{G}_t}{\max} \sum_{s=t_0}^{t} \hat{\delta}_s(a',a) > C_5\sqrt{\sum_{s=t_0}^t \frac{\log(T)}{|\mc{A}_s|} }$ holds}\right\}$. \label{line:evict-At}\\
 		%%\Indm
%\end{algorithm2e}
%\DecMargin{1em}
%
%\begin{thm}
	%\Cref{alg:elim-beta-small} achieves a regret bound of, w.p. at least $1-1/T$:
	%\[
		%\bld{R}_T \leq \tilde{O}\left( \min\{ T^{\frac{\beta+1/2}{\beta+1}} \cdot (\Lsig + 1)^{\frac{1/2}{\beta+1}}, (L+1)^{\frac{1}{\beta+1}} \cdot T^{\frac{\beta}{\beta+1}} , V^{\frac{1}{\beta+2}} \cdot T^{\frac{1+\beta}{\beta+2}} + T^{\frac{\beta}{\beta+1}}  \} \right),
	%\]
%\end{thm}
%
%\begin{proof}
	%Fix an episode and block and let $K$ be the number of subsampled arms.
	%Our main goal is to show that a concentration error bound on the aggregate regret estimates $\sum_{t\in I} \hat{\delta}_t(a)$ scaling like $O(K)$.
	%From this, the proof will follow similarly to the proof of \Cref{thm:upper-beta-small}.
%
	%To establish this concentration error bound, the key idea is to use a tighter variance-based concentration bound from Freedman's inequality (\Cref{lem:freedman}) that incorporates the second moments $\mb{E}[(1-Y_t(a))^2]$.
	%Then, by {\em self-bounding} (i.e., the fact that random variables in $[0,1]$ have second moments bounded above by first momenets), we use the critical fact that $\mb{E}[(1-Y_t(a))^2] \leq \delta_t(a)$.
	%Note by Freedman that for any arm $a$ retained on interval $I$:
	%\[
		%\left| \sum_{t\in I} \hat{\delta}_t(a) - \delta_t(a) \right|  \lesssim \sqrt{ \sum_{t\in I} \mb{E}[ (1 - Y_t(a))^2 \mid \mc{H}_{t-1}] \cdot |\mc{G}_t| } \leq \sqrt{\sum_{t\in I} \delta_t(a) \cdot |\mc{G}_t|} \leq \frac{1}{2} \sum_{t\in I} \delta_t(a) + \frac{K}{2},
	%\]
	%where the last inequality is by AM-GM.
	%Thus, an arm $a$ retained over interval $I$ implies its mean regret is bounded above by
	%\[
		%\sum_{t\in I} \delta_t(a) \lesssim K.
	%\]
	%On the other hand, if an arm $a$ is evicted over $I$, i.e. $\sum_{t\in I} \hat{\delta}_t(a) \gtrsim K$, then we must have
	%\[
		%\sum_{t \in I} \delta_t(a) \gtrsim K \geq |I|^{\frac{\beta}{\beta+1}}.
	%\]
	%This is also enough to conclude a per-episode regret bound of order $K = (t_{\ell+1} - t_{\ell})^{\frac{\beta}{\beta+1}}$.
	%\com{check above more carefully}
%
	%Now, an episode $\ho{t_{\ell}}{t_{\ell+1}}$ that terminates in a restart must then contain a significant shift.
	%Thus, we can conclude a
%
%
%\end{proof}


==> sigshift_discussion.tex <==
\section{Further Discussion of Significant Shifts and Comparison of Non-Stationarity Measures}


%However, so long as there's no rotting in the environment over $T$ rounds, there do exist algorithms (I was calling this ``proper'' earlier) for which no significant shift is recorded over $[T]$, e.g. \Cref{alg:blackbox} or \texttt{UCBT-ASW} \citep{kim24}.
%In other words, for these ``proper'' algorithms, \Cref{defn:sig-shift} is indeed a valid measure of significant rotting non-stationarity.

%\begin{prop}
	%Any algorithm achieving regret $O(T^{\frac{\beta}{\beta+1}})$ in all $T$-round stationary environments with probability at least $1/2$ must sample $\Omega(T^{\frac{1}{\beta+1}})$ arms.
	%We call this a {\bf proper} algorithm.
%\end{prop}
%
%\begin{proof}
	%Let $K$ be the number of arms sampled by the agent over $T$ rounds.
	%Let $\delta_{\min}$ be the minimum gap
	%We have by \Cref{ass:reservoir}:
	%\[
		%\mb{P}\left( \delta_{\min} \geq 1 - \frac{1}{2 \kappa_2 T^{\frac{1}{\beta+1}}} \right) \geq \left( 1 - \frac{1}{2 T^{\frac{\beta}{\beta+1}}} \right)^K \geq 0.5,
	%\]
	%where the second inequality follows from Bernoulli's inequality.
%\end{proof}

